ViSearch: Weak Consistency Measurement for Replicated Data Types

Large-scale replicated data type stores often resort to eventual consistency to guarantee low latency and high availability. It is widely accepted that programming over eventually consistent data stores is challenging, since arbitrary divergence among replicas is allowed. Moreover, pragmatic protocols actually achieve consistency guarantees stronger than eventual consistency, which can be and need to be utilized to facilitate the reasoning of and programming over replicated data types. Toward the challenges above, we propose the ViSearch framework for precise measurement of eventual consistency semantics. ViSearch employs the visibility-arbitration specification methodology in concurrent programming, which extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happen-before and linearization relations. The consistency measurement using ViSearch is NP-hard in general. To enable practical and efficient consistency measurement in replicated data type stores, the ViSearch framework refactors the existing brute-force checking algorithm to a generic algorithm skeleton, which further enables efficient pruning of the search space and effective parallelization. We employ the ViSearch framework for consistency measurement in two replicated data type stores Riak and CRDT-Redis. The experimental evaluation shows the usefulness and cost-effectiveness of consistency measurement based on the ViSearch framework in realistic scenarios.

==> ViSearch_complete_version/maintext/abs.tex <==
%--
\begin{abstract}

 Large-scale replicated data type stores often resort to eventual consistency to guarantee low latency and high availability. 
 It is widely accepted that programming over eventually consistent data type stores is challenging, since arbitrary divergence among replicas is allowed. 
 Moreover, pragmatic protocols actually achieve consistency guarantees stronger than eventual consistency, which can be and need to be utilized to facilitate the reasoning of and programming over replicated data types.
Toward the challenges above, we propose the \vs framework for precise measurement of eventual consistency semantics.
\vs employs the visibility-arbitration specification methodology in concurrent programming, which extends the linearizability-based specification methodology with a dynamic visibility relation among operations. %, in addition to the standard dynamic happen-before and linearization relations. 
The consistency measurement using \vs is NP-hard in general. To enable practical and efficient consistency measurement in replicated data type stores, the \vs framework refactors the existing brute-force checking algorithm to a generic algorithm skeleton, which further enables efficient pruning of the search space and effective parallelization.
We employ the \vs framework for consistency measurement in two replicated data type stores Riak and CRDT-Redis. 
The experimental evaluation shows the usefulness and cost-effectiveness of \vs in realistic scenarios.    

\end{abstract}

==> ViSearch_complete_version/maintext/concl.tex <==
%--
\section{Conclusion and Future Work} \label{Sec: Concl}

In this work, we develop the \vs framework for consistency measurement of eventually consistent replicated data type stores. 
In our framework, different consistency levels are specified via the relaxation of the visibility relations among operations.
The measurement of data consistency is based on the \vs algorithm skeleton, which enables efficient pruning of the search space and effective parallelization.
We employ the \vs framework for consistency measurement in two replicated data type stores Riak and CRDT-Redis. The experimental evaluation shows the usefulness and cost-effectiveness of consistency measurement based on the \vs framework in realistic scenarios.

Currently, the \vs framework is being integrated into the Jepsen framework \cite{Jepsen-GitHub} for black-box testing of distributed data stores (see details in the online repository of \vs \cite{ViSearch-GitHub}).
We will conduct more case studies to further demonstrate the usefulness of \vs on the basis of Jepsen testing.
%
In our future work, we will also investigate how to propose more predicate templates and extract efficient pruning predicates to further reduce the consistency measurement cost. 
Moreover, efficient heuristics can also be employed to reduce the search cost.

% Currently, the \vs framework is being integrated into the Jepsen framework \cite{Jepsen-GitHub} for black-box testing of distributed data stores (see details in the online repository of \vs \cite{ViSearch-GitHub}).
% We will conduct more case studies to further demonstrate the usefulness of \vs on the basis of Jepsen testing.
% In our future work, we will investigate how to propose more predicate templates and extract efficient pruning predicates to further reduce the consistency measurement cost. 
% Moreover, efficient heuristics can be employed to reduce the search cost.
% %We also need to explore load balancing techniques for the parallel \vs algorithm.
% Besides improvements on the \vs framework itself, we will conduct more case studies of realistic replicated data type stores and investigate whether semantic knowledge of the specific data type store can be effectively utilized to reduce the consistency measurement cost using \textsc{ViSearch}.

==> ViSearch_complete_version/maintext/exp.tex <==
%--
\section{Experimental Evaluation} \label{Sec: Exp}

In this section, we apply the \vs framework to consistency measurement in two open-source replicated data type stores.
The experiments are aimed at two research questions:

%--
\begin{itemize}
    \item RQ1. Can the \vs framework enable precise measurement of consistency semantics for eventually consistent replicated data types?
    \item RQ2. Is the consistency measurement based on \vs efficient?
\end{itemize}

%
%%--
%\begin{itemize}%[\itemindent=0.08cm]%[\itemindent=-0.08cm]
%    \item[RQ1.] Can the \vs framework enable precise measurement of consistency semantics for eventually consistent replicated data types?
%    \item[RQ2.] Is the consistency measurement based on \vs efficient?
%\end{itemize}

\noindent We first present our experiment setup and design, and then discuss the evaluation results.
The implementation of the \vs framework, as well as implementations, configurations and experiment scripts over the two replicated data type stores are available in our online GitHub repository \cite{ViSearch-GitHub}.

%--------------------------------------------------------------------------------
\subsection{Experiment Setup}

We employ \vs to conduct consistency measurement for Riak \cite{Riak} and CRDT-Redis \cite{CRDT-Redis}. 
Riak is a distributed NoSQL key-value database, which provides Riak-specific data types based on CRDTs. 
CRDT-Redis revises Redis, a popular in-memory data structure store with built-in replication, into a multi-master architecture and supports CRDT-based conflict resolution for concurrent updates on multiple master nodes.

We select three widely-used data container types, \textit{set}, \textit{map}, and \textit{priority queue}.
We further configure each container type we select as follows.
Riak exposes a parameter $r$ to the clients, which denotes how many replicas a query request must contact.
The two data types with different parameters $r$ $(r=1 \text{ or } 2$) are denoted \textit{Set-r1}, \textit{Set-r2}, \textit{Map-r1} and \textit{Map-r2} in our experiment. 
%
Each data type in CRDT-Redis is designed with different conflict-resolution strategies: add-win (\textit{A} in short), remove-win (\textit{R} in short), and the \rwf framework (\textit{F} in short) \cite{Zhang21}. 
Data types with different conflict-resolve strategies are denoted \textit{Set-A}, \textit{Set-R}, \textit{Set-F}, \textit{PQ-A}, \textit{PQ-R}, and \textit{PQ-F}. 

We run both data type stores in the Alibaba Cloud Elastic Compute Service (ECS) \cite{Alibaba-Cloud}. Each ECS server has two Intel Xeon Platinum CPU (2.50GHz), 4GB RAM, 40GB ESSD and 1MB/s network bandwidth. We build a Riak cluster with 5 servers, and replicate data types on 3 servers in the cluster. The CRDT-Redis cluster consists of 3 servers, and data types are replicated on all 3 servers. Another ECS server is dedicated to running the clients. 
%
The checking of data type access traces using \vs is conducted on one workstation with an Intel i9-9900X CPU (3.50GHz), with 10 cores and 20 threads, and 32GB RAM, running Ubuntu Desktop 16.04.6 LTS.

The basic workflow of consistency measurement using \vs is shown in Fig.~\ref{F: Exp}.
We first generate the workloads for each data type. 
%The workload module basically tells the clients what queries to send to the data store and when to issue the queries. %???
The clients record both the query and update invocation info, %(e.g., API name and arguments) 
and the return values %(e.g., the value returned by a query request and the ACK returned by an update request) 
for all queries issued.
All the info of data type access collected by the clients in one experiment forms one trace or history of data type access. 
Multiple traces of data type access are imported into the \vs module and \vs tells us the consistency levels of the traces measured. %, e.g., Co (complete visibility) or M (monotonic visibility). 
Detailed definitions of the consistency levels can be found in Section \ref{SubSec: Vis-Relax}.

% 单个client收集的叫info
% 所有client一起访问一个type，收集的叫一个trace，或者一个history。
% 一个实验，多次收集traces或者说histories。
% 这里，等于是把trace和history当成同义词。

%--
\begin{figure}[tb]
    \centering
    \includegraphics[width=0.9\linewidth]{figures/exp.pdf}
    \caption{\vs workflow.}
    \label{F: Exp}
\end{figure}


%\mybreak

%\slt{为了获得全面的trace，需要做的工作}


%--------------------------------------------------------------------------------
\subsection{Experiment Design} \label{SubSec: Exp-Design} 

The optimized trace checking using \vs (as detailed in Section \ref{Sec: VS}) still requires exponential time in the worst case. Thus we cannot directly apply \vs over CRDT access traces of arbitrary length. As inspired by the measurement in \cite{Emmi19}, we explore locality in consistency measurement over CRDT traces to circumvent the NP-hardness obstacle.

As for a CRDT, any replica can be modified without coordination with other replicas. Thus the replicas  may temporarily diverge. 
%When all updates are delivered to the replicas, possibly in different orders, the replicas converge, as required by the definition of eventual consistency \cite{Shapiro11a}.
We call the period when the replicas diverge the \textit{divergence interval}. 
Our key observation for consistency measurement is that, the consistency level of given trace is decided by the divergence intervals in the trace. Thus we only need to measure the divergence intervals in the trace, instead of measuring the whole trace of arbitrary length. The consistency level of the whole trace is decided by the divergence interval resulting in the weakest consistency level.
%
We can estimate the divergence interval by monitoring how large the number of updates in transmission can be. %during the experiment.
%
%monitoring the communication channel. According to the definition of eventual consistency, the replicas only diverge when the updates are still in transmission. 
%We estimate the maximum extent of divergence by monitoring how large the number of updates in transmission can be, during the experiment.
%
%We reproduce the experiments in our previous work %on CRDT design based 
%on CRDT-Redis \cite{Zhang21}.
%We set 1000 checkpoints for the replicas in the experiments where there are about 100,000 operations in the workload and the number of operations per second is up to 3000.
%
We find that the number of operations in transmission is bounded by 15 in our experiments. %, when the throughput is bounded by 3000 operations per second. 
Therefore we set the size of the workload, i.e., the number of operations to be sent to the data type, to 15. 
We let the clients launch the operations as quickly as possible to produce the maximal divergence.
Note that the specific value of the divergence interval is not essential in our experiment. 
In different experiment scenarios, we can estimate the divergence interval in the same way. 
%Generally speaking, the more the throughput of the data type store, the larger the divergence interval.


In our workloads, about 60\% operations are \textit{updates}, and about 40\% \textit{queries}. 
We randomly choose the parameters from a small interval of 0$\sim$5, which is no more than 1/3 of the workload size. 
This ensures that there exists sufficient collisions among operations.
As discussed above, each workload contains about 15$\sim$17 operations and 3$\sim$5 client threads share the operations in a workload. 

Note that the consistency measurement based on \vs is an approximation of the actual consistency semantics provided by the data type, since \vs cannot traverse the infinite space of possible traces.
%
To ensure the accuracy of our consistency measurement, we decide whether we have checked a sufficient number of traces in the Las Vegas manner \cite{Motwani95}.
%
We keep running \vs over the data type access traces round by round.
In each round, we check 100,000 traces. 
According to our experience in CRDT implementation and testing, 100,000 traces are large enough to cover all corner cases in the CRDT design.
%
%Then the \vs framework measures the consistency level of each trace, and 
The weakest consistency level measured over all the 100,000 traces is the measurement result in this round.
%
We stop the measurement when the measure results remain unchanged in 3 consecutive rounds.

%--------------------------------------------------------------------------------
\subsection{Evaluation Results} \label{SubSec: Eval-Results}

In light of our two research questions, we first discuss what the application developers and CRDT designers can obtain from our consistency measurement. 
Then we study the checking cost. 
We also study the effects of the two optimization techniques we develop. %, i.e., the pruning of the search space and the parallelization of the checking process.

%----------------------------------------
\subsubsection{Consistency Measurement Results}

We measure the consistency levels of 10 replicated data types from two data type stores. 
Due to different data type configurations and conflict resolution strategies, these replicated data types provide different consistency levels. %with high probability. 
We expect \vs can differentiate the consistency semantics of the 10 data types we study.
%
The measurement results are listed in Table. \ref{T: Result}. %, and each row is the experiment result of a replicated data type.
Each row of the table corresponds to one data type.
For each of the 6 consistency levels, we list the number of violations found by \textsc{ViSearch}.
The strongest consistency level with 0 violation (colored gray in the table) is the consistency level of the data type.
The `/' means that the checking is unnecessary and the violation must be zero, since there is no violation for stronger consistency levels.

We demonstrate the usefulness of the consistency measurement results from the perspective of the ``consistency-latency tradeoff", which is a refinement of the widely-used CAP theorem \cite{Brewer12, Gilbert12} and the PACELC tradeoff \cite{Abadi12} in CRDT scenarios.
Different CRDT designs and implementations principally have the same data update delay, since the replica is updated locally and the updates are propagated asynchronously. The query delay is also principally the same if the query only contacts one replica. In some data stores like Riak, the client can choose to contact multiple replicas, sacrificing certain query delay and improving the consistency level of the query.
Thus, from the perspective of the consistency-latency tradeoff, it is the consistency semantics of the data type which captures the primary differences in CRDT designs and implementations.
%
%We study whether the consistency measurement results can tell the CRDT designers and application developers the essential differences in different data types in our experiment.


The consistency measurement of CRDT-Redis data types demonstrates the different consistency semantics resulting from different conflict resolution strategies.
%that Redis replicated data types with different conflict-resolve strategies vary in consistency level. 
The priority queue \textit{PQ-R} with the remove-win strategy merely provides the ``Weak" consistency level, while the priority queue \textit{PQ-A} with the add-win strategy and \textit{PQ-F} with the \rwf framework both provide the stronger consistency level ``peer".
Moreover, the number of violations of the remove-win strategy is much larger than that of the other two strategies on the causal consistency level.
%The data type \textit{PQ-A} and \textit{PQ-F} satisfy the consistency level \textit{monotonic}, which guarantees the monotonic reads. 

Considering the high level design rationale, we may reasonably think that the remove-win strategy and the add-win strategy are dual of each other and are principally the same. However, the measurement by \vs shows important differences in the consistency semantics. 
%Add-win and remove-win are dual strategies. However, applied to a complex data type like the priority queue, the consistency semantics are different.
%The consistency level resulting from the add-win strategy is stronger ("Peer"), while the remove-win strategy provides weaker consistency level ("Weak").
%Moreover, the violations of the remove-win strategy are significantly more than those of the add-win strategy.
The \rwf framework is an improvement on the traditional remove-win strategy. The remove-win strategy puts the remove operation behind the non-remove operation. In \textsc{RWF}, the remove-operation just removes the element from the container, thus avoiding the conflict. This \rwf strategy, seen as an improvement of the traditional remove-win strategy, strengthens the consistency semantics to the same level with the semantics of the add-win strategy.
%further utilize the potential of the remove-win strategy. It not only eases the development, but also provides stronger consistency semantics.
The consistency measurement results can help the CRDT designers to further understand the semantics of different resolution strategies. The application developers can also use the measurement results to choose appropriate data types they actually need.

The consistency measurement results of the set data type have important differences with those of the priority queue data type.
As for the add-win and \rwf resolution strategies, the consistency level of \textit{Set-A} and \textit{Set-F} is still ``Peer", which is the same with the level of their counterparts \textit{PQ-A} and \textit{PQ-F}.
The main difference appears when considering the remove-win strategy. As for the set type, \textit{Set-R} also provides ``Peer", while \textit{PQ-R} only provides ``Weak".
The difference mainly results from that the priority queue has much more complex semantics than the set. When coping with complex semantics of the data type, the remove-win strategy will decrease the level of data consistency provided to the upper-layer applications. 
These measurement results show that the semantics of the data type should also be considered when choosing conflict resolution strategies. 

As for the Riak case, the configuration of parameter $r$ plays the most important role in the consistency measurement. The effect of $r$ can be quantified by the consistency measurement based on \textsc{ViSearch}.
%The measurement result of Riak data types is easier to explain. 
%The parameters $r$ dominates the consistency level of different Riak data types. 
%Data types provide a stronger consistency when $r$ is larger. 
We find that both data types merely provide the ``Weak" consistency level when $r=1$.
%In a high concurrency scenario, contacting only one replica before returning a query request guarantees a very weak data consistency. 
When $r=2$, a query request must contact a majority of replicas before returning. 
According to quorum-based protocol, data types with $r=2$ cannot strictly guarantee strong consistency. 
However, \textit{Set-r2} and \textit{Map-r2} actually provide strong consistency (the ``Complete" consistency level) in the experiment.
The measurement results show that when the network condition is relatively reliable and the communication delay is low, e.g., in an intra-datacenter environment, the ``$r=2$" configuration actually provides strong consistency, at least with high probability.
%because network condition is good in data center. 
This result is quite useful for applications which want strong consistency, but can tolerate data inconsistency in rare cases \cite{Wei17, Ouyang21}. 
%The limited sacrifice in data consistency can greatly reduce the query delay.

%--
\begin{table}[tb]
    \caption{Consistency measurement results.}
    \label{T: Result}
    \resizebox{\linewidth}{!}{  
        \begin{tabular}{|c|cccccc|l|l|}
            \hline
            & \multicolumn{6}{c|}{Violations}       &       &       \\ \cline{2-7}
            \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Data \\ Type\end{tabular}} & \multicolumn{1}{c|}{Co}            & \multicolumn{1}{c|}{Ca}       & \multicolumn{1}{c|}{P}        & \multicolumn{1}{c|}{M}        & \multicolumn{1}{c|}{B}        & W         & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}\# of \\ Histories\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Total \\ Time\end{tabular}} \\ \hline
            \textit{Set-r1}     & \multicolumn{1}{c|}{366}                      & \multicolumn{1}{c|}{339}                      & \multicolumn{1}{c|}{334}                              & \multicolumn{1}{c|}{295}       & \multicolumn{1}{c|}{188}       & \cellcolor[gray]{.8}0     & 300k          & 8h 3min      \\ \hline
            \textit{Set-r2}     & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}    & \multicolumn{1}{c|}{/}                        & \multicolumn{1}{c|}{/}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 300k          & 0h 11min      \\ \hline
            \textit{Map-r1}     & \multicolumn{1}{c|}{788}                      & \multicolumn{1}{c|}{734}                      & \multicolumn{1}{c|}{732}                                & \multicolumn{1}{c|}{712}    & \multicolumn{1}{c|}{542}      & \cellcolor[gray]{.8}0     & 300k          & 24h 26min       \\ \hline         
            \textit{Map-r2}     & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}    & \multicolumn{1}{c|}{/}                        & \multicolumn{1}{c|}{/}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 300k          & 0h 11min      \\ \hline
            \textit{PQ-A}       & \multicolumn{1}{c|}{478}                      & \multicolumn{1}{c|}{3}                        & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}            & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                        & 300k          & 4h 49min       \\ \hline                
            \textit{PQ-R}       & \multicolumn{1}{c|}{704}                      & \multicolumn{1}{c|}{131}                        & \multicolumn{1}{c|}{130}            & \multicolumn{1}{c|}{119}        & \multicolumn{1}{c|}{119}        & \cellcolor[gray]{.8}0                        & 300k          & 14h 17min       \\ \hline                
            \textit{PQ-F}       & \multicolumn{1}{c|}{1153}                      & \multicolumn{1}{c|}{3}                        & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}            & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                        & 300k          & 0h 18min       \\ \hline                
            \textit{Set-A}      & \multicolumn{1}{c|}{45}                        & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 500k          & 0h 19min         \\ \hline                
            \textit{Set-R}      & \multicolumn{1}{c|}{15}                        & \multicolumn{1}{c|}{4}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 400k          & 8h 9min         \\ \hline                
            \textit{Set-F}      & \multicolumn{1}{c|}{5}                        & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 500k          & 0h 19min         \\ \hline                
    \end{tabular}}
\end{table}

%----------------------------------------
\subsubsection{Consistency Measurement Cost}

To obtain the consistency measurement results in Table \ref{T: Result}, the checking time of \vs varies from 11 minutes to 24 hours. 
The consistency measurement time varies significantly for different data types. In our experiment 4 out of 10 types, \textit{Set-r1}, \textit{Map-r1}, \textit{PQ-R}, and \textit{Set-R}, require significantly more time than other data types. Thus for most data types, the number of traces checked can be increased to a much larger number (e.g., 1 million) in reasonable time. 
The checking time results demonstrate that consistency measurement using \vs can be accomplished under reasonable testing budget.
Also note that, the measurement process is not on the critical path of CRDT design, implementation, testing and maintenance. The consistency measurement can ``borrow" the traces from the testing process and be finished in parallel with the testing of CRDT implementations.

Besides the total checking time using \textsc{ViSearch}, we further study the effects of the optimizations we propose, namely the pruning of search space and the parallelization of checking.
%
We use \vs without pruning and parallelization as our baseline.
%
As for the parallelization of consistency measurement, we study two data types \textit{Set-r1} and \textit{PQ-F}.
We measure 100,000 traces and change the number of threads of checking from 1 to 16. 
 %Our second measurement demonstrates the impact of our parallel optimization consistency checking. 
%We check the consistency 100000 \textit{Set-r1} histories and 80000 \textit{PQ-F} histories with single thread checking as the baseline. 
%Then we use parallel {\vs} to check these histories with different thread number. 
As shown in Fig.~\ref{parallel}, the checking time decreases as we increase the number of threads, using pruning or not.
The decrease in time is quite significant when we increase the thread number from 1 to 6 in the cases of \textit{PQ-F} and \textit{Set-r1}. %, and 1 to 6 in the case of \textit{Set-r1}. 
As we add more threads, the checking time decreases approximately linearly. This means that the time decreases slowly than the ideal case where the time decreases to $\frac{1}{k}$ $(k$ is the number of threads).
%
This is mainly because the cost for thread scheduling increases when the thread number increases, which impacts the efficiency of parallelization. 
Also, when the thread number increases, the load balancing among threads becomes harder and more overloading/starvation of the threads will impact the efficiency of parallelization.
%
This evaluation results can tell us what the sweet points are, in order to choose the appropriate number of threads. 
It also motivates us to design better schemes to divide workloads among threads more efficiently.

%--
\begin{figure}[tb]
    \centering
    \subfigure[PQ-F] {
        \includegraphics[width=0.46\hsize]{figures/pq-f-bar.png}
    }
    \subfigure[Set-r1] {
        \includegraphics[width=0.46\hsize]{figures/set-r1-bar.png}
    }
    \caption{Evaluation of Time Cost.}
    \label{parallel}
\end{figure}




%--------------------
%\subsubsection{Efficacy of Filtering}
As for the pruning, we use the \textit{pruning ratio} as the performance metric. 
As for the checking of one data type access trace, we count the number of explored search states. 
We calculate the \textit{pruning ratio}, i.e. the ratio of the number of explored search states checked with the pruning to the number of states explored without the pruning.
%
For data types studied in the experiment, we pick one representative from multiple configurations of this data type. Specifically, we calculate the pruning ratio of four data types: \textit{Set-r1}, \textit{Map-r1}, \textit{Set-F}, and \textit{PQ-F}. %, and we check 10000 histories for each data type. 

As for the pruning ratio, we find that the effects of pruning significantly vary, as the number of search states (without pruning) increases. Our intuition is that the effects of pruning are more significant when there are more states to be explored by \textsc{ViSearch}, and the evaluation results prove this intuition correct.
Specifically, we divide the number of explored states without the pruning into four grades: \textit{small} ((0,30]), \textit{moderate} ([31, 300]), \textit{large} ([301, 3000]) and \textit{huge} ([3001, $+\infty$]).
As shown in Fig.~\ref{F: Pruning}, except for the `small' grade, the pruning can reduce the number of search states approximately by half. Note that, for `small' traces, the checking time is quite limited, with or without the pruning. This shows that, for the total checking time using the \vs framework, the pruning can significantly reduce the checking time (approximately by half).

One exception is \textit{Set-r1}. The pruning ratio of \textit{Set-r1} is more than 70\%, even for huge traces. This is mainly because \textit{Set-r1} provides weak visibility (see Table \ref{T: Result}), and the weak visibility checking takes most of the time. However, the weak visibility consistency predicate imposes few constraints on the visibility relation. We can find few pruning predicates conforming to the predicate template over all possible abstract executions. 
Therefore, the effect of pruning for \textit{Set-r1} is limited. 
%
We can further find that the pruning does not work well for the set type. Because the semantics of set only cares about the existence of elements and imposes fewer constraints on operations.
So we find fewer pruning predicates for the set type. 

%--
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{figures/pruningratio.png}
    \caption{Evaluation of State Filter}
    \label{F: Pruning}
\end{figure}


Besides the pruning ratio, we also directly compare the checking time with and without the pruning.
Note that the checking cost with pruning (the orange bars in Fig.~\ref{parallel}) includes the time for the extraction of pruning predicates.
%
In Fig.~\ref{F: Pruning}, \textit{PQ-F} has a better pruning ratio than \textit{Set-r1}, and this is reflected in the time cost. In Fig.~\ref{parallel}, the pruning also has a better effect in \textit{PQ-F} than in \textit{Set-r1}. The pruning reduces the checking time by half in most cases for \textit{PQ-F}, while the pruning reduces the checking time by less than 30\% for \textit{Set-r1}.

We also find in Fig.~\ref{parallel} that the effect of pruning becomes less significant as the number of threads increases.
Note that there is a sharp decrease in checking time as the number of threads goes beyond 4 in the \textit{PQ-F} case. 
It costs 0.36(0.30), 0.35(0.26), 0.26(0.21), 0.16(0.14) hours without(with) pruning when the number of parallel threads is 6, 8, 12, and 16.
The parallelization negatively affects the effect of the pruning, mainly because if any worker finds a certificate abstract execution, the searching process can be directly terminated.
Parallel checking greatly increases the odds of this type of early termination (in our searching, we can find some certificate abstract execution in most cases).
In light of the increased odds of early termination, the effects of pruning is significantly restricted as the number of worker threads increases.


==> ViSearch_complete_version/maintext/intro.tex <==
%--
\section{Introduction}

%\hy{背景}

Large-scale distributed systems often resort to replication techniques to achieve fault-tolerance and load distribution \cite{Burckhardt14, Shapiro11a, Enes19}. For a large class of applications, user-perceived latency and overall service availability are widely regarded as the most critical factors. Thus, many distributed systems are designed for low latency and high availability in the first place \cite{Lloyd13}. These systems have to trade data consistency for high availability and low latency \cite{Brewer12, Gilbert12}. A common approach is to resort to \textit{eventual consistency}, i.e., allowing data replicas to temporarily diverge, and making sure that these replicas will eventually converge to the same state in a deterministic way. The Conflict-free Replicated Data Type (CRDT) framework provides a principled approach to maintaining eventual consistency \cite{Shapiro11a, Burckhardt14}.

CRDTs are key components in modern geo-replicated systems, such as Riak \cite{Riak}, Redis-Enterprise \cite{Redis-Enterprise}, and Cosmos DB \cite{CosmosDB}. Though CRDT designs and implementations widely use the notion of eventual consistency, this is a rather fuzzy consistency term and covers a broad range of actual consistency behaviors. Providing only eventual consistency makes programming over CRDTs difficult, in the sense that there can be arbitrary divergence between the replicas \cite{Bermbach14, Lloyd13}. 

The tension between the wide use of eventual consistency and the difficulty of programming over eventually consistent CRDTs motivates the measurement of eventual consistency \cite{Bailis14-vldbj, Burckhardt14-book, Golab14}. On the one hand, both providers and consumers of the distributed storage service benefit from knowing the precise degree of data (in)consistency. Quantifying the degree of data inconsistency can even enable consumers and service providers to negotiate compensations proportional to the severity of violations in certain scenarios \cite{Golab11}.
On the other hand, pragmatic protocols, e.g. in Cassandra, Mongodb, and Eiger, actually achieve consistency guarantees stronger than eventual consistency \cite{Lloyd13}. 
Such stronger consistency semantics can be and should be utilized. Precise reasoning about the consistency semantics will significantly ease the burden of programming over CRDT data stores.

Existing consistency measurement schemes are mainly based on certain metrics delineating the staleness of data, e.g., how long the data has been stale \cite{Golab14} and how many new versions of data have been generated \cite{Golab18}.
%
Since the number of time units and that of data versions are numerical values, they simplify the issue of comparing different consistency semantics.
However, these consistency measurement schemes are external, i.e., they only describe in a black-box manner how consistent the data observed is.
%
We argue that, in order to better facilitate the programming over CRDTs, we need  white-box consistency measurement schemes which can give insights into how the data updates are propagated and observed across data replicas.

In this work we investigate a methodology for the precise measurement of eventual consistency semantics for CRDTs.
We employ a formal specification framework for concurrent objects \cite{Bermbach14, Emmi18, Emmi19}, which is based on the \textit{visibility} and \textit{arbitration} relation over operations in a data type access trace.
We name it the \textit{Visibility-Arbitration} framework (\visar in short).
The \visar framework extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happen-before and linearization relations. 
The arbitration relation is a total order and indicates how the system resolves conflicts among concurrent events. 
The visibility relation is an acyclic relation that describes the relative timing of update propagation among operations. 
%
The weaker the visibility relation, the more an operation is allowed to ignore the effects of concurrent operations that are linearized before it. 
%Tuning the definition of the visibility relation gives us different levels of data consistency. 
We use diverse constraints on the visibility relation to define different levels of data consistency.


Existing consistency measurement schemes based on the \visar framework are mainly designed for concurrent objects, 
which are optimized for high-performance multi-threaded code \cite{Emmi19, Emmi18}. 
Since concurrent objects often employ lock-free implementations and do not provide atomicity, the \visar framework is designed to measure the deviation from atomicity. 
However, in our scenarios, the replicated data types are designed to provide eventual consistency in the first place. %, and practical implementations often provide stronger semantics than the mere requirement of eventual consistency.
Our main objective is not to measure the deviation from strong consistency, but to measure the augmentation over weak consistency.

Though consistency measurement using the \visar framework is NP-hard in general \cite{Gibbons97, Emmi18}, brute-force checking algorithms are employed in practice \cite{Emmi19}. %in the measurement.
The key insight to circumvent the NP-hardness obstacle is that the violations are often local. That is, only a few operations can witness the violation. 
The small workload is repeated a sufficient number of (often millions of) times to find and measure the deviation from atomicity. 
%
However, the problem of eventual consistency measurement does not have the locality existing brute-force checking algorithms depend on.
We are confronted with the challenge of further optimizing existing checking algorithms.

Our intuition is that semantic knowledge of the data type under checking can be leveraged to reduce the measurement cost, while moderately sacrificing the generality of the measurement scheme.
Following this intuition, our first challenge is to refactor the brute-force consistency checking algorithm to a generic algorithm skeleton, which can conveniently incorporate semantic-aware optimizations.
The second challenge is to find the semantic information which can effectively reduce the checking cost while ensuring correct consistency measurement.

Toward the challenges above, we transform the brute-force checking algorithm for consistency measurement to a non-recursive algorithm skeleton.
Note that, the basic rationale of the measurement based on \visar is to enumerate all possible permutations of operations as well as all possible visibility relations among operations.
In the non-recursive algorithm skeleton, the intermediate state of enumeration is explicitly maintained at runtime.

Semantic knowledge of the data type under checking is expressed as \textit{pruning predicates}.
As indicated by its name, the pruning predicate prunes the state space while ensuring correct consistency checking.
We extract the pruning predicates from subhistories pertaining to one single data element. 
We enumerate all valid abstract executions over the subhistory and extract ``facts" which hold for all possible abstract executions.
Such facts are expressed as pruning predicates.
Given the generic algorithm skeleton for consistency checking, the pruning predicates can be flexibly ``plugged" into the \vs skeleton.
Whenever \vs finds violation of the pruning predicates, it can safely terminate the current search.
%
Moreover, since the construction of different abstract executions are independent, the search can be parallelized in a straightforward way.
We also periodically balance the load among the parallel worker threads.

We conduct consistency measurement experiments with \vs on two replicated data type stores Riak \cite{Riak} and CRDT-Redis \cite{CRDT-Redis}. 
%Since our optimization of the consistency checking algorithm is still exponential in the worst-case, it is still intractable to measure data type access traces of arbitrary length.
%As inspired by the application of the \visar framework in \cite{Emmi19}, we utilize the locality of consistency measurement in replicated data type scenarios, and measure the consistency of data type access traces at reasonable cost. We also study the effects of the pruning predicates and the parallelization through experiments.
The measurement quantifies the differences between different conflict resolution strategies, as well as the differences between different configurations of the replicated data type store. The consistency measurement results are useful for both replicated data type designers and upper-layer application developers.
The experiments also show the effects of our two optimizations and demonstrate the cost-effectiveness of \vs.

The rest of this work is organized as follows.
Section \ref{Sec: Preli} introduces the preliminaries of CRDTs and the \visar framework.
Section \ref{Sec: VS} presents the \vs framework, and Section \ref{Sec: Exp} presents the experimental evaluation.
Section \ref{Sec: RW} discusses the related work. 
In Section \ref{Sec: Concl}, we conclude this work and discuss the future work.


==> ViSearch_complete_version/maintext/preli.tex <==
%--
\section{Preliminaries} \label{Sec: Preli}

In this section, we first introduce the basic concepts of Conflict-free Replicated Data Types (CRDTs). Then we introduce the Visibility-Arbitration (\textsc{Vis-Ar}) framework and the consistency measurement based on visibility relaxation.

%--------------------------------------------------------------------------------
\subsection{Replicated Data Type}

We basically adopt the system model in \cite{Jiang20}.
We consider a replicated data store storing \textit{objects} of some abstract data type.

%--
\begin{definition}
    (Abstract Data Type). An abstract data type $\tau \in \textit{Type}$ is a pair $\tau = (\textit{Op}, \textit{Val})$ such that:
    \begin{itemize}
        \item \textit{Op} is the set of operations supported by $\tau$;
        \item \textit{Val} is the set of values allowed by $\tau$. We use $\perp \in \textit{Val}$ to denote that there is no return value for some operation. 
    \end{itemize}
\end{definition}

%--
\begin{definition}
    (Sequential Semantics). The sequential semantics of a data type $\tau \in \textit{Type}$ is defined by a function $\mathcal{F}_{\tau}: \textit{Op}^{*} \times \textit{Op} \rightarrow \textit{Val}$. It means that given a sequence of operations $S$ and an operation $o$, the return value of $o$ is $\mathcal{F}_{\tau}(S, o) \in \textit{Val}$ when $o$ is performed right after $S$. 
\end{definition}


We use ``$m(arg_1, \ldots, arg_n)\Rightarrow r$" to denote the invocation of a method $m$, with arguments $arg_1, \ldots, arg_n$, resulting in a return value $r$. 
We use the sequential semantics to explain the execution of operations. The return value of an operation is determined by a certain sequence of operations that are performed before or concurrent with it. 

In this work, we consider operations which are either \textit{queries} or \textit{updates}. 
Query operations only inspect state of the data type and do not change the state, while update operations modify state of the data type. 
Some data types may provide query-update primitives. %, i.e., operations inspect state of the data type and modify it at the same time. 
For example, the $extract\text{-}max()$ primitive of a priority queue is a query-update primitive. %, since it both obtains the maximum priority value and deletes the element with the maximum priority.
We can %rewrite the history with query-updates and 
decompose each query-update operation into a pair of query and update \cite{Wang19}. 
So we only consider query operations and update operations in this work. 

% The salient feature of the CRDT is that the update operations are handled immediately without communication with remote replicas. Then the updates are asynchronously propagated to remote replicas. 
% We often omit the return value of update operations as they usually only return \textsf{ACK}. 


% An implementation \textit{Impl} of a replicated data type is a mapping from operations sequence $o_1 o_2 \ldots o_n$ to a return value sequence $Impl (o_1 o_2 \ldots o_n)=r_1 r_2 \ldots r_n$. For a total order of operations conducted on the data type, the return values of query operations and effects of updates operations follow the semantics of the standard data types. As for concurrent and conflicting updates, the effects of the updates are decided by the semantics of the CRDT, which are rigorously specified by the CRDT protocol.
% The logics for querying multiple replicas and merging the results from different replicas are often left to the upper layer application.

%--------------------------------------------------------------------------------
\subsection{\visar Framework}

A consistency model acts as the contract between the underlying data type store and the upper-layer applications.
The \visar framework is an axiomatic consistency specification of concurrent objects \cite{Bermbach14, Emmi18, Emmi19}. 
It extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happens-before and linearization relations. 
The weaker the visibility relation, the more an operation is allowed to ignore the effects of concurrent operations that are linearized before it. 
Tuning the definition of the visibility relation gives us different levels of data consistency. We use various predicates (i.e., constraints) on the visibility relations to define different levels of data consistency.

% We consider an abstract notion of executions, or behaviors, which captures observed return values and platform-defined happens-before orders among invocations in a given program. 
% Histories, i.e., traces of data type access, are a set of observable behaviors $\mathcal{H}$. 
Histories, i.e., traces of data type access, are observable behaviors of a data store. 
The history defines how the clients interact with the data type store, and specifies what information is recorded about this interaction.
%--
\begin{definition}
    (History). A history is an event graph represented by a tuple $\mathcal{H} = (E, op, rval, so)$ such that:
    \begin{itemize}
        \item $E$ is the set of all events of operations performed by clients in a single execution; 
        \item $op : E \rightarrow Op$ describes the operation of an event; 
        \item $rval : E \rightarrow Val$ describes the return value of the operation $op(e)$ of an event $e$; 
        \item $so \subseteq E \times E$ is a partial order over $E$, called \textit{session order}. It describes the order of operations invoked by clients within a session. 
    \end{itemize}
\end{definition}

In this work, we only record the order between operations within the same session. The \textit{happen-before} relation %in this paper 
is limited to events/operations within the same session. 
We do not record the \textit{return-before} order over events which captures the real-time ordering of non-overlaping operations \cite{Burckhardt14-book}, since we do not have a global time in distributed scenarios. % considering the clock drifting.

%as there does not exist a unique write for each read operation in replicated data type scenarios. 

% Abstract Execution
In order to tell whether a history is consistent or not, the basic rationale underlying the \visar framework is that, a history is consistent if and only if we can justify it, by augmenting it with some additional information that explains the observed return values. 
%For example, the linearizability consistency model inserts commit points in the timeline to justify the correctness of the observed return values. 

Based on the \visar framework, we add arbitration (i.e., linearization) and visibility relations to a history, and the augmented history is called an \textit{abstract execution}.
%Abstract executions are histories enriched by additional information about visibility and arbitration. 
%In the Vis-ar framework, the methodology of checking consistency of an implementation is based on abstract executions. 
% * This allows us to define not just linearizability, but the 
% By turning the arbitration and visibility relations in abstract executions, we can define a spectrum of consistency models that are commonly used for eventually consistent data type stores. Specifically, \textit{arbitration} is a linearization or total order on operations which indicates how the system resolves conflicting updates.
% If an operation $a$ is arbitrated before $b$ (denoted by $a \stackrel{ar}{\rightarrow} b$), it means that the system considers operation $a$ to happen earlier than operation $b$. 

% The \textit{visibility} relation is an acyclic relation, which describes the relative timing of update propagation among operations.
% If an operation $a$ is visible to $b$ (denoted by $a \stackrel{vis}{\rightarrow} b$), it means that the effect of $a$ is visible to the client performing $b$. 
% In replicated data type stores where replicas communicate with each other via messages, this means that the replica that performs operation $b$ receives the message containing operation $a$ before operation $b$ was performed. 
% In this work, we use $vis$ to represent visibility relation. 
% Given the definition of $lin$ and $vis$, an abstract execution is defined as an event graph $\mathcal{A} = (E, op, rval, hb, ss, lin, vis)$. 
%where \textsf{vis} is an acyclic and natural relation, and \textsf{ar} is a total order. 

%--
\begin{definition}
    (Abstract Execution). An abstract execution is a triple $\mathcal{A} = ((E, op, rval, so), vis, ar)$ such that:
    \begin{itemize}
        \item $(E, op, rval, so)$ is a history;
        \item Visibility relation $vis \subseteq E \times E$ is an acyclic and natural relation. A relation $R \subseteq A \times A$ is natural if $\forall x \in A : \left\vert R^{-1}(x) \right\vert < \infty$;
        \item Arbitration relation $ar$ is a total order on $E$. 
    \end{itemize}
\end{definition}

If an operation $a$ is visible to $b$ (denoted by $a \stackrel{vis}{\rightarrow} b$), it means that the effect of $a$ is visible to the client performing $b$. 
If an operation $a$ is arbitrated before $b$ (denoted by $a \stackrel{ar}{\rightarrow} b$), it means that the system considers operation $a$ to happen earlier than operation $b$. 
We use $lin$ to denote the linearization of operations after we decide the arbitration for concurrent operations. 

\setlength\emergencystretch{\hsize}

% We introduce the notion of subhistory $\mathcal{H}' = (E', op', rval', hb', ss')$, which denotes the projection of history $\mathcal{H}$ on a subset of events $E' \subseteq E$. 
% The notions $op'$ and $rval'$ are $op$ and $rval$ restricted on $E'$ respectively.
% The happens-before order $hb'$ is defined as $hb' = hb \bigcap (E' \times E')$ and the same-session relation $ss'$ is defined as $ss' = ss \bigcap (E' \times E')$. 
% Similarly, we can define the notion of projection for an abstract execution. 
% The projection of an abstract execution $\mathcal{A}$ on $E'$ is $\mathcal{A'} = (E', op', rval', hb', ss', lin', vis')$, 
% where $(E', op', rval', hb', ss')$ is the projection of the original history on $E'$. 
% The arbitration $lin'$ is defined as $lin' = lin \bigcap (E' \times E')$ and the visibility relation $vis'$ is defined as $vis' = vis \bigcap (E' \times E')$. 

%--
\begin{definition}
    (Consistency Model). A consistency model is a set of consistency guarantees on abstract executions. 
    A consistency guarantee $\mathcal{\phi}$ is a constraint or property of an abstract execution $\mathcal{A}$. 
\end{definition}

We write $\mathcal{A} \models \mathcal{\phi}$ if the abstract execution $\mathcal{A}$ satisfies the consistency guarantee $\mathcal{\phi}$. 
We can define a large variety of consistency guarantees by formulating conditions on the various attributes and relations appearing in the abstract execution.
%
An abstract execution $\mathcal{A}$ satisfies consistency model $\Phi = \{\mathcal{\phi}_1, \mathcal{\phi}_2, \ldots, \mathcal{\phi}_n\}$, if it satisfies every consistency guarantees in $\Phi$. 
%Formally, $\mathcal{A} \models \Phi \Leftrightarrow \mathcal{A} \models \mathcal{\phi}_1 \land \mathcal{A} \models \mathcal{\phi}_2 \land \ldots \land \mathcal{A} \models \mathcal{\phi}_n$. 
%
A history $\mathcal{H}$ satisfies the consistency model $\Phi$, denoted $\mathcal{H} \models \Phi$, if it can be extended (by adding visibility and arbitration) to an abstract execution that satisfies consistency model $\Phi$. Formally, $\mathcal{H} (E, op, rval, so) \models \Phi \Leftrightarrow \exists vis, ar : ((E, op, rval, so), vis, ar) \models \Phi$. 

There are mainly two types of consistency guarantees. 
One is about the ordering of operations. This type of guarantees mainly consists of constraints on arbitration and visibility relations.
%guarantees (such as causality) that defines rules for reordering of operations, 
%and convergence guarantees that ensure eventual consistency. 
The other is about the data type semantics that gives meanings to the operations. %Every event in an abstract execution must have a return value which is allowed by the semantics $Impl$ of given replicated data type.

%----------------------------------------
\subsection{Consistency Measurement via Visibility Relaxation} \label{SubSec: Vis-Relax}

In \cite{Emmi19}, a consistency spectrum consisting of six consistency levels is defined by visibility relaxation. %, i.e., gradually relaxing the constraints on the visibility relations in the abstract execution.
These consistency levels, from weak to strong, are \textit{weak}, \textit{basic}, \textit{monotonic}, \textit{peer}, \textit{causal} and \textit{complete} visibility.
%
The two ends of the consistency spectrum are weak and complete visibility. The weak visibility permits any observation made by an operation, while the complete visibility requires that operations observe all operations which are arbitrated before them. 

Between these two ends, the basic visibility requires operations to see their happen-before predecessors which corresponds to a strengthening of the read-your-writes guarantee. 
%
The monotonic visibility requires each operation to see those operations its happen-before predecessors see. 
It corresponds to the monotonic reads guarantee. %, which states that read operations observe an increasing set of updates. 
%
On the basis of the monotonic visibility, the peer visibility requires a read to observe an update only if it has observed all the predecessors from the update's session.
This corresponds to the monotonic writes guarantee.
%
The causal visibility requires that the visibility relation be transitive. It means that each operation is required to see those operations visible to the operations it sees. 
%

We define a set of predicates which constraint the observation made by a given operation. 
Formally, a visibility predicate $\varphi(o, \mathcal{A})$ is a first-order predicate on operation $o$ in an abstract execution $\mathcal{A}$. Given an abstract execution $\mathcal{A}$, we define $vis(o)$ is a set of operations visible to $o$; $hb(o)$ is a set of operations that happens before $o$ according to the session order $so$; $lin(o)$ is a set of operations arbitrated before $o$. 
\begin{itemize} \label{vis-level}
    \item weak$(o, \mathcal{A}) \Leftrightarrow \textbf{\textit{true}}$
    \item basic$(o, \mathcal{A}) \Leftrightarrow hb(o) \subseteq vis(o)$
    \item monotonic$(o, \mathcal{A}) \Leftrightarrow \forall o' \in hb(o): vis(o') \subseteq vis(o)$
    \item peer$(o, \mathcal{A}) \Leftrightarrow$ monotonic$(o, \mathcal{A}) \land \forall o' \in vis(o): hb(o') \subseteq vis(o)$ 
    \item causal$(o, \mathcal{A}) \Leftrightarrow$ basic$(o, \mathcal{A}) \land \forall o' \in vis(o): vis(o') \subseteq vis(o)$ 
    \item complete$(o, \mathcal{A}) \Leftrightarrow lin(o) \subseteq vis(o)$
\end{itemize}

In Fig.~\ref{F: Visibility} we illustrate these four consistency levels by examples, which are inspired from \cite{Emmi19}. 
The operations (rounded rectangle) visible to the given operation (bold rounded rectangle) depend on the visibility level. 
The \textit{basic} visibility implies visibility (solid arrow) of happens-before predecessors (horizontal line) while the \textit{monotonic} visibility implies visibility of those visible (dashed arrow) to predecessors. 
The \textit{peer} visibility implies visibility of predecessors of visible operations, and the \textit{causal} visibility implies transitive visibility. 
%
In the rest of this work, we use this 6-level scale of consistency levels for the consistency measurement.

%We define a set of predicates which constrain the observation made by a given operation.
%Formally, a visibility predicate $\varphi(o, \mathcal{A})$ is a first-order predicate on operation $o$ in an abstract execution $\mathcal{A}$. 
%Given an abstract execution $\mathcal{A}$, we define $vis(o)$ as a set of operations visible to $o$, define $hb(o)$ as a set of operations that happens before $o$ according to the session order $so$, and define $lin(o)$ as a set of operations arbitrated before $o$.
%The six consistency levels we use can be defined as:
%%--
%\begin{itemize}[leftmargin=*]
%    \item weak$(o, \mathcal{A}) \Leftrightarrow \textbf{\textit{true}}$
%    \item basic$(o, \mathcal{A}) \Leftrightarrow hb(o) \subseteq vis(o)$
%    \item monotonic$(o, \mathcal{A}) \Leftrightarrow \forall o' \in hb(o): vis(o') \subseteq vis(o)$
%    \item peer$(o, \mathcal{A}) \Leftrightarrow$ monotonic$(o, \mathcal{A}) \land \forall o' \in vis(o): hb(o') \subseteq vis(o)$ 
%    \item causal$(o, \mathcal{A}) \Leftrightarrow$ basic$(o, \mathcal{A}) \land \forall o' \in vis(o): vis(o') \subseteq vis(o)$ 
%    \item complete$(o, \mathcal{A}) \Leftrightarrow lin(o) \subseteq vis(o)$
%\end{itemize}


% In Figure \ref{F: Visibility}, 
%visibility of predecessors of visible operations


%--
\begin{figure}[tb]
    \includegraphics[width=\linewidth]{figures/visibility.pdf}
    \centering
    \caption{Examples of four consistency levels.}
    \label{F: Visibility}
\end{figure}

Basically, the consistency measurement is conducted on one history or trace of replicated data type access. Theoretically speaking, to measure the consistency level of one data type, we need to measure all possible (infinitely many) traces of this data type, which is simply not possible. Moreover, it is usually quite difficult to strictly prove the consistency level certain replicated data type provides. In this work, when we say consistency measurement for one data type, we mean that a sufficiently large number of traces generated by this data type are measured, and the result of this measurement is a sufficiently accurate approximation of the consistency level provided by this data type (more details can be found in Section \ref{SubSec: Exp-Design}).


==> ViSearch_complete_version/maintext/rw.tex <==
%--
\section{Related Work} \label{Sec: RW}

%\hy{怎么规约}

The fuzzy nature of eventual consistency and its wide adoption motivate the quantification of severity of consistency violations \cite{Golab11, Golab14, Golab18}. Existing quantification techniques can be viewed from two perspectives. From the micro-perspective, existing consistency measurement schemes are mainly based on certain metrics delineating the staleness of data, e.g., how long the data has been stale and how many new versions of data have been generated.
%The metric can be how long the data has been stale, e.g. $\Delta$- and $\Gamma$-consistency \cite{Golab14}, and how many new versions of data has been generated, e.g. $k$-atomicity \cite{Golab18}. 
Time-based quantification techniques, e.g. $\Delta$-atomicity \cite{Golab11} and $\Gamma$-atomicity \cite{Golab14}, are adopted for applications sensitive to realtime consistency requirements. Time-based techniques measure data consistency by how many time units the value returned has been stale. 
For applications sensitive to the frequency of data updates, version-based quantification techniques , e.g. k-atomicity \cite{Golab18}, are proposed. Version-based techniques measure data consistency by how many times the data has been updated when the returned value is obtained.
From the macro-perspective, Yu and Vahdat propose TACT (Tunable Availability and Consistency Tradeoffs), a middleware layer that supports application-dependent consistency
semantics expressed as a vector of metrics defined over a logical consistency unit or conit \cite{Yu02-TOCS}. Inconsistencies in the observed value of a conit are bounded using three metrics: numerical error, order error, and staleness.

The consistency measurement schemes above are from the end user's perspective. In order to better facilitate the development of upper-layer applications, we need measurement schemes which focus on how data items are updated, in a similar way with how linearizability is specified. To this end, in this work we borrow the \visar framework which is an axiomatic consistency specification framework of concurrent objects. %which consider operation visibility. 
The \visar framework extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happens-before and linearization relations. 
The \visar framework is more suitable for developers to reason about the correctness of the implementation of a replicated data type. It is also suitable for upper-layer application developers to reason about the correctness of applications.

%\hy{关于checking}

The checking of data type access traces is NP-Complete in general \cite{Gibbons97}.
However, this intractability result can be circumvented by reasonable assumptions in specific scenarios. For example, the write values are often assumed to be unique %, which can makes the checking problem tractable in many scenarios 
\cite{Gibbons97}. This assumption is reasonable and easy to satisfy, since we can append certain meta-data to the values written to make them unique. 
In replicated data type store scenarios, the number of concurrent writes is often assumed to be bounded by some constant \cite{Golab18}. 
Practitioners can also limit the pattern of the input and derive an input specific efficient checking algorithm \cite{Bouajjani17}. 

The checking of data type access traces using \vs is also intractable in the worst case. As inspired by the existing techniques to circumvent the NP-hardness obstacle, we refactor the brute-force checking algorithm to a generic algorithm skeleton. This refactor enables practical pruning of the exponential search space. We also employ the locality of the checking of CRDT access traces to make the consistency measurement practical in realistic replicated data type store scenarios.

%\slt{关于粒度}
% The existing work measures the consistency of Java's concurrent objects at the per-method granularity \cite{Emmi19}. 


==> ViSearch_complete_version/maintext/vs.tex <==
%--
\section{\vs Framework} \label{Sec: VS}

In this section, we first overview the basic design rationale behind the \vs framework. Then we present the key techniques. In the next Section \ref{Sec: Exp}, we will demonstrate how to apply \vs in realistic data type store scenarios.

%--------------------------------------------------------------------------------
\subsection{\vs  Overview}

Consistency measurement using \vs boils down to the search of an abstract execution satisfying certain constraints on the arbitration and visibility relations. 
This search process involves enumerating the linearizations, i.e. arbitrations of all operations, as well as the visibility relations among operations.
To prove that one trace satisfies certain consistency model, it is sufficient to find one single abstract execution that satisfies all the constraints. % on the arbitration and visibility relations.
We name this abstract execution the \textit{certificate abstract execution} (there could be more than one certificate execution).
%The success in finding one single abstract execution which satisfies the consistency model can prove that the trace satisfied certain consistency model
%Below we note arbitration as linearization because arbitration is actually a permutation of all operations. 
%The checking of each consistency level boils down to finding an arbitration of as well as the visibility among all operations. 

The search process is intractable in general \cite{Gibbons97, Emmi19, Emmi18}. However, the search can still be practical and cost-effective in replicated data type store scenarios. %, since the traces in real scenarios do not always force the checking algorithm to the worst case.
To enable efficient search of abstract executions, we first refactor the existing recursive search algorithm to a non-recursive algorithm skeleton.
The intermediate states for construction of the abstract executions are explicitly maintained by the algorithm skeleton at runtime. 


Based on the \vs skeleton, we propose optimizations from two orthogonal dimensions. 
First, the non-recursive algorithm skeleton enables efficient pruning of the search space. 
We can flexibly plug pruning predicates into the algorithm skeleton to avoid the unnecessary search of certain abstract executions. 
The pruning predicates can be automatically extracted from the subhistory concerning multiple update operations and one query operation on one single data element. 
Second, we find that the enumeration of different candidate executions are independent. Thus we further parallelize the search. 
The non-recursive search skeleton also facilitates the load balancing among the parallel worker threads.

%--------------------------------------------------------------------------------
\subsection{\vs Algorithm Skeleton}

We first briefly review the existing recursive search algorithm \cite{Emmi19, Emmi18}. Then we present the non-recursive algorithm skeleton.

%----------------------------------------
\subsubsection{The Original Recursive Search Algorithm}

Consistency measurement using the \vs framework can simply use a recursive backtracking algorithm to search the possible arbitration and visibility relations among operations in a brute-force manner. We use $\ang{lin, vis}$ to denote an abstract execution. If an abstract execution $\ang{lin, vis}$ satisfies a consistency model $\Phi$, we have $\langle lin, vis \rangle \models \Phi$. 
During the search process, we manipulate some prefix of $lin$, denoted by $lin_i$. We use $vis_i$ to denote the visibility relation on operations in $lin_i$. 
The search algorithm can be viewed as extending candidate executions from $\ang{lin_i, vis_i}$ to $\ang{lin_{i+1}, vis_{i+1}}$.


%It is intuitive that $\langle lin_i, vis_i \rangle \models \varPhi$ if $\langle lin, vis \rangle \models \varPhi$. 
\setlength\emergencystretch{\hsize}
%until the abstract execution includes all operations.

The search algorithm tries all possible extensions from the current ``candidate execution" $\ang{lin_i, vis_i}$. 
When valid extensions cannot be obtained, the current candidate is discarded and the search algorithm backtracks to another candidate execution.
%An abstract execution $\langle lin_i, vis_i \rangle$ can be extended with different choices of operations, and obtains a series of abstract execution $\left\{ \langle lin_{i+1}', vis_{i+1}' \rangle, \langle lin_{i+1}'', vis_{i+1}'' \rangle, \ldots \right\}$ as candidates. 
%We can select one of them as the extension of $\langle lin_i, vis_i \rangle$. 
When we finally extend the prefix to a whole abstract execution containing all the operations in the data type access trace, we successfully get the certificate abstract execution, and the search algorithm returns \textsf{TRUE}.
If no certificate execution can be obtained after trying all possible candidates, the search algorithm returns \textsf{FALSE}.


%----------------------------------------
\subsubsection{The Refactored Non-recursive Search Skeleton} \label{SubSubSec: Revised-VS}

The main improvement made to the recursive search algorithm is that we refactor it to a non-recursive algorithm skeleton. 
This means that, the algorithm skeleton itself maintains a double-ended queue (\textit{deque} in short) to store the intermediate search states $\ang{lin_i, vis_i}$ at runtime.
%To enable flexible optimization, we revise the original recursive search.
%The key in the refactorization is to use a stack to explicitly maintain the intermediate state of the search at runtime.
The explicit maintenance of intermediate search states greatly facilitates further pruning of unnecessary searches.

The non-recursive \vs algorithm searches abstract executions through phases, as shown in Fig.~\ref{F: Tree}. 
In each phase, it extends $\ang{lin_i, vis_i}$ to $\ang{lin_{i+1}, vis_{i+1}}$. 
There are two steps in each phase. 
In the ``ar step", we add one operation to $lin_i$ and obtain $lin_{i+1}$. 
In the ``vis step", we extend $vis_i$ to $vis_{i+1}$ by adding visibility relations concerning the newly added operation. 
%--
\begin{figure}[tb]
    \includegraphics[width=\linewidth]{figures/tree.pdf}
    \centering
    \caption{Search of the certificate execution.}
    \label{F: Tree}
\end{figure}


As shown in Fig.~\ref{F: Tree}, the algorithm has already constructed a certificate abstract execution $\ang{lin_2, vis_2}$ that contains operations \textit{add}(1) and \textit{add}(2). Then the algotirhm starts phase 3. 
In the ar step, the algorithm first appends operation \textit{size}() to the $lin_2$ and obatins $lin_3$. 
In this example, we require each operation be visible to operations within the same session. 
So the operation \textit{size}() can return 1 if $add(1) \stackrel{vis}{\rightarrow} size()$, or return 2 if $\{add(1), add(2)\} \stackrel{vis}{\rightarrow} size()$. 
But neither of these two visibility relations bring the required return value $size \Rightarrow 0$. 
Thus the algorithm backtracks for other candidates.

Then we append operation \textit{remove}(2) to the $lin_2$. We can construct a certificate abstract execution $\ang{lin_3, vis_3}$ and finish phase 3. 
Then we proceed to phase 4, and the algorithm appends the last operation $size\Rightarrow0$ to the linearization. 
%
There are four possible cases of visibility extension concerning the newly added operation $size\Rightarrow0$: 
$\left\{ add(2) \right\}\stackrel{vis}{\rightarrow} size()\Rightarrow 0$, 
$\left\{ add(1), add(2) \right\}\stackrel{vis}{\rightarrow} size()\Rightarrow 0$,
$\left\{ add(2), remove(2) \right\}\stackrel{vis}{\rightarrow} size() \Rightarrow 0$, 
and $\left\{\textit{add(1)}, \textit{add(2)}, \textit{remove}(2)\right\}\stackrel{vis}{\rightarrow}\textit{size}()$.
%
We only show two of the four possible cases in Fig.~\ref{F: Tree}, due to the limit of space. 
%
The operation \textit{size}() returns 0 only if $\{add(2), remove(2)\} \stackrel{vis}{\rightarrow} size()$. %, which means the operation \textit{size}() ignore the effect of the operation \textit{add}(1). 
Finally, we find a certificate abstract execution, and prove that the history satisfies the \textit{basic} consistency level. 


Upon initialization, we build a \textit{search state deque} with the initial search state $\ang{lin_0, vis_0}$. State $\ang{lin_0, vis_0}$ contains no operation and has an empty visibility relation. 
During the search process, we keep polling search states from the head of the deque.
The newly popped search state is verified by the method \textsf{isValidAbstractExecution} ({Line 6 in Algorithm \ref{A: VS}}). This method basically checks whether the return values of all query operations in the current search state are allowed by the sequential semantics \textit{Impl} of the data type.
Invalid search states are discarded and valid ones are extended as follows. %We throw invalidated \textit{search states} away and extend validated \textit{search states}. 

For a given valid search state $\ang{lin_i, vis_i}$, we first extend the linearization by \textsf{linExtend} (Line 10 in Algorithm \ref{A: VS}), and get a set of new search states:
$$newLin = \left\{ \ang{lin_{i+1}^1, vis_i}, 
\ang{lin_{i+1}^2, vis_i}, \ldots, \ang{lin_{i+1}^p, vis_i} \right\}.$$

\noindent Then we extend visibility relations according to the newly added operation.
%extend each \textit{search state} in \textit{newLins} for visibility. 
Each newly-extended \textit{search state} $\ang{lin_{i+1}^{r}, vis_i}$ will be extended to a set of \textit{search states}:
%--
\begin{eqnarray*}
    newVis_r &=& \{ \ang{lin_{i+1}^{r}, vis_{i+1}^1}, \ang{lin_{i+1}^{r}, vis_{i+1}^2}, \ldots, \\
    &\;& \ang{lin_{i+1}^{r}, vis_{i+1}^{q}} \}
\end{eqnarray*}


\noindent Each search state in $\bigcup_{i=1}^{p} newVis_i$ is a possible extension of $\ang{lin_i, vis_i}$.We push all these candidate states into the head of the deque. 
In the next step, the search algorithm will get a candidate from the head of the deque and repeat this extension process. 
Once the search state cannot be extended any more, the algorithm will backtrack by polling older candidates from the head of the deque. 

The {\vs} algorithm returns \textsf{TRUE} if it obtains a certificate abstract execution.
The algorithm returns \textsf{FALSE} if it runs out of candidates but still cannot obtain any certificate execution.
The pseudocode of the \vs algorithm skeleton is listed in Algorithm \ref{A: VS}.

%--
\begin{algorithm}[tb]
    \caption{The \vs Algorithm Skeleton}
    \label{A: VS}
    \KwIn{history $\mathcal{H}$, 
        data type implementation \textit{Impl}, 
        consistency model $\Phi$}
    \KwOut{whether history $\mathcal{H}$ satisfies the given consistency model $\Phi$}
    \textit{deque} $\leftarrow$ \{\ \}\\
    \textit{initState} $\leftarrow$ $\ang{\emptyset, \emptyset}$\\
    \textit{deque}.\textsf{push}(\textit{initState})\\
    \While{$\lnot$deque.\textnormal{\textsf{isEmpty}( )}}{
        \textit{state} $\leftarrow$ \textit{deque}.\textsf{pollHead}( )\\
        \If{\textnormal{\textsf{isValidAbstractExecution}(}Impl, state\textnormal{)}}{
            \If{state\textnormal{.\textsf{isComplete}( )}}{
                \Return{\textnormal{\textbf{true}}}
            }
            \textit{newLin} $\leftarrow$ \textit{state}.\textsf{linExtend}($\mathcal{H}$)\\
            \ForEach{\textit{newLinState} $\in$ \textit{newLin}}{
                \textit{newVis} $\leftarrow$ \textit{newLinState}.\textsf{visExtend}($\Phi$)\\
                \text{$\langle$search space pruning plugged here$\rangle$}\\
                \textit{deque}.\textsf{pushHeadAll}(\textit{newVis})\\
            }
        }
    }
    \Return{\textnormal{\textbf{false}}}
\end{algorithm}


%---------------------------------------
\subsection{Pruning of the Search Space}

The key to circumventing the NP-hardness obstacle of abstract execution search is to leverage the semantic knowledge of the data type under search and prune the search space. 
%We prune the search space to reduce the cost for searching valid abstract executions.
Thus, we inspect the data type access trace and automatically extract \textit{pruning predicates}, which can be plugged into the \vs algorithm skeleton (Algorithm \ref{A: VS}). 
For each candidate abstract execution, the search algorithm checks the pruning predicates. 
Once any pruning predicate is detected \textsf{FALSE}, the candidate abstract execution is directly discarded.
We will prove that the pruning process is ``safe", in the sense that the pruning process never discards any candidate abstract execution which can be extended to a certificate abstract execution.

In this section, we first present the basic rationale of the pruning algorithm with three illustrative examples.
Then we present the design and correctness proof of the pruning algorithm.

%--------------------
\subsubsection{Rationale of Pruning}

The search algorithm enumerates every valid abstract execution in a brute-force way.
The insight behind our pruning scheme is that, for a  given data element in a container type, the update and query operations concerning this element cannot be linearized in an arbitrary way. Moreover, the visibility relations among can only have limited patterns.

For example, for each read operation \textit{r}, there exists a unique write operation \textit{w}. 
The operation \textit{w} must happen before \textit{r}. 
The rule mentioned above can be formally defined as the write-to order \cite{Wei16}. 
%
However, the \vs algorithm is ignorant of this type of knowledge concerning one specific data element, and enumerates all abstract executions it thinks that is possible.
Thus, we can extract this type of knowledge and express it as pruning predicates. 
%The predicates can be plugged into the \vs algorithm skeleton and prune the search space. %reduce the search cost.
We will use these pruning predicates before adding new search states into the deque ({Line 13 in Algorithm \ref{A: VS}}). 

Based on the observation above, we introduce the notion of \textit{query cluster}. 
All operations in the query cluster are associated with the same data element.
The query cluster contains exactly one query operation, which is denoted the \textit{dictated query}. The query cluster contains one or more update operations, which are denoted the \textit{dictating updates}. The dictating updates are those update operations which can potentially affect the return value of the dictated query. 

We consider two situations in extraction of the pruning predicates. One situation is that the update operations are the necessary and sufficient condition for the result of a query operation. For example, whether the set contains the element $x$ is determined by the arbitration and visibility of all $add$ and $remove$ operations associated with element $x$. 
The other situation is that the update operations are only the necessary condition for the result of a query operation. For example, $get\_max$ returns that the maximum element of the priority queue is $x$ with value $v$. All update operations associated with element $x$ only guarantee that there exists an element $x$ with value $v$ in the priority queue at that point.
But only these update operations cannot decide the return value of $get\_max()$.
Fortunately, the necessary condition is enough to ensure the safety of the pruning algorithm. 
%
In extraction of the pruning predicates, we do not consider operations which correspond to multiple data elements, e.g., the $isEmpty()$ operation, which returns whether the data container is empty.

%like this, and do not take operations like $isEmpty()$ into account as they do not refer to a specific element. 

%\mybreak

%\slt{query被几个update完全决定}


% >>>>>具体的单元素操作的例子
%
%For example, an operation \textit{contains}(\textit{z}) is related to the its argument, the element \textit{z}, 
%and an operation \textit{get\_max}()$\Rightarrow$(\textit{x; v}) is related to its return value. 
%
%Update operations involved in the related element potentially determine the return value of the query operation. 
%
%The return value of operation \textit{contains}(\textit{z}) is totally decided by operation \textit{add} and \textit{remove} on element \textit{z}. 
%
%Similarly, operation \textit{get\_pri}(\textit{e}) is totally decided by operation \textit{insert}, \textit{remove}, and \textit{inc} on element \textit{e}. 
%
%Different from \textit{contains}() and \textit{get\_pri}(), operation \textit{get\_max}()$\Rightarrow$(\textit{x;v}) is not decided by update operation on element \textit{x}. 
%Because we need to assure that there does not exist any other element whose \textit{priority} is bigger than \textit{v}, 
%besides the necessary condition that there exists an element in the priority queue whose \textit{id} is \textit{x} and \textit{priority} is \textit{v}. 
%However, the existence of the element (\textit{x;v}) is totally decided by updates on element \text{x}. 
%So due to the the necessary condition, we say that operation \textit{get\_max}()$\Rightarrow$(\textit{x;v}) is partly decided by operation \textit{insert}, \textit{remove}, and \textit{inc} on element \textit{x}. 
%
% >>>>>


We will use two data types \textit{set} and \textit{priority queue} as illustrative examples. %for the extraction of pruning predicates.
The set is a container of elements, in which each element is identified by its unique \textit{id}. 
The following primitives are involved in our examples: 
%--
\begin{itemize}
    \item $add(e)$ : add element $e$. 
    \item $remove(e)$ : remove element $e$. 
    \item $contains(e)$ : return \textsf{TRUE} if $e$ is in the set.
    % \item $isEmpty()$ : return \textsf{TRUE} if the set is empty. 
\end{itemize}

\noindent The priority queue is a container of elements of the form $e = (id, priority)$.
The following primitives are involved in the examples: 
%--
\begin{itemize}
    \item $insert(e, x)$ : enqueue element $e$ with initial priority $x$. 
    % \item $remove(e)$ : remove the element \textit{e}. 
    \item $inc(e, \delta)$ : increase the priority of element $e$ by $\delta$ (may be negative). 
    \item $get\_pri(e)$ : return the priority value of $e$.
    \item $get\_max()$ : return the \textit{id} and \textit{priority} of the element with the highest priority. 
    % \item $isEmpty()$ : return \textsf{TRUE} if the priority queue is empty. 
\end{itemize}

% 之前的版本侧重于讲我们如何利用cluster之间的locality去进行剪枝
% 新增的部分主要是说明为什么需要有template和extraction, 因为 
%   1. data type的语义变复杂了, 不是简单的shared variables, 读写之间的因果链条不再是直接的了. 很难人工为每一个data type定义出write-to order那样的规则
%   2. 引入vis之后一个操作可以忽略之前的操作了, 变得更加烧脑, 人定规则可能会遗漏case
% 所以需要template和extraction保证不管什么data type都能剪, 提取的剪枝谓词肯定safe

%\color{blue}
%It becomes difficult to seek out explicit rules like write-to order to extract pruning predicates, when we check data types with enriched semantics. For example, we can add or remove an element in the data type set. We can even increase and decrease the priority of an element. All these rich semantics of data types make the cause and effect between query operation and update operation are unclear. 
%Visibility relations being introduced into consistency specification makes things much more complicated. because an operation may ignore the effects of other operations. Pruning predicates formulated by human are hardly perfectly safe. 
%
%We want to extract pruning predicates automatically, and make sure that they are correct. In this context we define some templates which applies to various data types, and design a suite of algorithms that extract correct pruning predicates. 
%\color{black}


The pruning predicate is obtained by inspecting the query cluster pertaining to one specific data element.
There can be two types of pruning predicates. 
The first type is simpler, which only considers the arbitration relation between operations, while the second type considers both the arbitration and the visibility relations.

%\mybreak

By in-depth inspection of the data type access trace and manual exploration of the brute-force checking process, we come up with three predicate templates, i.e. patterns of pruning predicates we want to extract.
The first predicate template focuses on the arbitration relation. It aims to find that two operations always have the arbitration relation, no matter how you construct the linearization of operations. Specifically, $\tarb$ states that operation $x$ must be arbitrated before operation $y$ in every search state $\ang{lin, vis}$:
%--
\begin{eqnarray*}
    \tarb(x, y) \mydef \forall \ang{lin, vis}: (x,y) \in lin
\end{eqnarray*}

\noindent To extract pruning predicates following the template $\tarb$, we enumerate all valid abstract executions of the subhistory consisting of all operations in one query cluster.

For example, assume that there is a subhistory with two client sessions, as shown in Fig.~\ref{F: Template}.
One session has operation $insert(x,5)$, followed by $inc(x,1)$.
The second session has one single operation $get\_pri(x) \Rightarrow 6$.
For ease of illustration, we simply assume that there are no other operations on $x$ in the whole trace. 
%
It is evident that the return value of $get\_pri(x)$ can be 6 only if it is linearized after $inc(x,1)$.
All valid abstract executions of this query cluster must have this arbitration order $inc(x,1)  \stackrel{ar}{\rightarrow} get\_pri(x) \Rightarrow 6$.
This fact must also hold for all candidate abstract executions the \vs algorithm constructs. Thus it can be extracted as a pruning predicate and plugged into the \vs algorithm skeleton to avoid unnecessary searches.

%The second and the third predicate templates are 
There are two more predicate templates 
of the second type, which concern both the arbitration and the visibility relations. 
As for the $\tvis$ example in Fig.~\ref{F: Template}, if the arbitration relations among operations have been decided, we can infer that there must be the visibility relation between $remove(z)$ and $contains(z) \Rightarrow \textsf{FALSE}$. Otherwise, the semantics of the set type are violated.
The $\tnotvis$ template is the dual of $\tvis$. If the return value of $contain(z)$ is \textsf{TRUE}, there should be no visibility relation between $remove(z)$ and $contain(z)$.

%According to *rulearb, we find a filter that $(ins, inc) \in lin$. In running the \vs checking algorithm, whenever this pruning predicate is false, the candidate abstract execution is discarded.

%Therefore, whenever the algorithm constructs an abstract execution which \textit{inc}(\textit{x},1) is linearized before \textit{insert}(\textit{x},5), 
%we prune this search state as the current abstract execution cannot be extended to a complete one. 

%The pair of \textit{insert}(\textit{x},5) and \textit{inc}(\textit{x},1) is a fact for $\mathcal{P}_{A}(x, y)$. 

%Moreover, it is reasonable to infer that \textit{insert}(\textit{x},5) and \textit{inc}(\textit{x},1) must be linearized before \textit{get\_pri}(\textit{x})$\Rightarrow$6. 

%\slt{Fig2要换成我们黑板上讨论的例子，不然文字读起来，读者易误解}

%--
\begin{figure}[tb]
    \includegraphics[width=\linewidth]{figures/rule.pdf}
    \centering
    \caption{Examples of three predicate templates.}
    \label{F: Template}
\end{figure}

%\slt{图里的true，false要改字体，与正文统一。\\
%    \indent \indent 用not-vis，而不是non-vis。\\
%    \indent \indent rulea，ruleb要改，要是数学不好写，可以写the arb template, the vis template, the not-vis template之类的。}

Generalizing the examples above, $\tvis$ states that certain arbitration relations and certain visibility relation always co-exist:
%--
\begin{eqnarray*}
    \tvis(S_{lin}, x, y) &\mydef& \forall \ang{lin, vis} : \\
    &\ & S_{lin} \subseteq lin \rightarrow (x,y) \in vis
\end{eqnarray*}

\noindent where $S_{lin}$ is a subset of the arbitration relation (a subset of operation pairs having the arbitration relation).
The dual template $\tnotvis$ states that if there are certain arbitration relations, certain visibility relation cannot occur:
%--
\begin{eqnarray*}
    \tnotvis(S_{lin}, x, y) &\mydef& \forall \ang{lin, vis} : \\
    &\ & S_{lin} \subseteq lin \rightarrow (x,y) \not \in vis
\end{eqnarray*}

\noindent We scan all valid abstract executions of the query cluster and check whether there are operation patterns that can be matched by the two predicate templates $\tvis$ and $\tnotvis$.

%To solve these problems, we develop a predicate extraction method. 

%We focus on subhistories consisting of multiple updates and one query all pertaining to one data element.

%We enumerate all possible abstract executions of the subhistory. 

%We match the predicate template over all possible executions, to see whether there are pruning predicates.

%We present the details below.

%For every abstract execution, we check whether there are predicates predicate template 

%This method enumerates all complete abstract executions of a small cluster, and extracts necessary conditions from all complete abstract executions to generate predicates. 



%----------------------------------------
\subsubsection{Extraction of Pruning Predicates}

Extraction of the pruning predicates is similar to the ``string matching" process. 
The predicate template is analogous to the pattern string to be searched, while all valid abstract executions of a query cluster as a whole is analogous to the text string being scanned.
Note that we are interested in predicates which are \textsf{TRUE} for all abstract executions of a given query cluster.
The query cluster can simply be treated like normal traces of data type access, and we can directly use the brute-force \vs algorithm (Algorithm \ref{A: VS}) to search all valid abstract executions. 
We extract concrete pruning predicates following the templates $\tarb$, $\tvis$ and $\tnotvis$ from the abstract executions. 
%
We assume that the size of the query cluster is bounded and the extraction of predicates takes constant time.
We validate our assumption and study the cost of predicate extraction in Section \ref{SubSec: Eval-Results}.

For an abstract execution $\pi_t$ = $\ang{{lin}^t, {vis}^t}$, we define that $lin(\pi_t)$ = $lin^t$, $vis(\pi_t)$ = $vis^t$. 
We define the not-visible relation of an abstract execution $\pi_t$ by $notvis(\pi_t)$ = $\{(x,y) \mid (x,y) \in lin^t \land (x,y) \notin vis^t\}$. 
%
It is straightforward to extract pruning predicates of template $\tarb$ from valid abstract executions. 
We just need to intersect every linearization of valid abstract executions, as shown in Algorithm \ref{A: T-ARB}.
Specifically, linearization of an abstract execution $\pi$ is a total order of operations. For each pair of operations, $(x,y) \in lin(\pi)$ means that operation $x$ is arbitrated before operation $y$ in abstract execution $\pi$. 
The intersection of all linearization is the arbitration order that every valid abstract execution must obey. 
Each concrete operation pair $(op1, op2)$ in the final intersection of linearizations can generate a concrete pruning predicate $\tarb(op1, op2)$. 

%--
\begin{algorithm}[tb]
    \caption{Extraction of Pruning Predicates for $\tarb$}
    \label{A: T-ARB}
    
    \KwIn{a set of abstract executions $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
    \KwOut{a set of pruning predicates of $\tarb$}
    
    $S_{\text{arb}}$ $\leftarrow$ $U$\quad\CommentSty{/* U is the complete relation which contains all possible pairs of operations. */}\\
    \ForEach{$\pi \in \mathcal{A}$}{
        $S_{\text{arb}}$ $\leftarrow$ $S_{\text{arb}} \bigcap lin(\pi)$
    }
    
    \ForEach{pair $(x,y) \in S_{\text{arb}}$}{
        \textbf{yield} $\tarb(x,y)$
    }
\end{algorithm}


To extract pruning predicates following the template $\tvis$, we union the visibility relation of all valid abstract executions: $\mathcal{V} = \bigcup_{t=1}^{m} vis(\pi_t)$. 
For each pair $(x,y) \in \mathcal{V}$, it means that operation $x$ is visible to operation $y$ in some valid abstract execution. 
Then we try to generate a concrete predicate of template $\tvis$ for every pair $(x,y) \in \mathcal{V}$. 

We first intersect the linerarization of valid abstract executions that contains the pair $(x,y)$. 
Any valid abstract execution whose visibility relation contains pair $(x,y)$ must obey the arbitration order in the intersection $S_{\text{arb}}$. 

Next we need to ensure that there exists no counterexample for this concrete predicate. %, or this concrete predicate is not a necessary condition for the subhistory. 
Because we extract this concrete predicate only from valid abstract executions which contain pair $(x,y)$ in their visibility relation. 
We must check whether it is a necessary condition for those valid abstract executions which do not contain pair $(x,y)$ in their visibility relation.
We discard this concrete predicate, if there is a valid abstract execution whose visibility relation does not contain pair $(x,y)$ but it obeys all arbitration order in the intersection $S_{\text{arb}}$.
The pseudocode of the extraction algorithm for $\tvis$ are listed in Algorithm \ref{A: T-VIS}.

%\slt{文字解释一下：为什么这个二次检测是必须的，不能遗漏。}

%--
\begin{algorithm}[tb]
    \caption{Extraction of Pruning Predicates for $\tvis$}
    \label{A: T-VIS}
    
    \KwIn{a set of abstract executions $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
    \KwOut{a set of pruning predicates of $\tvis$}
    
    $S_{vis}$ $\leftarrow$ $\bigcup_{t=1}^{m} vis(\pi_t)$\\
    \ForEach{pair $(x,y) \in S_{vis}$}{
        $S_{arb}$ $\leftarrow$ $U$\\
        \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \in vis(\pi)$}{
            $S_{arb}$ $\leftarrow$ $S_{arb} \bigcap lin(\pi)$
        }
        
        \textit{review} $\leftarrow$ \textsf{TRUE}\\
        \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \notin vis(\pi)$}{
            \If{$S_{arb} \subseteq lin(\pi)$}{
                \textit{review} $\leftarrow$ \textsf{FALSE}\\
                \textbf{break}
            }
        }
        \If{\textit{review} \textnormal{is} \textnormal{\textsf{TRUE}}}{
            \textbf{yield} $\tvis(S_{{arb}}, x, y)$
        } 
    }
\end{algorithm}

Since the template $\tnotvis$ is just the dual of $\tvis$, the extraction of concrete predicates for $\tnotvis$ is similar to the extraction for $\tvis$. 
We just replace the visibility relation in the $\tvis$ extraction algorithm with the not-visibility relation. 
The pseudocode of the extraction algorithm for $\tnotvis$ are listed in Algorithm \ref{A: T-NOT-VIS}.

%--
\begin{algorithm}[tb]
    \caption{Extraction of Pruning Predicates for $\tnotvis$}
    \label{A: T-NOT-VIS}
    
    \KwIn{a set of abstract executions $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
    \KwOut{a set of pruning predicates of $\tnotvis$}
    
    $S_{notvis}$ $\leftarrow$ $\bigcup_{i=1}^{m} notvis(\pi_i)$\\
    \ForEach{pair $(x,y) \in S_{notvis}$}{
        %$S_{arb}$ $\leftarrow$ $\mathcal{U}(\mathcal{H}_q)$\\
        $S_{arb}$ $\leftarrow$ $U$\\
        \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \in notvis(\pi)$}{
            $S_{arb}$ $\leftarrow$ $S_{arb} \bigcap lin(\pi)$
        }
        
        \textit{review} $\leftarrow$ \textsf{TRUE}\\
        \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \notin notvis(\pi)$}{
            \If{$S_{arb} \subseteq lin(\pi)$}{
                \textit{review} $\leftarrow$ \textsf{FALSE}\\
                \textbf{break}
            }
        }
        \If{\textit{review} \textnormal{is} \textnormal{\textsf{TRUE}}}{
            \textbf{yield} $\tnotvis(S_{arb}, x, y)$
        } 
    }
\end{algorithm}


%----------------------------------------
\subsubsection{Correctness of Pruning}

We now prove that the pruning is safe, i.e., no certificate abstract execution will be falsely discarded by the pruning predicates. 
Here we present a sketch of the proof. 

Given a history $\mathcal{H}$ and a consistency model $\Phi$, if $\mathcal{H} \not\models \Phi$, it means that there exists no certificate abstract execution for $\Phi$. 
So the pruning must be safe. 
Therefore in the rest of the proof, we focus on the case in which history $\mathcal{H}$ has a certificate abstract execution satisfying the consistency model $\Phi$. 

The \vs algorithm prunes abstract executions during the construction of a candidate execution at runtime. 
So we need to prove that no candidate execution, which can be extended to a certificate abstract execution in the future, is pruned.
%
If an abstract execution violates a pruning predicate, all of its extensions violate the pruning predicate too. 
Hence, we only need to prove that there does not exist a certificate abstract execution which violates the pruning predicate. 

We assume for contradiction that there exists a certificate abstract execution $\pi$ of history $\mathcal{H}$ which violates a pruning predicate $P$.
The pruning predicate $P$ is extracted from some query cluster in history $\mathcal{H}$. 
We project the abstract execution $\pi$ on the query cluster and get the sub-execution $\pi'$. The sub-execution $\pi'$ is an abstract execution of the query cluster from which the predicate $P$ is extracted.
%
The arbitration and visibility relations among \textit{dictating updates} and \textit{dictated query} is reserved after projection. 
So $\pi'$ still violates the predicate $P$. 
Moreover, the \textit{dictated query} of the query cluster has the same return value after the projection. 

Since $\pi$ is a certificate abstract execution, each operation in $\pi$ can see all the operations it is required to see by the visibility constraint of $\Phi$. In other words, each operation in $\pi$ does not ignore any operation it is required to see. 
Compared to $\pi$, each operation in $\pi'$ only omits those operations discarded in the projection to a query cluster. 
It means that each operation in $\pi'$ does not ignore any operation it is required to see. 
%
% Note that a query cluster contains one dictated query, together with all dictating updates which can potentially affect this dictated query. 
Thus the projection $\pi'$ still satisfies the visibility constraint. This means that the projection $\pi'$ still satisfies the consistency model $\Phi$. 

We can also prove that the abstract execution $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$ in a formal way. 

As we construct the abstract execution by operation, the visibility relation of the first $k-1$ operations is fixed when we choose the visibility of the $k$-th operation $o_k$. 
We define a set $\mathcal{V}_k$ consisting of operations that is visible to the $k$-th operation. 
We extend the abstract execution $\ang{lin_{k-1}, vis_{k-1}}$ to $\ang{lin_{k}, vis_{k}}$ by adding 
$\mathcal{V}_k$ to $vis_{k-1}$ and adding $o_k$ to the end of $lin_{k}$. 

We define a function $\mathcal{G}$ mapping a tuple $(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k)$ to a set $\mathcal{M}$. 
The set $\mathcal{M}$ is the visibility relation that describles what $o_k$ must see according to the visibility constraint of the consistency model. If $\mathcal{M} \subseteq \mathcal{V}_k$, $\mathcal{V}_k$ is a legal visibility extension for the consistency model $\Phi$. 
For example, we list some function $\mathcal{G}$ according to the visibility predicates in \ref{SubSec: Vis-Relax}, 
\begin{itemize}
    \item $\mathcal{G}_{weak}(\_, \_, o_k) = \emptyset$, which has no constraint for visibility. 
    \item $\mathcal{G}_{basic}(\_, \_, o_k) = \{(x, o_k)\ \vert\ \forall x: (x, o_k) \in so \}$, which means $o_k$ must see all the operations that happens before it according to the session order. 
    \item $\mathcal{G}_{monotonic}(\ang{lin_{k-1}, vis_{k-1}}, \_, o_k) = \{(x, o_k)\ \vert\ \forall x \exists y : (y, o_k) \in so \land (x, y) \in vis_{k-1}\}$, which means $o_k$ must see the operations that its predecessors see. For the sake of simplicity, each operation is visible to itself. 
    \item $\mathcal{G}_{causal}(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k) =  \{(x, o_k)\ \vert\ \forall x :(x, o_k) \in (vis_{k-1} \bigcup \mathcal{V}_k)^{+}\} \bigcup \mathcal{G}_{basic}(\_, \_, o_k)$, which means $o_k$ must see operations visible to those $o_k$ sees, and the visibility is a transitive closure. 
    \item $\mathcal{G}_{complete}(\ang{lin_{k-1}, vis_{k-1}}, \_, o_k) = \{(x, o_k)\ \vert\ \forall x: (x, \_) or (\_, x) \in lin_{k-1} \}$
\end{itemize}

The set $\mathcal{R}$ contains relation pairs in the abstract execution $\pi$ but not in the projection $\pi$. 
$\mathcal{V}_{k'}$ is the visibility relation that describles operations visible to the $k$-th operation in $\pi$, i.e. the $k'$-th operation in $\pi'$ after projection.  
All relation pairs in $\mathcal{R}$ are removed from $\mathcal{V}_k$ after projection, so $\mathcal{V}_{k'} = \mathcal{V}_k \setminus \mathcal{R}$. 
Also operations in $\mathcal{R}$ are removed from $\mathcal{M}$ after projection. Considering the transitivity, some operations cannot see another operation via removed operations in $\mathcal{R}$ any more, 
\begin{equation*}
    \begin{split}
        &\mathcal{M}' = \mathcal{G}(\ang{lin_{k'-1}, vis_{k'-1}}, \mathcal{V}_{k'}, o_{k'}) \\
        &\subseteq \mathcal{G}(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k) \setminus \mathcal{R} = \mathcal{M} \setminus \mathcal{R}.
    \end{split}
\end{equation*} 

As the original abstract execution $\pi$ satisfies the visibility constraint of the consistency model $\Phi$, we can conclude that
$\mathcal{M} \subseteq \mathcal{V}_k$ and further deduce that $\mathcal{M} \setminus \mathcal{R} \subseteq \mathcal{V}_k \setminus \mathcal{R}$. 
Combining the transitivity of $\subseteq$, we can conclude that 
$\mathcal{M}' \subseteq \mathcal{V}_{k'}$. 
Therefore, the projection $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 

Because the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
Therefore, the pruning in \vs is safe, in the sense that the candidate abstract executions discarded can never be extended to a valid certificate one. 



%----------------------------------------
%\subsubsection{Correctness of Pruning}
%
%We now prove that the pruning is safe, i.e., no certificate execution can be discarded by the pruning predicates. 
%Given a history $\mathcal{H}$ and a consistency model $\Phi$, if $\mathcal{H} \not\models \Phi$, it means that there exists no certificate abstract execution for $\Phi$. %, i.e., an abstract execution of history $\mathcal{H}$ that satisfies the requirement of $\Phi$. 
%So the pruning must be safe. 
%Therefore in the rest of the proof, we focus on the case in which history $\mathcal{H}$ has a certificate abstract execution satisfying the consistency model $\Phi$. 
%
%In fact, the \vs algorithm prunes abstract executions during the search at runtime. 
%So we need to prove that no candidate abstract execution, which can be extended to a certificate execution in the future, is pruned.
%%no constructing abstract execution which can be extended to a correct one is pruned by filter. 
%If an abstract execution violates a pruning predicate, all of its extensions violate the filter too. 
%Hence, we only need to prove that there does not exist a certificate execution which violates the pruning predicate. 
%
%% 证明剪枝正确性的方法一, 避开了繁琐的分类讨论, 引入新的概念函数G作为一个vis是否合法的判断依据
%% 然后简单地通过投影后必须看见的操作应该相应地减少, 通过集合 \subseteq 的传递关系去完成证明
%% 优点是证明看起来比较有理有据 不像分类讨论都是文字的叙述
%% 缺点是引入了新的符号 新的形式化语言
%
%\pur
%
%证明采用反证法。如果$\pi$是certificate，且被prune（违反P）。
%
%因为vis关系的某种单调性，$\pi$满足Phi，则$\pi'$不会xxx，只会单调xxx，$\pi'$必然满足Phi。
%
%所以$\pi'$也会满足P，因为xxx。
%
%所以$\pi'$同时满足P，且违背P，所以矛盾。
%
%细节见\ref{}。
%
%\bla


%--------------------------------------------------------------------------------
\subsection{Parallelization of \vs}

All legal search states of a history are organized as a tree, as shown in Fig.~\ref{F: Parallel}. 
Each search state is a node in the tree, and the root node is the empty abstract execution $\ang{lin_0, vis_0}$.
For a node $\ang{lin, vis}$ in the tree, search states which are possible extensions of $\ang{lin, vis}$ in the next phase are the children of $\ang{lin, vis}$. 
%Conversely, $\ang{lin, vis}$ is the parent of all search states which are possible growth of it in one phase. 
There may exist many candidate extensions in one phase, and different choices of extensions result in the search of different subtrees. %split into different branches of the tree. 

%--
\begin{figure}[tb]
    \includegraphics[width=0.9\linewidth]{figures/p_tree.pdf}
    \centering
    \caption{Parallel \vs}
    \label{F: Parallel}
\end{figure}


%\slt{因为是树所以可以无脑并行}

%The tree has a recursive structure. 
%A tree consists of a root, and zero or more subtrees $T_1, T_2, \ldots , T_k$, and the root of each subtree is the child node of root of the tree. 
Consistency checking with \vs is principally a depth-first search, aiming to find a search state which constructs a certificate abstract execution.
Therefore, there exists natural parallelization for the search. 
Subtrees do not share any nodes and are independent of each other. 
We can search the subtrees in parallel. 
If we find a certificate execution in any subtree, we terminate the search. %tasks in other subtrees and the history satisfies the consistency model. 
If no certificate executions could be found in any subtree, the history does not satisfy the consistency model. 

In preparation for the parallel search, the central coordinator runs the sequential \vs algorithm and generates a batch of search states. 
These search states are evenly allocated to different threads. Then each thread runs an instance of the sequential \vs algorithm.
Note that here we use the term ``thread" in a broad sense. The thread is more like an abstract worker. It can also be, for example, a virtual or physical machine.
%
As shown in the example in Fig.~\ref{F: Parallel}, we generate four search states (the root node of each subtree in the dashed box). 
Each of the four states is allocated to a worker thread. The four threads extend the search states in parallel and obtain four different subtrees (the colored subtrees in four dashed boxes).

Since the search cost for different subtrees may vary quite a lot, we further design a load balancing scheme for the coordinator.
Specifically, when a thread finishes its search task, it asks the coordinator for more tasks.
Meanwhile, the fully loaded threads periodically contact the coordinator to see whether there are idle threads which they can share their workloads with.
In this way, the working thread can allocate part of its own tasks to other threads via the coordinator.
Since the thread maintains its tasks as search states in the deque (see detailed design in Section \ref{SubSubSec: Revised-VS}), it simply transfers part of its workloads from the tail of its deque to other threads via the coordinator.

We let the working threads periodically contact the coordinator, instead of letting the coordinator interrupt the working threads.
This is mainly because interrupting a running thread usually imposes more overhead.
Based on the statistics from running \vs without load balancing, we let the working thread contact the coordinator every 1000 search states in our experiments in the following Section \ref{Sec: Exp}.


==> ViSearch_complete_version/maintext_backup/abs.tex <==
%--
\begin{abstract}

    Large-scale replicated data type stores often resort to eventual consistency to guarantee low latency and high availability. It is widely accepted that programming over eventually consistent data stores is challenging, since arbitrary divergence among replicas is allowed. Moreover, pragmatic protocols actually achieve consistency guarantees stronger than eventual consistency, which can be and need to be utilized to facilitate the reasoning of and programming over replicated data types.
    Toward the challenges above, we propose the \vs framework for precise measurement of eventual consistency semantics.
    \vs employs the visibility-arbitration specification methodology in concurrent programming, which extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happen-before and linearization relations. 
    The consistency measurement using \vs is NP-hard in general. To enable practical and efficient consistency measurement in replicated data type stores, the \vs framework refactors the existing brute-force checking algorithm to a generic algorithm skeleton, which further enables efficient pruning of the search space and effective parallelization.
    We employ the \vs framework for consistency measurement in two replicated data type stores Riak and CRDT-Redis. The experimental evaluation shows the usefulness and cost-effectiveness of consistency measurement based on the \vs framework in realistic scenarios.    

\end{abstract}

==> ViSearch_complete_version/maintext_backup/concl.tex <==
%--
\section{Conclusion and Future Work} \label{Sec: Concl}

In this work, we develop the \vs framework for consistency measurement of replicated data type stores. In our framework, different consistency levels are specified via the relaxation of the visibility relations among operations.
The measurement of data consistency is based on the \vs algorithm skeleton, which enables efficient pruning of the search space and effective parallelization.
We employ the \vs framework for consistency measurement in two replicated data type stores Riak and CRDT-Redis. The experimental evaluation shows the usefulness and cost-effectiveness of consistency measurement based on the \vs framework in realistic scenarios.

In our future work, we will investigate how to propose more predicate templates and extract efficient pruning predicates to further reduce the consistency measurement cost. 
Moreover, efficient heuristics can be employed to reduce the search cost.
%We also need to explore load balancing techniques for the parallel \vs algorithm.
Besides improvements on the \vs framework itself, we will conduct more case studies of realistic replicated data type stores and investigate whether knowledge of the specific data type store can be effectively utilized to reduce the consistency measurement cost using \textsc{ViSearch}.

==> ViSearch_complete_version/maintext_backup/exp.tex <==
%--
\section{Experimental Evaluation} \label{Sec: Exp}

\begin{tbm}
    In this section, we apply the \vs framework for consistency measurement in two realistic replicated data stores in order to answer two main questions. One is that whether the \vs framework can measure out the subtle difference between different replicated data types. 
    The other one is how efficient the \vs framework is. 
\end{tbm}

We first present our experiment setup and design. Then we discuss the evaluation results.

The implementation of the \vs framework, as well as implementations, configurations and experiment scripts over the two replicated data type stores are available on the github \footnote{https://github.com/ViSearch/ViSearch}.

%--------------------------------------------------------------------------------
\subsection{Experiment Setup}

\begin{tbm}
We employ \vs to measure consistency for Riak \cite{Riak} and CRDT-Redis \cite{CRDT-Redis}. 
Riak is a distributed NoSQL key-value database, which provides Riak-specific data types based on CRDTs. 
CRDT-Redis revises Redis, a popular in-memory data structure store with built-in replication, into a multi-master architecture and supports CRDT-based conflict resolution for concurrent updates on multiple master nodes. 

We choose data types for experiments from two perspectives. The first perspective is the semantics of data type, in other words the interface exposed to users. 
We select three widely-used containers, \textit{set}, \textit{map}, and \textit{priority queue}, which are are representative and cover a range of data type semantics. 
Among them, \textit{set} is supported by both Riak and CRDT-Redis. \textit{Map} is only supported by Riak while \textit{priority queue} is only supported by CRDT-Redis. 
Riak and CRDT-Redis also support other data types like register, counter, and hyperloglog, but we think register and counter have too simple semantics, and hyperloglog seems like a probability algorithm rather than a traditional data structure. 

However, different implementations of the same data structure vary from each other. For example, the JDK provides LinkedList and ArrayList which both implement List interface, but they have different performance. 
Similarly, distributed data storage provides replicated data types with the same interface but different implementations. 
The second perspective is the implementation of data type, including different configurations and different conflict resolutions. 

Riak exposes a parameter $r$ to the clients, which denotes how many replicas a query request must contact. Contacting more replicas before returning a query request reduces the data inconsistency but increases the query delay.
The two data types with different parameters $r$ $(r=1$ or $r=2$) are denoted \textit{Set-r1}, \textit{Set-r2}, \textit{Map-r1} and \textit{Map-r2} in our experiment. 
Each data type in CRDT-Redis is designed with different conflict-resolution strategies: add-win (\textit{A} in short), remove-win (\textit{R} in short), and the \rwf framework (\textit{F} in short) \cite{Zhang21}. 
Data types with different conflict-resolve strategies are denoted \textit{Set-A}, \textit{Set-R}, \textit{Set-F}, \textit{PQ-A}, \textit{PQ-R}, and \textit{PQ-F}. 
All of our experiments is conducted on these ten data types, which combines high-level semantics and concrete implementations up. 
\end{tbm}

%% We study two widely-used container types \textit{Riak-set} and \textit{Riak-map}. Riak exposes a parameter $r$ to the clients, which denotes how many replicas a query request must contact. Contacting more replicas before returning a query request reduces the data inconsistency but increases the query delay.
%To match application needs, Riak KV enables users to trade off between data consistency and availability by adjusting replication configuration. 
%There exists wide and varied replication parameters available in Riak KV, and we focus on the number of servers that must respond to a read request(denoted as \textit{r}), which is concerned with the conflict-resolve strategy of Riak-specific data types. 
%Users can archieve higher accuracy by choosing higher values for \textit{r}, while higher values will also entail degraded responsiveness. 
%% The two data types with different parameters $r$ $(r=1$ or $r=2$) are denoted \textit{Set-r1}, \textit{Set-r2}, \textit{Map-r1} and \textit{Map-r2} in our experiment. 

%We experiment on Riak-specific data types with parameter \textit{r}=1, and 2 (3 replicas in total), marked as \textit{Set-r1}, \textit{Set-r2}, \textit{Map-r1}, and \textit{Map-r2}. 



%% CRDT-Redis currently provides two container types \textit{Redis-set} and \textit{Redis-priority-queue} (\textit{Redis-PQ} in short).


We run both distributed data stores in the Alibaba Cloud Elastic Compute Service (ECS) \cite{Alibaba-Cloud}. Each ECS server has two Intel Xeon Platinum CPU (2.50GHz), 4GB RAM, 40GB ESSD and 1MB/s network bandwidth. We build a Riak cluster with 5 servers, and replicate data types on 3 servers in the cluster. The CRDT-Redis cluster consists of 3 servers, and data types are replicated on all 3 servers. Another ECS server is dedicated to running clients. 

The checking of data type access traces using \vs is conducted on one workstation with an Intel i9-9900X CPU (3.50GHz), with 10 cores and 20 threads, and 32GB RAM, running Ubuntu Desktop 16.04.6 LTS.

The basic workflow of consistency measurement using \vs is shown in Figure \ref{F: Exp}.
We first generate the workloads for each data type. The workload module basically tells the clients what queries to send to the data store and when to issue the queries. %???
%The clients send queries to the data store as instructed by the workload module and wait for the reply. 
The clients record both the query invocation info (e.g., API name and arguments) and the return values (e.g., the value returned by a query request and the ACK returned by an update request) for all queries issued.
All the info of data type access collected by the clients in one experiment form one trace or history of data type access. 
Multiple traces of data type access are imported into the \vs module and \vs tells us the consistency levels of the traces measured, e.g., Co (complete visibility) or M (monotonic visibility). Detailed definitions of the consistency levels can be found in Section \ref{SubSec: Vis-Relax}.

% 单个client收集的叫info
% 所有client一起访问一个type，收集的叫一个trace，或者一个history。
% 一个实验，多次收集traces或者说histories。
% 这里，等于是把trace和history当成同义词。

%--
\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/exp.jpg}
    \caption{\vs workflow.}
    \label{F: Exp}
\end{figure}


%\mybreak

%\slt{为了获得全面的trace，需要做的工作}


%--------------------------------------------------------------------------------
\subsection{Experiment Design}

The optimized trace checking using \vs (as detailed in Section \ref{Sec: VS}) still requires exponential time in the worst case. Thus we cannot directly apply \vs over CRDT access traces of arbitrary length. As inspired by the measurement in \cite{Emmi19}, we explore locality in consistency measurement over CRDT traces to circumvent the NP-hardness obstacle.

As for a CRDT, any replica can be modified without coordination with other replicas. Thus the replicas  may temporarily diverge. 
When all updates are delivered to the replicas, possibly in different orders, the replicas converge, as required by the definition of eventual consistency \cite{Shapiro11a}.
We call the period when the replicas diverge the \textit{divergence interval}. 

Our key observation for consistency measurement of real data type access traces is that, the consistency level of given trace is decided by the divergence intervals in the trace. Thus we only need to measure the divergence intervals in the trace, instead of measuring the whole trace of arbitrary length. The consistency level of the whole trace is decided by the divergence interval of the weakest consistency level.

We can estimate the divergence interval by monitoring the communication channel. According to the definition of eventual consistency, the replicas only diverge when the updates are still in transmission. 
We estimate the maximum extent of divergence by monitoring how large the number of updates in transmission can be, during the experiment.

We reproduce the experiments in our previous work on CRDT design based on CRDT-Redis \cite{Zhang21}.
We set 1000 checkpoints for the replicas in the experiments where there are about 100,000 operations in the workload and the number of operations per second is bounded by 3000.
We find that the number of operations in transmission is bounded by 15. %, when the throughput is bounded by 3000 operations per second. 
Therefore in our experiment, we set the size of the workload, i.e., the number of operations to be sent to the data type, to 15. We let the clients launch the operations as quickly as possible to produce the maximal divergence.
Note that the specific value of the divergence interval is not essential in our experiment. In different experiment scenarios, we can estimate the divergence interval in the same way. Generally speaking, the more the throughput of the data type store, the larger the divergence interval.

\begin{tbm}
To obtain comprehensive and typical data type access traces, we generate a wide range of workloads. 
To avoid any bias and human factor in the collection of traces, we fill workloads with randomly-generated methods with randomly-generated arguments. 
As discussed above, each workload contains about 15$\sim$17 operations and 3$\sim$5 client threads shares the operations in a workload. 

In detail, we randomly choose arguments of operations from a small space. 
The space is usually set as 0$\sim$5, which is no more than 1/3 of the workload size. 
This ensures that there exists many collisions with operations, i.e. conflict operations invoked at the same element, since we generate sufficient workloads and execute workloads sufficient times. 
In our workloads, about 60\% operations are \textit{update}, and about 40\% operations are \textit{query}. 
For example, there are 40\% \textit{add} operations, 20\% remove operations, 20\% \textit{contains}, and 20\% \textit{size} operations in workloads for data type \textit{set} in CRDT-Redis. 
\end{tbm}

%According to experience and others' work, most of inconsistent behaviours can be exposed by several operations across two or three threads. 
%As long as there are sufficient executions, we can catch all these inconsistent behaviours with high probability. 
%On the other hand, we have to restrict the size of a single program to avoid combinatorial explosion in consistency checking. 

%The arguments are generated from a certain range to ensure that there exists collisions with operations invoked on the same elements concurrently. 
%For example, in the experiment of set, we make the range of elements small so that there might be more \textit{add} and \textit{remove} invoked on the same elements concurrently. 

\begin{tbm}
Though we try to generate comprehensive and typical traces, the final result of the measurement is still an approximation of the consistency level but not a guarantee. 
Because our finite workloads cannot exhaust all possible executions of a replicated data type, unless we make a strict proof or do model checking on these data types. 

To ensure accuracy, we measure the consistency level of a certain data type by round. 
Every round we generate workloads randomly and obtain 100K data type access traces. 
According to our experience, 100K traces is large enough to construct all corner cases in the CRDT design and cover the various cases in the conflict resolution. 
Then the \vs framework measures the consistency level of each trace, and the weakest consistency level measured over all these 100K traces is the measurement result in this round. 
The final measurement result will be updated if the measurement result of the current round is weaker than it. 
We repeat above procedure, and terminate when at least 3 rounds have been finish and the final measurement result keeps unchanged in the last two consecutive rounds. 

We believe that our measurement over a sufficiently large number of workloads is a cost-effective and accurate enough approach to obtaining the precise consistency semantics of one replicated data type. 
\end{tbm}

% In our experiment, we randomly generate 400,000 workloads for each data type. According to our experience in testing CRDT implementations, the workload of 15 operations is sufficient for constructing all corner cases in the CRDT design, and 400,000 workloads are sufficient to cover the various cases in the conflict resolution \cite{Zhang21}. 
% The  weakest consistency level measured over all the workloads is approximately the actual consistency level the data type provides. 
% Since it is usually quite difficult to strictly prove the consistency level certain CRDT design guarantees, we believe that our measurement over a sufficiently large number of workloads is a cost-effective and accurate enough approach to obtaining the precise consistency semantics of one replicated data type.

Given the workloads generated above, the main objective of the experimental evaluation is to answer the following two questions:
%--
\begin{itemize}
    \item[Q1.] Are the measurement results useful, for the developers to understand the consistency semantics a CRDT design actually provides?

    \item[Q2.] Can the consistency measurement be efficiently conducted with reasonable testing budget?
\end{itemize}

\noindent We discuss the evaluation results below in light of these two questions.

%--------------------------------------------------------------------------------
\subsection{Evaluation Results}

Based on the evaluation results, we first discuss what the application developers and CRDT designers can obtain from our consistency measurement. Then we study the time cost for the measurement. We also study the checking cost saved by the two optimization we develop, i.e., the pruning of search space and the parallelization of the checking process.

%----------------------------------------
\subsubsection{Consistency Measurement Results}

\begin{tbm}
We measure the consistency levels of 10 replicated data types from two data type stores. 
Due to different configurations and conflict resolutions, these replicated data types satisfy different consistency levels with high probability. 
If \vs can measure the consistency level precisely, the measurement results should spread on different consistency levels. 
\end{tbm}

The measurement results are listed in Table. \ref{T: Result}. %, and each row is the experiment result of a replicated data type.
Each row of the table corresponds to one data type.
For each of the 6 consistency levels, we list the number of violations found by \textsc{ViSearch}.
The strongest consistency level with 0 violation (colored gray in the table) is the consistency level of the data type.
The '/' means that the checking is unnecessary and the violation must be zero, since there are no violations for stronger consistency levels.

We demonstrate the usefulness of the consistency measurement results from the perspective of the "cosistency-latency tradeoff", which is a refinement of the widely used CAP theorem \cite{Brewer12, Gilbert12} and the PACELC tradeoff \cite{Abadi12} in CRDT scenarios.
Different CRDT designs and implementations principally have the same data update delay, since the replica is updated locally at once and the updates are propagated asynchronously. The query delay is also principally the same if the query only contacts one replica. In some data stores like Riak, the client can choose to contact multiple replicas, sacrificing certain query delay and improving the consistency level of the query.
Thus, from the perspective of the consistency-latency tradeoff, it is the consistency semantics of the data type which capture all the differences in CRDT designs and implementations.

In light of the discussions above, we study whether the consistency measurement results can tell the CRDT designers and application developers the essential differences in different data types in our experiment.
%In each store, the data type can adopt different implementations with different conflict resolution strategies. The data type can also have different configuration, e.g., $Set\text{-}r1$ and $Set\text{-}r2$. 
%
%The eventual consistency semantics cannot show the differences among different implementations and configurations. 
%Our consistency measurement using \vs show the different consistency semantics provided by different implementations and configurations.
%
Specifically, the consistency measurement of CRDT-Redis data types demonstrates the different consistency semantics resulting from different conflict resolution strategies.
%that Redis replicated data types with different conflict-resolve strategies vary in consistency level. 
The priority queue \textit{PQ-R} designed with the remove-win strategy merely provides the "Weak" consistency level, while the priority queue \textit{PQ-A} designed with the add-win strategy and \textit{PQ-F} designed with the \rwf framework both provide the stronger consistency level "Peer".
Moreover, the number of violations of the remove-win strategy is much larger than that of the other two strategies on the causal consistency level.
%The data type \textit{PQ-A} and \textit{PQ-F} satisfy the consistency level \textit{monotonic}, which guarantees the monotonic reads. 

Considering the high level design rationale, we may reasonably think that the remove-win strategy and the add-win strategy are dual of each other and are principally the same. However, the measurement by \vs show important difference in the consistency semantics. 
%Add-win and remove-win are dual strategies. However, applied to a complex data type like the priority queue, the consistency semantics are different.
%The consistency level resulting from the add-win strategy is stronger ("Peer"), while the remove-win strategy provides weaker consistency level ("Weak").
%Moreover, the violations of the remove-win strategy are significantly more than those of the add-win strategy.
The \rwf framework is an improvement on the traditional remove-win strategy. The remove-win strategy puts the remove operation behind the non-remove operation. In \textsc{RWF}, the remove-operation just removes the element from the container, thus avoiding the conflict. This \rwf strategy, seen as an improvement of the traditional remove-win strategy, strengthens the consistency semantics to the same level with the semantics of the add-win strategy.
%further utilize the potential of the remove-win strategy. It not only eases the development, but also provides stronger consistency semantics.
The consistency measurement results can help the CRDT designers to further understand the semantics of different resolution strategies. The application developers can also use the measurement results to choose appropriate data types they actually need.

The consistency measurement results of the set data type have important differences with those of the priority queue data type.
As for the add-win and \rwf resolution strategy, the consistency level of \textit{Set-A} and \textit{Set-F} is still "Peer", which is the same with the level of their counterparts \textit{PQ-A} and \textit{PQ-F}.
The main difference appears when considering the remove-win strategy. As for the set type, \textit{Set-R} also provides "Peer", while \textit{PQ-R} only provides "Weak".
The difference mainly results from that the priority queue has much more complex semantics than the set. When coping with complex semantics of the data type, the remove-win strategy will reduce the consistency semantics provided to the upper-layer applications. 
These measurement results show that the semantics of the data type should also be considered when choosing the conflict resolution strategies. 

%This measurement result can better instruct the applications developers to choose conflict resolution strategies. 
%The result can also help the CRDT designer better understand the cons and pros of each conflict resolution strategy and design more efficient strategies.

%Overall the data types designed with remove-win strategy generally provide weaker consistency than the ones designed with add-win strategy or the \rwf framework. 
%Moreover, we find that the data types designed with add-win strategy satisfy the same consistency level with the ones designed with the \rwf framework. 

%The findings are useful for designers and users of CRDTs. 
%Designers can choose a proper conflict-resolve strategy for data types, and users can minimize compensations to the inconsistency of data store during developing applications. 

As for the Riak case, the configuration of parameter $r$ plays the most important role in the consistency measurement. The effect of $r$ can be quantified by the consistency measurement based on \textsc{ViSearch}.
%The measurement result of Riak data types is easier to explain. 
%The parameters $r$ dominates the consistency level of different Riak data types. 
%Data types provide a stronger consistency when $r$ is larger. 
We find that both data types merely provide the "Weak" consistency level when $r=1$.
%In a high concurrency scenario, contacting only one replica before returning a query request guarantees a very weak data consistency. 
When $r=2$, a query request must contact a majority of replicas before returning. 
According to quorum-based protocol, data types with $r=2$ cannot strictly guarantee strong consistency. 
However, \textit{Set-r2} and \textit{Map-r2} actually provide strong consistency (the "Complete" consistency level) in the experiment.
The measurement results show that when the network condition is relatively reliable and the communication delay is low, e.g., in an intra-datacenter environment, the "$r=2$" configuration actually provides strong consistency, at least with high probability.
%because network condition is good in data center. 
This result is quite useful for applications which want strong consistency, but can tolerate data inconsistency in rare cases \cite{Wei17, Ouyang21}. The limited sacrifice in data consistency can greatly reduce the query delay.

%This measurement result may help Riak users a lot. 
%They can choose a small $r$ for lower latency without loss of consistency when network condition is good. 
%For subsequent improvements of Riak, the findings are also helpful. 

%\color{black}

%Though replicated data types are designed for eventual consistency, their behavior may actually adhere to stronger consistency models due to different client-server interaction modes and conflict resolution strategies, 
%and {\vs} can identify how much the consistency is strengthened.

%We will continue to measure consistency level across a wide range of replicated data types and consistency models. 
%We also try to increase the size of histories in the future, including more operations and concurrent threads. 

%--
\begin{table}[htb]
    \caption{Measurements for Data Types}
    \label{T: Result}
    \resizebox{\linewidth}{!}{  
        \begin{tabular}{|c|cccccc|l|l|}
            \hline
            & \multicolumn{6}{c|}{Violations}       &       &       \\ \cline{2-7}
            \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Data \\ Type\end{tabular}} & \multicolumn{1}{c|}{Co}            & \multicolumn{1}{c|}{Ca}       & \multicolumn{1}{c|}{P}        & \multicolumn{1}{c|}{M}        & \multicolumn{1}{c|}{B}        & W         & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}\# of \\ Histories\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Total \\ Time\end{tabular}} \\ \hline
            \textit{Set-r1}     & \multicolumn{1}{c|}{366}                      & \multicolumn{1}{c|}{339}                      & \multicolumn{1}{c|}{334}                              & \multicolumn{1}{c|}{295}       & \multicolumn{1}{c|}{188}       & \cellcolor[gray]{.8}0     & 300k          & 8h 3min      \\ \hline
            \textit{Set-r2}     & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}    & \multicolumn{1}{c|}{/}                        & \multicolumn{1}{c|}{/}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 300k          & 0h 11min      \\ \hline
            \textit{Map-r1}     & \multicolumn{1}{c|}{788}                      & \multicolumn{1}{c|}{734}                      & \multicolumn{1}{c|}{732}                                & \multicolumn{1}{c|}{712}    & \multicolumn{1}{c|}{542}      & \cellcolor[gray]{.8}0     & 300k          & 24h 26min       \\ \hline         
            \textit{Map-r2}     & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}    & \multicolumn{1}{c|}{/}                        & \multicolumn{1}{c|}{/}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 300k          & 0h 11min      \\ \hline
            \textit{PQ-A}       & \multicolumn{1}{c|}{478}                      & \multicolumn{1}{c|}{3}                        & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}            & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                        & 300k          & 4h 49min       \\ \hline                
            \textit{PQ-R}       & \multicolumn{1}{c|}{704}                      & \multicolumn{1}{c|}{131}                        & \multicolumn{1}{c|}{130}            & \multicolumn{1}{c|}{119}        & \multicolumn{1}{c|}{119}        & \cellcolor[gray]{.8}0                        & 300k          & 14h 17min       \\ \hline                
            \textit{PQ-F}       & \multicolumn{1}{c|}{1153}                      & \multicolumn{1}{c|}{3}                        & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}            & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                        & 300k          & 0h 18min       \\ \hline                
            \textit{Set-A}      & \multicolumn{1}{c|}{45}                        & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 500k          & 0h 19min         \\ \hline                
            \textit{Set-R}      & \multicolumn{1}{c|}{15}                        & \multicolumn{1}{c|}{4}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 400k          & 8h 9min         \\ \hline                
            \textit{Set-F}      & \multicolumn{1}{c|}{5}                        & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 500k          & 0h 19min         \\ \hline                
    \end{tabular}}
\end{table}

%----------------------------------------
\subsubsection{Consistency Measurement Cost}

To obtain the consistency measurement results in Table \ref{T: Result}, the checking time of \vs varies from 11 minutes to 24 hours. 
The consistency measurement time varies significantly as for different data types. In our experiment three out of ten types, \textit{Set-r1}, \textit{Map-r1} and \textit{PQ-R}, require significantly more time that other data types. Thus for most data types, the number of traces checked can be increased to a much larger number (e.g., 1 million) in bounded time. 
The checking time results demonstrate that consistency measurement using \vs can be accomplished under reasonable testing budget.
Also note that, the measurement process is not on the critical path of CRDT design, implementation, testing and maintenance. It can "borrow" the traces from the testing process and be finished in parallel with testing of CRDT implementations.

%The results of measurement clearly demonstrate the efficiency of {\vs} checking framework, and the ability of measuring out different consistency model. 
%The {\vs} framework can check a large number of histories which satisfy different consistency models in an acceptable time. 

Besides the total checking time using \textsc{ViSearch}, we further study the effects of the optimizations we propose, namely the pruning of search space and the parallelization of checking.
\begin{tbm}
    We use the \vs without pruning and parallelization as our baseline. Considering that the \vs without any optimization is just a non-recursive version of the existing algorithm, we actually compare the effects of optimizations with the checking algorithm in \cite{Emmi18}. 
\end{tbm}

%----------------------------------------
%\subsubsection{Efficay of parallelization}

As for the parallelization of consistency measurement, we study two data types \textit{Set-r1} and \textit{PQ-F}.
We measure 100K traces and change the number of threads of checking from 1 to 16. 
 %Our second measurement demonstrates the impact of our parallel optimization consistency checking. 
%We check the consistency 100000 \textit{Set-r1} histories and 80000 \textit{PQ-F} histories with single thread checking as the baseline. 
%Then we use parallel {\vs} to check these histories with different thread number. 
As shown in Figure \ref{parallel}, the checking time decreases as we increase the number of threads regardless of using or not using pruning.
The decrease in time is quite significant when we increase the thread number from 1 to 6 in the case of \textit{PQ-F}, and 1 to 6 in the case of \textit{Set-r1}. 
As we add more threads, the checking time decreases approximately linearly. This means that the time decreases slowly than the ideal case where the time decreases to $\frac{1}{k}$ $(k$ is the number of threads).
%The checking time is not exactly $\frac{1}{k}$ of the single-threaded(\textit{k} is thread number) 
\begin{tbm}
This is because we cannot totally get rid of the overloading of some threads and the starvation of some other threads. 
Also the cost of thread scheduling increases when the thread number becomes larger, which drags the efficiency of parallelization. 
\end{tbm}
% This is because we simply divide the subtrees to be checked to the threads (see Figure \ref{F: Parallel}). This straightforward allocation of workloads often results in significantly uneven workloads on the threads, especially when the number of threads increases.
% The overloading of some threads and the starvation of some other threads greatly reduce the effectiveness of parallelization.
This evaluation results can tell us what are the sweet points to choose the number of threads. It also motivates us to design better schemes to evenly divide the workload among threads.

\color{red}
    It is worth noting that there is a sharp fall of time consumption between 4 and 6 parallel threads in the evaluation of \textit{PQ-F}. 
    It costs 0.36(0.30), 0.35(0.26), 0.26(0.21), 0.16(0.14) hours without(with) pruning when parallel threads is 6, 8, 12, and 16.
\color{blue}
    If a history satisfies a consistency model, the time consumption of checking is determined by the first thread that find a certificate abstract execution. 
    For a thread, it may construct a certificate abstract execution after hausting most of allocated search state, or it may construct one just after several search state. 
    When we use more threads checking in parallel, there is a higher probability that a thread constructs a certificate abstract execution only in a short time. 
    So it is reasonable that the time consumption decreases steeply from the number of parallel threads is 4 to the number of parallel threads is 6. 
\color{black}


%The effect of parallel optimization becomes less noticeable when thread number becomes large, because thread scheduling overhead drags the efficiency of parallelization. 
%In general, parallelization substantially improves the efficiency of measurement, and reduces the time costs. 

%--
\begin{figure}[htb]
    \centering
    \subfigure[PQ-F] {
        \includegraphics[width=0.47\hsize]{figures/pq-f-bar.png}
    }
    \subfigure[Set-r1] {
        \includegraphics[width=0.47\hsize]{figures/set-r1-bar.png}
    }
    \caption{Evaluation of Time Cost}
    \label{parallel}
\end{figure}

%--------------------
%\subsubsection{Efficacy of Filtering}
As for the pruning, we use the \textit{pruning ratio} as the performance metric. 
For a data access trace, we measure the consistency level serially and count the number of explored search states. 
We calculate the \textit{pruning ratio}, i.e. the ratio of the number of explored search states checked with the pruning to the number without the pruning.
%Our third measurement demonstrates the efficacy of filter. 
%We check a history without filter, and check the same history with filter. 
%We count the explored \textit{search states} for two checking. 
%We evaluate the optimization of filter by the ratio of explored states with filter to explored states without filter. 
For data types studied in the experiment, we pick one representative from multiple configurations of this data type. Specifically, we calculate the pruning ratio of four data types: \textit{Set-r1}, \textit{Map-r1}, \textit{Set-F}, and \textit{PQ-F}. %, and we check 10000 histories for each data type. 

As for the pruning ratio, we find that the effects of pruning significantly vary, as the number of search states (without pruning) increases. Our intuition is that the effects of pruning are more significant when there are more states to be explored by \textsc{ViSearch}, and the evaluation results prove this intuition correct.
Specifically, we divide the number of explored states without the pruning into four grades: small ((0,30]), moderate ([31, 300]), large ([301, 3000]) and huge ([3001, $+\infty$]).
%types by the number of explored states without state filter: 
%(0,30] for small search, [31,300] for medium search, [301, 3000] for big search, and [3001, +$\infty$) for huge search. 
%Then we calculate the average optimization ratio for histories of each type . 
As shown in Figure \ref{F: Pruning}, except for the 'small' grade, the pruning can reduce the number of search states approximately by half. Note that, for 'small' traces, the checking time is quite limited, with or without the pruning. This shows that, for the total checking time using the \vs framework, the pruning can significantly reduce the checking time (approximately by half).

One exception is \textit{Set-r1}. The pruning ratio of \textit{Set-r1} is more than 70\%, even for huge traces. This is mainly because \textit{Set-r1} provides weak visibility (see Table \ref{T: Result}), and the weak visibility checking takes most of the time. However, the weak visibility consistency predicate imposes few constraints on the visibility relation. We can find few pruning predicates conforming to the predicate template over all possible abstract executions. 
Therefore, the effect of pruning for \textit{Set-r1} is limited. 

We can also find that the pruning does not work well for the set type. Because the semantics of set only cares about the existence of elements and imposes fewer constraints on operations than other data types. 
So we find fewer pruning predicates for set. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/pruningratio.png}
    \caption{Evaluation of State Filter}
    \label{F: Pruning}
\end{figure}

\begin{tbm}
Since the extraction and application of pruning predicates is also time-consuming, we also evaluate its impact on the overall checking time. 
As shown in Figure \ref{parallel}, the blue bar is the checking time without pruning and the orange bar is the checking time including predicate extraction and application. 
The orange bars is generally lower than the blue bars, which means pruning reduce the time consumption. Though the extraction algorithm is exponential, it is worth doing. 

In Figure \ref{F: Pruning}, \textit{PQ-F} has a better pruning ratio than \textit{Set-r1}, and it reflects on the time cost. In Figure \ref{parallel}, pruning has a better effect in \textit{PQ-F} compared to \textit{Set-r1}. 

We find that there is a negtive correlation between the effect of pruning and parallelization. When the effect of parallelization does not increases with the number of parallel threads any more, the effect of pruning is notable either. The parallelization increases the search state examined by \vs in unit time, and the pruning generally reduces a constant amount of state in the search space. So the pruning has a smaller impact on the time consumption, when the number of parallel threads becomes larger. 
\end{tbm}

%Our extraction of pruning predicates cannot find effective predicates for the pruning.

%the filter works well on big and huge searches which need to explore over 300 \textit{search states}, and these searches consume most of measuring time. 
%On short checkings, the filter does not have a good performance
%because the checking algorithm can easily find out an abstract execution for these histories by exploring only a few \textit{search states}, which can not leverage the state filter fully. 
%In general, the filter significantly reduces the explored \textit{search states} of checking, especially for those histories which cost long time to check. 

%--










==> ViSearch_complete_version/maintext_backup/intro.tex <==
%--
\section{Introduction}

%\hy{背景}

Large-scale distributed systems often resort to replication techniques to achieve fault-tolerance and load distribution \cite{Burckhardt14, Shapiro11a, Enes19}. For a large class of applications, user-perceived latency and overall service availability are widely regarded as the most critical factors. Thus, many distributed systems are designed for low latency and high availability in the first place \cite{Lloyd13}. These systems have to trade data consistency for high availability and low latency \cite{Brewer12, Gilbert12}. A common approach is to resort to \textit{eventual consistency}, i.e., allowing replicas of some data type to temporarily diverge, and making sure these replicas will eventually converge to the same state in a deterministic way. The Conflict-free Replicated Data Type (CRDT) framework provides a principled approach to maintaining eventual consistency \cite{Shapiro11a, Burckhardt14}. 

CRDTs are key components in modern geo-replicated systems, such as Riak \cite{Riak}, Redis-Enterprise \cite{Redis-Enterprise}, and Cosmos DB \cite{CosmosDB}. Though CRDT designs and implementations widely use the notion of eventual consistency, this is a rather fuzzy consistency term and covers a broad range of actual consistency behaviors. Providing only eventual consistency makes programming over CRDTs difficult, in the sense that there can be arbitrary divergence between the replicas \cite{Bermbach14, Lloyd13}. 

The tension between the wide use of eventual consistency and the difficulty of programming over CRDTs motivates the measurement of eventual consistency \cite{Bailis14-vldbj, Burckhardt14-book, Golab14}. On the one hand, both providers and consumers of the distributed storage service benefit from knowing the precise degree of data (in)consistency. Quantifying the degree of data inconsistency can even enable customers and service providers to negotiate compensations proportional to the severity of violations in certain scenarios \cite{Golab11}.
\begin{tbm} On the other hand, pragmatic protocols in the practice of Cassandra, Mongodb, and Eiger actually achieve consistency guarantees stronger than eventual consistency \cite{Lloyd13}. \end{tbm} Existing practical stronger consistency semantics can be and should be utilized. Precise reasoning about the consistency semantics will significantly ease the burden of programming over CRDT data stores.

\begin{tbm}
Existing consistency measurement schemes are mainly based on certain metrics delineating the staleness of data, e.g., how long the data has been stale and how many new versions of data has been generated. 
These schemes measure data consistency by how many time units the value returned has been stale, or how many versions the data has been updated when the returned value is obtained. 
Since time units and versions can be expressed in numerical values, it is easy to compare the consistency of different data types. 
However, above consistency measurement schemes have their drawbacks. 
Neither time-based or version-based consistency measurement schemes can give a insight about how the data type actually works and how updates propogate across replicas. 
\end{tbm}

\begin{tbm} 
In this work we investigate a methodology for the precise measurement of replicated data type consistency semantics. 
We employ a formal specification framework for concurrent objects \cite{Bermbach14, Emmi18, Emmi19}. 
It is based on the \textit{visibility} and \textit{arbitration} relation over events of a history, and we call it the \textit{Visibility-Arbitration} framework (\visar in short). 
The \visar framework extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happen-before and linearization relations. 
The arbitration relation is a total order and plays the role as linearization in the linearizability. 
It indicates how the system resolves the conflicts between concurrent events. 
The visibility relation is an acyclic relation that describes the relative timing of update propagation among operations. 
If an operation $a$ is visible to $b$, it means that the effect of $a$ is visible to the client performing $b$. 
We consider that two events are concurrent, if they are invisibile to each other. 
\end{tbm}
The weaker the visibility relation, the more an operation is allowed to ignore the effects of concurrent operations that are linearized before it. 
Tuning the definition of the visibility relation gives us different levels of data consistency. 
We use diverse constraints on the visibility relation to define different levels of data consistency.

%\mybreak

%\hy{挑战}
\begin{tbm}
Visibility relaxation using the \visar framework is mainly used to precisely specify the consistency semantics of concurrent objects optimized for high-performance multithreaded code \cite{Emmi19, Emmi18}. 
Since concurrent objects often employ lock-free implementations and do not provide atomicity, the \visar framework is designed to measure the deviation from atomicity. 
However, in our replicated data type store scenarios, the replicated data types are designed to provide eventual consistency in the first place, and practical implementations often provide stronger semantics than the mere requirement of eventual consistency. 
Our main objective is not to measure the deviation from strong consistency, but to measure the augmentation over weak consistency.
\end{tbm}

\begin{tbm}
Though consistency measurement using the \visar framework is NP-hard in general \cite{Gibbons97, Emmi18}, brute-force checking algorithm is employed in the measurement. 
In Emmi et al.'s work, they use a brute-force checking algorithm to enumerate all correct executions, and quite small workload is studied (two threads, no more than 6 operations, and up to 2 values) \cite{Emmi19}. 
The key insight to circumvent the NP-hardness obstacle is that the violations are often local. That is, only a few operations can witness the violation. 
The small workload is repeated a sufficient number of (millions of) times to find and measure the deviation from atomicity. 

An optimization with greedy algorithm is proposed in another work \cite{Emmi18}. 
This algorithm constructs the correct execution with minimal exetension, which avoids some unnecessary enumeration in the above brute-force checking algorithm. 
However, the performance of the recursive algorithm is not efficient enough for consistency measurement in replicated data type store scenarios. 
We continue to optimize the checking algorithm based on this. 
\end{tbm}

%To find atomicity violations in concurrent programming, this is enough and it works. Small workload guarantees exhaustive checking. Exhaustiveness is more essential to find atomicity violations.

%\color{teal}

Our intuition is that the NP-hardness obstacle can also be circumvented in consistency measurement in replicated data type store scenarios. 
Certain domain knowledge can be leveraged to reduce the measurement cost, while moderately sacrificing the generality of the measurement algorithm.
Following this intuition, our first challenge is to refactor the brute-force consistency algorithm to conveniently incorporate such optimizations.
The second challenge is to find the locality of weak consistency measurement in realistic replicated data type store scenarios.

Toward the challenges above, we first transform the brute-force recursive algorithm for consistency measurement to a non-recursive algorithm skeleton.
Note that, the basic rationale of the measurement based on \visar is to try all possible abstract executions, i.e., all possible permutations of operations as well as all possible visibility relations between operations.
In the non-recursive algorithm skeleton, the intermediate state for construction of the abstract execution is explicitly maintained at runtime.
\begin{tbm}
Although it is a rewirte of the recursive algorithm, it facilitates the pruning and parallelization. 
Thus predicates which can be used to prune the search space can be flexibly "plugged" into the search skeleton. 
For load balancing, the algorithm needs to dynamic dispatch work to threads. 
But the recursive algorithm maintains the intermediate state in stack frame, which means that the visit order of states is fixed at recursive call, and cannot adjust dynamically any more. 
We discuss more details about the gains achieved from the transformation from recursive to non-recursive in Sec \ref{Sec: VS}. 
\end{tbm}

We extract useful filters by exhaustively enumerate all valid abstract executions for subhistories pertaining to one single data element. 
We name the subhistory we consider the query cluster. The query cluster contains multiple \textit{dictating updates} on some data element and one \textit{dictated query} on the very data element.
We enumerate all valid abstract executions over the query cluster, to extract "pruning predicates", i.e., arbitration and visibility relations that any valid abstract execution of the query cluster must hold. These pruning predicates must also hold on all valid abstract executions of the whole history. Thus \vs can use the pruning predicates to avoid unnecessary searching.
Moreover, since the construction of different abstract executions are independent, the search can be parallelized in a straightforward way.

We conduct experiments on two replicated data type stores Riak \cite{Riak} and CRDT-Redis \cite{CRDT-Redis}. %\footnote{Redis-CRDT is our revision of Redis. Redis-CRDT adopts the peer-to-peer multi-master architecture and CRDTs are used to resolve conflicting updates.} \cite{} 
Since our optimization of the consistency checking algorithm is still exponential in the worst-case, it is still intractable to measure data type access traces of arbitrary length.
As inspired by the application of the \visar framework in \cite{Emmi19}, we utilize the locality of consistency measurement in replicated data type scenarios, and measure the consistency of data type access traces at reasonable cost. We also study the effects of the pruning predicates and the parallelization through experiments.

The experimental evaluation also shows that the consistency measurement results are useful for both replicated data type designers and upper-layer application developers.
The measurement quantifies the difference between different conflict resolution strategies, as well as the difference between different configurations of the replicated data type store. 

The rest of this work is organized as follows.
Section \ref{Sec: Preli} introduces the basic concepts of conflict-free replicated data types and those of the \visar framework.
Section \ref{Sec: VS} introduces the \vs consistency measurement framework, and Section \ref{Sec: Exp} presents the experimental evaluation.
Section \ref{Sec: RW} discusses the related work. 
In Section \ref{Sec: Concl}, we conclude this work and discuss the future work.


==> ViSearch_complete_version/maintext_backup/preli.tex <==
%--
\section{Preliminaries} \label{Sec: Preli}

In this section, we first introduce the basic concepts of Conflict-free Replicated Data Types (CRDTs). Then we introduce the Visibility-Arbitration (\textsc{Vis-Ar}) framework and consistency measurement based on visibility relaxation.

%--------------------------------------------------------------------------------
\subsection{Data Types}

We consider objects of data types stored in a replicated data store. 

\begin{definition}
    (Data Types). A data type $\tau \in \textit{Type}$ is a pair $\tau = (\textit{Op}, \textit{Val})$ such that
    \begin{itemize}
        \item \textit{Op} is the set of operations supported by $\tau$;
        \item \textit{Val} is the set of values allowed by $\tau$. We denote $\perp \in \textit{Val}$ to indicate that there is no return values for some operations. 
    \end{itemize}
\end{definition}

\begin{definition}
    (Sequential Semantics). The sequential semantics of a data type $\tau \in \textit{Type}$ is defined by a function $\mathcal{F}_{\tau}: \textit{Op}^{*} \times \textit{Op} \rightarrow \textit{Val}$. It means that given a sequence of operations $S$ and an operation $o$, the return value of $o$ is $\mathcal{F}_{\tau}(S, o) \in \textit{Val}$ when $o$ is performed right after $S$. 
\end{definition}

We denote an operation in the form of "$m(arg_1, \ldots, arg_n)\Rightarrow r$" to represent the invocation of a method $m$, with arguments $arg_1, \ldots, arg_n$, resulting in a return value $r$. 
We use sequential semantics to explain the execution of operations. The return value of an operation is determined by a certain sequence of operations that are performed before or concurrent with it. 

In this work, we consider operations are either queries or updates. 
Query operations only inspect state of the data type and do not change the state, while update operations modify state of the data type. 
Some data types may provide query-update primitives, i.e., operations inspect state of the data type and modify it at the same time. For example, the $extract\text{-}max()$ primitive of a priority queue is a query-update primitive, since it both obtains the maximum priority value and deletes the element with the maximum priority.
We can rewrite the history with query-updates and decompose each query-update operation into a pair of query and update \cite{Wang19}. 
So we only consider query operations and update operations in this work. 

% The salient feature of the CRDT is that the update operations are handled immediately without communication with remote replicas. Then the updates are asynchronously propagated to remote replicas. 
% We often omit the return value of update operations as they usually only return \textsf{ACK}. 


% An implementation \textit{Impl} of a replicated data type is a mapping from operations sequence $o_1 o_2 \ldots o_n$ to a return value sequence $Impl (o_1 o_2 \ldots o_n)=r_1 r_2 \ldots r_n$. For a total order of operations conducted on the data type, the return values of query operations and effects of updates operations follow the semantics of the standard data types. As for concurrent and conflicting updates, the effects of the updates are decided by the semantics of the CRDT, which are rigorously specified by the CRDT protocol.
% The logics for querying multiple replicas and merging the results from different replicas are often left to the upper layer application.

%--------------------------------------------------------------------------------
\subsection{\visar Framework Basics}

A consistency model acts as the contract between the underlying data type store and the upper-layer applications.
The \visar framework is an axiomatic consistency specification of concurrent objects \cite{Bermbach14, Emmi18, Emmi19}. 
It extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happens-before and linearization relations. 
The weaker the visibility relation, the more an operation is allowed to ignore the the effects of concurrent operations that are linearized before it. 
Tuning the definition of the visibility relation gives us different levels of data consistency. We use various predicates (i.e., constraints) on the visibility relations to define different levels of data consistency.

% We consider an abstract notion of executions, or behaviors, which captures observed return values and platform-defined happens-before orders among invocations in a given program. 
Histories, i.e., traces of data type access, are a set of all observable behaviors $\mathcal{H}$. The history defines how the clients interact with the data type store, and specifies what information is recorded about this interaction.
\begin{definition}
    (History). A history is an event graph represented by a tuple $\mathcal{H} = (E, op, rval, so)$ such that
    \begin{itemize}
        \item $E$ is the set of all events of operations performed by clients in a single execution; 
        \item $op : E \rightarrow Op$ describes the operation of an event; 
        \item $rval : E \rightarrow Val$ describes the return value of the operation $op(e)$ of an event $e$; 
        \item $so \subseteq E \times E$ is a partial order over $E$, called \textit{session order}.It describes the order of operations invoked by clients within a session. 
    \end{itemize}
\end{definition}

In this work, we only record the order between operations within the same session. The happens-before relation in this paper is limited to events/operations within the same session. 
 We do not record the \textit{returns-before} order over events which captures the real-time ordering of non-overlaping operations \cite{Burckhardt14-book}. Because we do not have a global time in distributed scenarios considering the clock drifting. 

%as there does not exist a unique write for each read operation in replicated data type scenarios. 

% Abstract Execution
In order to tell whether a history is consistent or not, the basic rationale underlying the \visar framework is that, a history is consistent if and only if we can justify it, by augmenting it with some additional information that explains the observed return values. 
For example, the linearizability consistency model inserts commit points in the timeline to justify the correctness of the observed return values. 

Based on the \visar framework, we add arbitration (i.e., linearization) and visibility relations to a history, and the augmented history is called an \textit{abstract execution}.
%Abstract executions are histories enriched by additional information about visibility and arbitration. 
%In the Vis-ar framework, the methodology of checking consistency of an implementation is based on abstract executions. 
% * This allows us to define not just linearizability, but the 
% By turning the arbitration and visibility relations in abstract executions, we can define a spectrum of consistency models that are commonly used for eventually consistent data type stores. Specifically, \textit{arbitration} is a linearization or total order on operations which indicates how the system resolves conflicting updates.
% If an operation $a$ is arbitrated before $b$ (denoted by $a \stackrel{ar}{\rightarrow} b$), it means that the system considers operation $a$ to happen earlier than operation $b$. 

% The \textit{visibility} relation is an acyclic relation, which describes the relative timing of update propagation among operations.
% If an operation $a$ is visible to $b$ (denoted by $a \stackrel{vis}{\rightarrow} b$), it means that the effect of $a$ is visible to the client performing $b$. 
% In replicated data type stores where replicas communicate with each other via messages, this means that the replica that performs operation $b$ receives the message containing operation $a$ before operation $b$ was performed. 
% In this work, we use $vis$ to represent visibility relation. 
% Given the definition of $lin$ and $vis$, an abstract execution is defined as an event graph $\mathcal{A} = (E, op, rval, hb, ss, lin, vis)$. 
%where \textsf{vis} is an acyclic and natural relation, and \textsf{ar} is a total order. 

\begin{definition}
    (Abstract Execution). An abstract execution is a triple $\mathcal{A} = ((E, op, rval, so), vis, ar)$ such that
    \begin{itemize}
        \item $(E, op, rval, so)$ is a history;
        \item Visibility $vis \subseteq E \times E$ is an acyclic and natural relation; A relation $R \subseteq A \times A$ is natural if $\forall x \in A : \left\vert R^{-1}(x) \right\vert < \infty$;
        \item Arbitration $ar \subseteq E \times E$ is a total. 
    \end{itemize}
\end{definition}

If an operation $a$ is visible to $b$ (denoted by $a \stackrel{vis}{\rightarrow} b$), it means that the effect of $a$ is visible to the client performing $b$. 
If an operation $a$ is arbitrated before $b$ (denoted by $a \stackrel{ar}{\rightarrow} b$), it means that the system considers operation $a$ to happen earlier than operation $b$. 
We use $lin$ to denote the linearization of operations after we decide the arbitration for concurrent operations. 

\setlength\emergencystretch{\hsize}

% We introduce the notion of subhistory $\mathcal{H}' = (E', op', rval', hb', ss')$, which denotes the projection of history $\mathcal{H}$ on a subset of events $E' \subseteq E$. 
% The notions $op'$ and $rval'$ are $op$ and $rval$ restricted on $E'$ respectively.
% The happens-before order $hb'$ is defined as $hb' = hb \bigcap (E' \times E')$ and the same-session relation $ss'$ is defined as $ss' = ss \bigcap (E' \times E')$. 
% Similarly, we can define the notion of projection for an abstract execution. 
% The projection of an abstract execution $\mathcal{A}$ on $E'$ is $\mathcal{A'} = (E', op', rval', hb', ss', lin', vis')$, 
% where $(E', op', rval', hb', ss')$ is the projection of the original history on $E'$. 
% The arbitration $lin'$ is defined as $lin' = lin \bigcap (E' \times E')$ and the visibility relation $vis'$ is defined as $vis' = vis \bigcap (E' \times E')$. 

\begin{definition}
    (Consistency Models). A consistency model is a set of consistency guarantees on abstract executions. 
\end{definition}

A consistency guarantee $\mathcal{\phi}$ is a constraint or property of an abstract execution $\mathcal{A}$. 
We write $\mathcal{A} \models \mathcal{\phi}$ if the abstract execution $\mathcal{A}$ satisfies the consistency guarantee $\mathcal{\phi}$. 

We can define a large variety of consistency guarantees by formulating conditions on the various attributes and relations appearing in the abstract execution.

An abstract execution $\mathcal{A}$ satisfies consistency model $\Phi = \{\mathcal{\phi}_1, \mathcal{\phi}_2, \ldots, \mathcal{\phi}_n\}$, if it satisfies every consistency guarantees in $\Phi$. Formally, $\mathcal{A} \models \Phi \Leftrightarrow \mathcal{A} \models \mathcal{\phi}_1 \land \mathcal{A} \models \mathcal{\phi}_2 \land \ldots \land \mathcal{A} \models \mathcal{\phi}_n$. 

A history $\mathcal{H}$ satisfies the consistency model $\Phi$, denoted $\mathcal{H} \models \Phi$, if it can be extended (by adding visibility and arbitration) to an abstract execution that satisfies consistency model $\Phi$. Formally, $\mathcal{H} (E, op, rval, so) \models \Phi \Leftrightarrow \exists vis, ar. ((E, op, rval, so), vis, ar) \models \Phi$. 

There are mainly two types of consistency guarantees. 
One is about ordering of operations. This type of guarantees mainly consist of constraints on arbitration and visibility relations.
%guarantees (such as causality) that defines rules for reordering of operations, 
%and convergence guarantees that ensure eventual consistency. 
The other is about data type semantics that gives meaning to operations. %Every event in an abstract execution must have a return value which is allowed by the semantics $Impl$ of given replicated data type. 

\subsection{Consistency Measurement via Visibility Relaxation} \label{SubSec: Vis-Relax}

In \cite{Emmi19}, a consistency spectrum consisting of six consistency models is defined by visibility relaxation, i.e., gradually relaxing the constraints on the visibility relations in the abstract execution.
These models, from weak to strong, are \textit{weak}, \textit{basic}, \textit{monotonic}, \textit{peer}, \textit{causal} and \textit{complete} visibility.

The two ends of the consistency spectrum are weak and complete visibility. The weak visibility permits any observations made by an operation, while the complete visibility requires that operations observe all operations which are linearized before them. 

Between the two ends, the basic visibility requires operations to see their happens-before predecessors which corresponds to a strengthening of the read-your-writes guarantee. 
The monotonic visibility requires each operation to see those its happens-before predecessors see. It corresponds to the monotonic reads guarantee, which states that reads observe an increasing sets of updates. 
On the basis of monotonic, the peer visibility requires a read to observe an update only if it has observed all the predecessors from the update's session, which corresponds to the monotonic writes guarantee.
The causal visibility requires that the visibility relation be transitive. It means that each operation is require to see those visible to the operations that it sees. 

We call them six consistency levels in the rest of this work, and use this 6-level scale of consistency levels for the consistency measurement.

\begin{tbm}
    We define a set of predicates which constraint the observation made by a given operation. 
    Formally, a visibility predicate $\varphi(o, \mathcal{A})$ is a first-order predicate on operation $o$ in an abstract execution $\mathcal{A}$. Given an abstract execution $\mathcal{A}$, we define $vis(o)$ is a set of operations visible to $o$; $hb(o)$ is a set of operations that happens before $o$ according to the session order $so$; $lin(o)$ is a set of operations arbitrated before $o$. 
    \begin{itemize}
        \item weak$(o, \mathcal{A}) \Leftrightarrow \textbf{\textit{true}}$
        \item basic$(o, \mathcal{A}) \Leftrightarrow hb(o) \subseteq vis(o)$
        \item monotonic$(o, \mathcal{A}) \Leftrightarrow \forall o' \in hb(o): vis(o') \subseteq vis(o)$
        \item peer$(o, \mathcal{A}) \Leftrightarrow$ monotonic$(o, \mathcal{A}) \land \forall o' \in vis(o): hb(o') \subseteq vis(o)$ 
        \item causal$(o, \mathcal{A}) \Leftrightarrow$ basic$(o, \mathcal{A}) \land \forall o' \in vis(o): vis(o') \subseteq vis(o)$ 
        \item complete$(o, \mathcal{A}) \Leftrightarrow lin(o) \subseteq vis(o)$
    \end{itemize}
\end{tbm}

\color{blue}
In Figure \ref{F: Visibility}, we show the difference of several level of visibility. 
The operations(rounded rectangle) visible to the given operation(bold rounded rectangle) depend on the visibility level. 
The \textit{basic} imples that visibility(solid arrow) of happens-before predecessors(horizontal line) while \textit{monotonic} implies visibility of those visible(dashed arrow) to predecessors. 
The \textit{peer} implies visibility of predecessors of visible operations, and \textit{causal} implies transitive visibility. 
visibility of predecessors of visible operations
\color{black}

\begin{figure}[htb]
    \includegraphics[width=\linewidth]{figures/visibility.jpg}
    \centering
    \caption{Visibility}
    \label{F: Visibility}
\end{figure}

Basically, the consistency measurement is conducted on one history or trace of replicated data type access. Theoretically speaking, to measure consistency guarantee of one data type, we need to measure all possible traces of this data type, which is simply not possible. Moreover, it is usually quite difficult to strictly prove the consistency level certain replicated data type provides. In this work, when we say consistency measurement for one data type, we mean that a sufficiently large number of traces generated by this data type is measured, and the result of this measurement is a sufficiently accurate approximation of the consistency level provided by this data type.

==> ViSearch_complete_version/maintext_backup/rw.tex <==
%--
\section{Related Work} \label{Sec: RW}

%\hy{怎么规约}

The fuzzy nature of eventual consistency and its wide adoption motivate the quantification of severity of consistency violations \cite{Golab11, Golab14, Golab18}. Existing quantification techniques can be viewed from two perspectives. From the micro-perspective, existing consistency measurement schemes are mainly based on certain metrics delineating the staleness of data, e.g., how long the data has been stale and how many new versions of data has been generated.
%The metric can be how long the data has been stale, e.g. $\Delta$- and $\Gamma$-consistency \cite{Golab14}, and how many new versions of data has been generated, e.g. $k$-atomicity \cite{Golab18}. 
Time-based quantification techniques, e.g. $\Delta$-atomicity \cite{Golab11} and $\Gamma$-atomicity \cite{Golab14}, are adopted for applications sensitive to realtime consistency requirements. Time-based techniques measure data consistency by how many time units the value returned has been stale. 
For applications sensitive to the frequency of data updates, version-based quantification techniques , e.g. k-atomicity \cite{Golab18}, are proposed. Version-based techniques measure data consistency by how many times the data has been updated when the returned value is obtained.
From the macro-perspective, Yu and Vahdat propose TACT (Tunable Availability and Consistency Tradeoffs), a middleware layer that supports application-dependent consistency
semantics expressed as a vector of metrics defined over a logical consistency unit or conit \cite{Yu02-TOCS}. Inconsistencies in the observed value of a conit are bounded using three metrics: numerical error, order error, and staleness.

The consistency measurement schemes above are from the end user's perspective. In order to better facilitate the development of upper-layer applications, we need to measurement schemes which focus on how data are updated, in a similar way to how linearizability is specified. To this end, in this work we borrow the \visar framework which is an axiomatic consistency specification framework of concurrent objects. %which consider operation visibility. 
The \visar framework extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happens-before and linearization relations. 
The \visar framework is more suitable for developers to reason about the correctness of the implementation of a replicated data type. It is also suitable for upper-layer application developers to reason about the correctness of applications.

%\hy{关于checking}

The checking of data type access traces is NP-Complete in general \cite{Gibbons97}.
However, this intractability result can be circumvented by reasonable assumptions in specific scenarios. For example, the write values are often assumed to be unique %, which can makes the checking problem tractable in many scenarios 
\cite{Gibbons97}. This assumption is reasonable and easy to satisfy, since we can append certain meta-data to the values written to make them unique. 
In replicated data type store scenarios, the number of concurrent writes is often assumed to be bounded by some constant \cite{Golab18}. 
Practitioners can also limit the pattern of the input and derive an input specific efficient checking algorithm \cite{Bouajjani17}. 

The checking of data type access traces using \vs is also intractable in the worst case. As inspired by the existing techniques to circumvent the NP-hardness obstacle, we refactor the brute-force checking algorithm to a generic algorithm skeleton. This refactor enables practical pruning of the exponential search space in certain scenarios. We also employ the locality of the checking of CRDT access traces to make the consistency measurement practical in realistic scenarios.

%\slt{关于粒度}
% The existing work measures the consistency of Java's concurrent objects at the per-method granularity \cite{Emmi19}. 


==> ViSearch_complete_version/maintext_backup/vs.tex <==
%--
\section{\vs Framework} \label{Sec: VS}

In this section, we first overview the basic design rationale behind the \vs framework. Then we present the key techniques. In the next Section \ref{Sec: Exp}, we will demonstrate how to apply the \vs framework in realistic data type store scenarios.

%--------------------------------------------------------------------------------
\subsection{\vs  Overview}

Consistency measurement using \vs boils down to the search of an abstract execution satisfying certain constraints on the arbitration and visibility relations. 
This search process involves enumerating the linearizations, i.e. arbitrations of all operations, as well as the visibility relations between operations.
To prove that one trace satisfies certain consistency model, it is sufficient to find one single abstract execution that satisfies all the constraints. % on the arbitration and visibility relations.
We name this abstract execution the "certificate" abstract execution (there could be more than one certificate execution).
%The success in finding one single abstract execution which satisfies the consistency model can prove that the trace satisfied certain consistency model
%Below we note arbitration as linearization because arbitration is actually a permutation of all operations. 
%The checking of each consistency level boils down to finding an arbitration of as well as the visibility among all operations. 

The search process is intractable in general \cite{Gibbons97, Emmi19, Emmi18}. However, the search can still be practical and cost-effective in replicated data type store scenarios. %, since the traces in real scenarios do not always force the checking algorithm to the worst case.
To enable efficient search of abstract executions, we first refactor the existing search algorithm to a non-recursive algorithm skeleton.
The intermediate states for construction of the abstract executions are explicitly maintained by the algorithm skeleton at runtime. 

\color{blue}
The traversal order of search is fixed in the existing recursive algorithm as the intermediate states are stored in the stack frame, which is actually a depth-first search. 
This is a simple way but has a drawback. The algorithm cannot adjust the traversal order according the runtime feedback, which impacts the parallel performance greatly. 
Because we only roughly estimate the workload of each thread before parallel search starting, and it leads to overloading and starvation between threads. We need to re-allocate the workload in a regular cycle, moving intermediate search states from overloading threads to starving threads. We can hardly do this in the recursive algorithm since all the intermediate search states are stored in the system's stack. 
\color{black}

Based on the \vs skeleton, we propose optimizations from two orthogonal dimensions. 
First, the non-recursive algorithm skeleton enables efficient pruning of the search space. 
We can flexibly plug pruning predicates into the algorithm skeleton to avoid the unnecessary search of certain abstract executions, while the pruning predicates can be extracted from the subhistory concerning multiple update operations and one query operation on one single data element. %certain part of the data type access traces. 
\begin{tbm}
Noted that a subhistory $\mathcal{H}'$ is the projection history $\mathcal{H}$ on a subset of events $E' \subseteq E$, and only keeps relations in the set $E' \times E'$. 
\end{tbm}
Second, we also find that the search process is stateless, i.e., the enumerate of different candidate executions are independent. Thus we further parallelize the search.  

%--------------------------------------------------------------------------------
\subsection{\vs Algorithm Skeleton}

We first briefly review the existing recursive search algorithm \cite{Emmi19, Emmi18}. Then we present the non-recursive algorithm skeleton.

%----------------------------------------
\subsubsection{The Original Recursive Search Algorithm}

Consistency measurement using the \vs framework can simply use a recursive backtracking algorithm to search the possible arbitration and visibility relations among operations in a brute-force way. We use $\ang{lin, vis}$ to denote an abstract execution. If an abstract execution $\ang{lin, vis}$ satisfies a consistency model $\Phi$, we have $\langle lin, vis \rangle \models \Phi$. 
During the search process, we manipulate some prefix of $lin$, denoted by $lin_i$. We use $vis_i$ to denote the visibility relation on operations in $lin_i$. 
The search algorithm can be view as extending candidate executions from $\ang{lin_i, vis_i}$ to $\ang{lin_{i+1}, vis_{i+1}}$.


%It is intuitive that $\langle lin_i, vis_i \rangle \models \varPhi$ if $\langle lin, vis \rangle \models \varPhi$. 
\setlength\emergencystretch{\hsize}
%until the abstract execution includes all operations.

The search algorithm tries all possible extensions from the current candidate execution $\ang{lin_i, vis_i}$. 
When valid extensions cannot be obtained, the current "candidate" is discarded and the search algorithm backtracks to another candidate execution.
%An abstract execution $\langle lin_i, vis_i \rangle$ can be extended with different choices of operations, and obtains a series of abstract execution $\left\{ \langle lin_{i+1}', vis_{i+1}' \rangle, \langle lin_{i+1}'', vis_{i+1}'' \rangle, \ldots \right\}$ as candidates. 
%We can select one of them as the extension of $\langle lin_i, vis_i \rangle$. 
When we finally extend the prefix to a whole abstract execution containing all the operations in the data type access trace, we successfully get the certificate abstract execution, and the search algorithm returns \textsf{TRUE}.
If no certificate extension can be obtained after trying all possible candidates, the search algorithm returns \textsf{FALSE}.

%At some point in construction, the abstract execution is invalidated if it is extended with any operation, and at that time the algorithm has to backtracks and search for other candidates. 

%If the algorithm finally manage to construct a complete abstract execution that includes all operation in the history, we obtain the certificate abstract execution which proves that the history satisfies the consistency model.

%Otherwise, the history does not satisfy the consistency model. 

%As construction of abstract execution follows the way of backtracking to search in a solution space, we name our algorithm framework {\vs} which means \textit{visibility-relaxation search}. 

%----------------------------------------
\subsubsection{The revised non-recursive search} \label{SubSubSec: Revised-VS}

The main improvement made to the recursive search algorithm is that we refactor it to a non-recursive one. This means that, the algorithm skeleton itself maintains a double-ended queue to store the intermediate search states $\ang{lin_i, vis_i}$ at runtime.
%To enable flexible optimization, we revise the original recursive search.
%The key in the refactorization is to use a stack to explicitly maintain the intermediate state of the search at runtime.
The explicit maintenance of intermediate search states greatly facilitates further pruning of unnecessary searches.

The non-recursive \vs algorithm searches abstract executions through phases, as shown in Figure \ref{F: Tree}. In each phase, it extends $\ang{lin_i, vis_i}$ to $\ang{lin_{i+1}, vis_{i+1}}$. There are two steps in each phase. In the 'ar step', we add one operation to $lin_i$ and obtain $lin_{i+1}$. In the 'vis step', we extend $vis_i$ to $vis_{i+1}$ by adding visibility relations concerning the newly added operation. 

%In each phase, we start from $\ang{lin_i, vis_i}$ and add a new operation to the linearization of the old search state and find a proper visibility relation for the newly added operation. 

\color{blue}
Formally, we denote a set $\mathcal{O}$ that contains all operations already in the $\ang{lin_i, vis_i}$. And we denote a set $\mathcal{U}$ that contains all operations in the history. 
In the 'ar step', we select an operation $o \in \mathcal{U} \setminus \mathcal{O}$, and obtain the new arbitration order $lin_{i+1} = lin_{i} \bigcup \mathcal{O} \times \{o\}$. 
In the 'vis step', we extend the visibility relation $vis_{i}$ by unioning a subset of $\mathcal{O} \times \{o\}$. And the new visibility relation $vis_{i+1}$ must satisfy the visibility constraint of consistency model. 

%--
\begin{figure}[htb]
    \includegraphics[width=\linewidth]{figures/tree.jpg}
    \centering
    \caption{Search State Extension}
    \label{F: Tree}
\end{figure}


As shown in Figure \ref{F: Tree}, the algorithm has already constructed a certificate abstract execution $\ang{lin_2, vis_2}$ that contains operations \textit{add}(1) and \textit{add}(2). Then the algotirhm starts phase 3. In the "ar step", the algorithm first appends operation \textit{size}() to the $lin_2$ and obatins $lin_3$. In this example, we require each operation must be visible to operations within the same session. So the operation \textit{size}() can return 1 if $add(1) \stackrel{vis}{\rightarrow} size()$, or return 2 if $add(1), add(2) \stackrel{vis}{\rightarrow} size()$. But neither of two visibility relations bring the correct return value, the algorithm backtracks for other candidates. 

Then we append operation \textit{remove}(2) to the $lin_2$. We can construct a certificate abstract execution $\ang{lin_3, vis_3}$ and finish phase 3. At last we start phase 4, and append the last operation \textit{size}() to the linearization. The operation \textit{size}() has four visibility extension candidates: $\left\{\textit{add(2)}\right\}\stackrel{vis}{\rightarrow}\textit{size}()$, $\left\{\textit{add(1)}, \textit{add(2)}\right\}\stackrel{vis}{\rightarrow}\textit{size}()$, $\left\{\textit{add(2)}, \textit{remove(2)}\right\}\stackrel{vis}{\rightarrow}\textit{size}()$, and $\left\{\textit{add(1)}, \textit{add(2)}, \textit{remove}(2)\right\}\stackrel{vis}{\rightarrow}\textit{size}()$. We omit candidates $\{\textit{add(2)}\}\stackrel{vis}{\rightarrow}\textit{size}()$ and $\{\textit{add(1)}, \textit{add(2)}, \textit{remove}(2)\}\stackrel{vis}{\rightarrow}\textit{size}()$ due to limited space in the picture. The operation \textit{size}() returns 0 only if $add(2), remove(2) \stackrel{vis}{\rightarrow} size()$, which means the operation \textit{size}() ignore the effect of the operation \textit{add}(1). Finaly, we find a certificate abstract execution, and prove the history satisfies the consistency model. 
\color{black}

%\slt{这里Impl前面没有定义？预计要在sec2定义，参考ra-lin的定义方式。}
%\mybreak
%\slt{下面，明确写出phase的概念，然后phase中分arb部分和vis部分。第一部分，统一用lin，不用再跟arb混着讲。}

%In detail, there are two steps in a phase: one for linearization and the other for visibility. 
%We first add a new operation to the total order, whose predecessors must have been already in the \textit{linearization}. 
%It means that $\langle \textit{lin}_i, \textit{vis}_i \rangle$ is extended to $\langle \textit{lin}_{i+1}, \textit{vis}_i \rangle$. 

%Then we extend the visibility relation which is compatible with the new linearization. 
%The visibility $\textit{vis}_i$ can be regarded as $\bigcup_{k = 1}^{i} v_k$ where $v_k$ is the visibility relation for the \textit{k}th operation in the linearization. 
%We construct the visibility relation incrementally by choosing a visibility relation \textit{v} for the operations that is newly added. 
%The visibility relation \textit{v} must adhere to the visibility specification of the given consistency model. 
%It means that we extend $\langle \textit{lin}_i, \textit{vis}_i \rangle$ to $\langle \textit{lin}_{i+1}, \textit{vis}_{i+1} \rangle$, where $\textit{vis}_{i+1} = \textit{vis}_{i} \cup v $. 

%There may be multiple choices to extend the linearization the visibility relation. 
%The candidate extensions of linearization are all equal. 
%But the candidate extensions of visibility can be ordered according to set inclusion, and we only need to consider the minimal visibility relations \cite{Emmi18}.

%\mybreak

%\slt{因为现在是强调我们的非递归重构，所以需要专门讲“非递归，自己搞栈”的一些细节，如果成功，就压栈如何继续。当不成功，就丢弃xxx，然后从栈里抽取出xxx，如何如何继续。}

%During the search process, we keep checking the consistency predicate. Whenever the consistency predicate is violated, the current candidate execution is discarded and we backtrack to search new candidates.

Upon initialization, we build a \textit{search state deque} with the initial search state $\ang{lin_0, vis_0}$. State $\ang{lin_0, vis_0}$ contains no operation and has an empty visibility relation. 
During the search process, we keep polling search states from the head of deque.
The newly popped search state is verified by the method \textsf{isValidAbstractExecution} ({Line 6 in Algorithm \ref{A: VS}}). This method basically checks whether the return values of all query operations in the current search state are allowed by the semantics \textit{Impl} of the data type under concern.
Invalid search states are discarded and valid ones are extended as follows. %We throw invalidated \textit{search states} away and extend validated \textit{search states}. 

For a given valid search state $\ang{lin_i, vis_i}$, we first extend the linearization by \textsf{linExtend} (Line 10 in Algorithm \ref{A: VS}), and get a set of new search states:
$$newLin = \left\{ \ang{lin_{i+1}^1, vis_i}, 
\ang{lin_{i+1}^2, vis_i}, \ldots, \ang{lin_{i+1}^p, vis_i} \right\}.$$
\color{blue}
Each new search state in \textit{newLin} represents a selection in $\mathcal{U} \setminus \mathcal{O}$. In fact, the number of new states $p$ should be less than or equal to the cardinality of \textit{newLin} because the extension of linearization needs to adhere to the same-session order. 
\color{black}

%\slt{把下标的i加上。把尖括号命令，换成新定义的ang{}命令。后续的search state不用再斜体。\\
%    \indent 发现i这个下标过载了，商量一下新的下标体系。}

Then we extend visibility relations according to the newly added operation.
%extend each \textit{search state} in \textit{newLins} for visibility. 
Each newly-extended \textit{search state} $\ang{lin_{i+1}^{r}, vis_i}$ will be extended to a set of \textit{search states}, 
$$newVis_r = \left\{ \ang{lin_{i+1}^{r}, vis_{i+1}^1}, \ang{lin_{i+1}^{r}, vis_{i+1}^2}, \ldots, \ang{lin_{i+1}^{r}, vis_{i+1}^{q}} \right\}.$$

%\slt{改下标等所有细节。}
\color{blue}
Each search state in $newVis_r$ corresponds to the selection of a subset of $\mathcal{O} \times \{o\}$, where $o$ is the newly-added operation and $\mathcal{O}$ contains operations in $lin_{i}$. 
\color{black}
Each search state in $\bigcup_{i=1}^{p} newVis_i$ is a possible extension of $\ang{lin_i, vis_i}$.We push all the candidate states into the head of deque. 
In the next step, the search algorithm will get a candidate from the head of deque and repeat this extension process. 
Once the search state cannot be extended any more, the algorithm will backtrack by polling older candidates from the head of deque. 

The {\vs} algorithm returns \textsf{TRUE} if it obtains a certificate abstract execution.
The algorithm returns \textsf{FALSE} if it runs out of candidates and still cannot obtain any certificate execution.
The pseudocode of the \vs algorithm skeleton is listed in Algorithm \ref{A: VS}.

%--
\begin{algorithm}[ht]
    \caption{The \vs Algorithm Skeleton}
    \label{A: VS}
    \KwIn{history $\mathcal{H}$, 
        data type implementation \textit{Impl}, 
        consistency model $\Phi$}
    \KwOut{whether history $\mathcal{H}$ satisfies the given consistency model $\Phi$}
    \textit{deque} $\leftarrow$ \{\ \}\\
    \textit{initState} $\leftarrow$ $\ang{\emptyset, \emptyset}$\\
    \textit{deque}.\textsf{push}(\textit{initState})\\
    \While{$\lnot$deque.\textnormal{\textsf{isEmpty}( )}}{
        \textit{state} $\leftarrow$ \textit{deque}.\textsf{pollHead}( )\\
        \If{\textnormal{\textsf{isValidAbstractExecution}(}Impl, state\textnormal{)}}{
            \If{state\textnormal{.\textsf{isComplete}( )}}{
                \Return{\textnormal{\textbf{true}}}
            }
            \textit{newLin} $\leftarrow$ \textit{state}.\textsf{linExtend}($\mathcal{H}$)\\
            \ForEach{\textit{newLinState} $\in$ \textit{newLin}}{
                \textit{newVis} $\leftarrow$ \textit{newLinState}.\textsf{visExtend}($\Phi$)\\
                \text{/* <Pruning is Plugged Here> */}\\
                \textit{deque}.\textsf{pushTailAll}(\textit{newVis})\\
            }
        }
    }
    \Return{\textnormal{\textbf{false}}}
\end{algorithm}


%---------------------------------------
\subsection{Pruning of the Search Space}

The key to circumventing the NP-hardness obstacle of abstract execution searching is to leverage specific knowledge of the data type under search and prune the search space. 
%We prune the search space to reduce the cost for searching valid abstract executions.
Thus, we inspect the data type access trace and automatically extract \textit{pruning predicates}, which can be plugged into the \vs algorithm skeleton (Algorithm \ref{A: VS}). 
For each candidate abstract execution, the search algorithm check the pruning predicates. Once any pruning predicate is detected \textsf{FALSE}, the candidate abstract execution is directly discarded.
We will prove that the pruning process is "safe", i.e., the pruning process never discards any candidate abstract execution which can be extended to a certificate abstract execution.

In this section, we first present the basic rationale of pruning with three illustrating examples.
Then we present the design and correctness proof of the pruning algorithm.

%--------------------
\subsubsection{Rationale of the Pruning}

The search algorithm enumerates every valid abstract execution in a brute-force way.
The insight behind our pruning scheme is that, for a  given data element in a container type, the update and query operations concerning this element cannot be linearized in an arbitrary way. Moreover, the visibility relations among these operations also have only limited patterns.
\color{blue}
% The insight behind our pruning scheme is that, the linearizations and visibility relations must follow some rules. 
For example, when we check a history of multiple shared variable access, 
% for each query operation that the set contains a certain element, there exists an update operation that add the element into the set.  
for each read operation \textit{r}, there exists a unique write operation \textit{w}. The operation \textit{r} and \textit{w} reads/writes the same variable and the same value. The operation \textit{w} must happen before \textit{r}. The rule mentioned above can be formally defined as the write-to order \cite{Wei16}. 
\color{black}

However, the \vs algorithm is not aware of this type of knowledge concerning one specific data element, and enumerates all abstract executions it thinks that is possible.
Thus, we can extract this type of knowledge and express it as pruning predicates. The predicates can be plugged into the \vs algorithm skeleton and prune the search space. %reduce the search cost.
\color{blue}
We will use these pruning predicates before adding new search states into deque ({Line 6 in Algorithm \ref{A: VS}}). 

We find that in a data type update and query operations invoked on a same data element usually form a cluster. The update operations determine the return values of query operations in the same cluster, while update operations rarely affect the query operations in the other cluster. 
\color{black}

Based on the insight above, we introduce the notion of a \textit{query cluster}. All operations in the query cluster are explicitly associated with the same data element.
The query cluster contains exactly one query operation, which is denoted the \textit{dictated query}. The query cluster contains one or more update operations, which are denoted \textit{dictating updates}. The dictating updates are those update operations which can potentially affect the return value of the dictated query. 

\color{blue}
We consider two situations. One situation is that the update operations are the necessary and sufficient condition for the result of a query operation. For example, whether the set contains the element \textit{x} is determined by the arbitration and visibility of all \textit{add} and \textit{remove} operations associated with element \textit{x}. 
The other situation is that the update operations are the necessary condition for the result of a query operation. For example, \textit{get\_max} tells that the maximum element of the priority queue is \textit{x} with value \textit{v}. All update operations associated with element \textit{x} only guarantee that there exists an element \textit{x} with value \textit{v} in the priority queue at that point, but there might be some elements with larger value than \textit{x}. However, the necessary condition is enough to ensure the safety of pruning. 

\color{black}

For example, inserting one element into the priority queue and increasing the priority value of the element, and returning the existence or priority value of the element.
We do not consider operations which correspond to multiple data elements, e.g., the $isEmpty()$ operation, which returns whether the data container is empty.

%like this, and do not take operations like $isEmpty()$ into account as they do not refer to a specific element. 

%\mybreak

%\slt{query被几个update完全决定}


% >>>>>具体的单元素操作的例子
%
%For example, an operation \textit{contains}(\textit{z}) is related to the its argument, the element \textit{z}, 
%and an operation \textit{get\_max}()$\Rightarrow$(\textit{x; v}) is related to its return value. 
%
%Update operations involved in the related element potentially determine the return value of the query operation. 
%
%The return value of operation \textit{contains}(\textit{z}) is totally decided by operation \textit{add} and \textit{remove} on element \textit{z}. 
%
%Similarly, operation \textit{get\_pri}(\textit{e}) is totally decided by operation \textit{insert}, \textit{remove}, and \textit{inc} on element \textit{e}. 
%
%Different from \textit{contains}() and \textit{get\_pri}(), operation \textit{get\_max}()$\Rightarrow$(\textit{x;v}) is not decided by update operation on element \textit{x}. 
%Because we need to assure that there does not exist any other element whose \textit{priority} is bigger than \textit{v}, 
%besides the necessary condition that there exists an element in the priority queue whose \textit{id} is \textit{x} and \textit{priority} is \textit{v}. 
%However, the existence of the element (\textit{x;v}) is totally decided by updates on element \text{x}. 
%So due to the the necessary condition, we say that operation \textit{get\_max}()$\Rightarrow$(\textit{x;v}) is partly decided by operation \textit{insert}, \textit{remove}, and \textit{inc} on element \textit{x}. 
%
% >>>>>



We will use two data types \textit{set} and \textit{priority queue} as illustrating examples for the extraction of pruning predicates.
The set is a container of elements, in which each element is identified by its unique \textit{id}. 
The following primitives are involved in examples: 
%--
\begin{itemize}
    \item $add(e)$ : add element $e$. 
    \item $remove(e)$ : remove the element $e$. 
    \item $contains(e)$ : return \textsf{TRUE} if $e$ is in the set.
    % \item $isEmpty()$ : return \textsf{TRUE} if the set is empty. 
\end{itemize}

\noindent The priority queue is a container of elements of the form $e = (id, priority)$.
The following primitives are involved in examples: 
%--
\begin{itemize}
    \item $insert(e, x)$ : enqueue element $e$ with initial priority $x$. 
    % \item $remove(e)$ : remove the element \textit{e}. 
    \item $inc(e, \delta)$ : increase the priority of element $e$ by $\delta$ (may be negative). 
    \item $get\_pri(e)$ : return the priority value of $e$.
    \item $get\_max()$ : return the \textit{id} and \textit{priority} of the element with the highest priority. 
    % \item $isEmpty()$ : return \textsf{TRUE} if the priority queue is empty. 
\end{itemize}

% 之前的版本侧重于讲我们如何利用cluster之间的locality去进行剪枝
% 新增的部分主要是说明为什么需要有template和extraction, 因为 
%   1. data type的语义变复杂了, 不是简单的shared variables, 读写之间的因果链条不再是直接的了. 很难人工为每一个data type定义出write-to order那样的规则
%   2. 引入vis之后一个操作可以忽略之前的操作了, 变得更加烧脑, 人定规则可能会遗漏case
% 所以需要template和extraction保证不管什么data type都能剪, 提取的剪枝谓词肯定safe

\color{blue}
It becomes difficult to seek out explicit rules like write-to order to extract pruning predicates, when we check data types with enriched semantics. For example, we can add or remove an element in the data type set. We can even increase and decrease the priority of an element. All these rich semantics of data types make the cause and effect between query operation and update operation are unclear. 
Visibility relations being introduced into consistency specification makes things much more complicated. because an operation may ignore the effects of other operations. Pruning predicates formulated by human are hardly perfectly safe. 

We want to extract pruning predicates automatically, and make sure that they are correct. In this context we define some templates which applies to various data types, and design a suite of algorithms that extract correct pruning predicates. 
\color{black}


The pruning predicate is obtained by inspecting the query cluster pertaining to one specific data element.
There can be two types of pruning predicates. 
The first type is simpler, which only considers the arbitration relation between operations, while the second type considers both the arbitration and the visibility relations.

%\mybreak

By in-depth inspection of the data type access trace and manual exploration of the brute-force checking process, we come up with three predicate templates, i.e. patterns of pruning predicates we want to extract.
The first predicate template focuses on the arbitration relation. It aims to find that two operations always have the arbitration relation, no matter how you construct the linearization of operations. Specifically, $\tarb$ states that operation $x$ must be arbitrated before operation $y$ in every search state $\ang{lin, vis}$:
%--
\begin{eqnarray*}
    \tarb(x, y) \mydef \forall \ang{lin, vis}, (x,y) \in lin
\end{eqnarray*}


To extract pruning predicates following the template $\tarb$, we enumerate all valid abstract executions of the subhistory consisting of all operations in one query cluster.
For example, assume that there is a subhistory with two client sessions.
One session has operation $insert(x,5)$, followed by $inc(x,1)$.
The second session has one single operation $get\_pri(x) \Rightarrow 6$.
For the ease of illustration, we simply assume that there are no other operations on $x$ in the whole trace. 

It is evident that the return value of $get\_pri(x)$ is 6 only if it is linearized after $inc(x,1)$.
All valid abstract executions of this query cluster must have this arbitration order $inc(x,1)  \stackrel{ar}{\rightarrow} get\_pri(x) \Rightarrow 6$.
This fact must also hold for all candidate abstract executions the \vs algorithm constructs. Thus it can be extracted as a pruning predicate and plugged into \vs to avoid unnecessary searches.

The second and the third predicate templates are of the second type and concern both the arbitration and the visibility relations. 
As for the $\tvis$ example in Figure \ref{F: Template}, if the arbitration relations among operations have been decided, we can infer that there must be the visibility relation between $remove(z)$ and $contains(z) \Rightarrow \textsf{FALSE}$. Otherwise, the semantics of the set type are violated.
The $\tnotvis$ example is the dual of the $\tvis$ one. If the return value of $contain(z)$ is \textsf{TRUE}, there should be no visibility relation between $remove(z)$ and $contain(z)$.

%According to *rulearb, we find a filter that $(ins, inc) \in lin$. In running the \vs checking algorithm, whenever this pruning predicate is false, the candidate abstract execution is discarded.

%Therefore, whenever the algorithm constructs an abstract execution which \textit{inc}(\textit{x},1) is linearized before \textit{insert}(\textit{x},5), 
%we prune this search state as the current abstract execution cannot be extended to a complete one. 

%The pair of \textit{insert}(\textit{x},5) and \textit{inc}(\textit{x},1) is a fact for $\mathcal{P}_{A}(x, y)$. 

%Moreover, it is reasonable to infer that \textit{insert}(\textit{x},5) and \textit{inc}(\textit{x},1) must be linearized before \textit{get\_pri}(\textit{x})$\Rightarrow$6. 

%\slt{Fig2要换成我们黑板上讨论的例子，不然文字读起来，读者易误解}

%--
\begin{figure}[htb]
    \includegraphics[width=\linewidth]{figures/rule.jpg}
    \centering
    \caption{Rule Examples}
    \label{F: Template}
\end{figure}

%\slt{图里的true，false要改字体，与正文统一。\\
%    \indent \indent 用not-vis，而不是non-vis。\\
%    \indent \indent rulea，ruleb要改，要是数学不好写，可以写the arb template, the vis template, the not-vis template之类的。}

Generalizing the examples above, $\tvis$ states that certain arbitration relations and certain visibility relation always co-occur:
%--
\begin{eqnarray*}
    \tvis(S_{lin}, x, y) \mydef \forall \ang{lin, vis} : (a,b) \in S_{lin} \rightarrow (x,y) \in vis %\\
    %\mathcal{P}(a, b, x, y) \stackrel{\triangle}{=} \forall \langle lin, vis \rangle : (a,b) \in lin \rightarrow (x,y) \in vis
\end{eqnarray*}

\noindent where $S_{lin}$ is a subset of the arbitration relation (a subset of operation pairs having the arbitration relation).
The dual template $\tnotvis$ states that if there are certain arbitration relations, certain visibility relation cannot occur:
%--
\begin{eqnarray*}
    \tnotvis(S_{lin}, x, y) \mydef \forall \ang{lin, vis} : (a,b) \in S_{lin} \rightarrow (x,y) \not \in vis %\\
    %\mathcal{P}(a, b, x, y) \stackrel{\triangle}{=} \forall \langle lin, vis \rangle : (a,b) \in lin \rightarrow (x,y) \not \in vis
\end{eqnarray*}

\noindent We scan all valid abstract executions of the query cluster and check whether there are operation patterns that can be match by the two predicate templates $\tvis$ and $\tnotvis$.

%To solve these problems, we develop a predicate extraction method. 

%We focus on subhistories consisting of multiple updates and one query all pertaining to one data element.

%We enumerate all possible abstract executions of the subhistory. 

%We match the predicate template over all possible executions, to see whether there are pruning predicates.

%We present the details below.

%For every abstract execution, we check whether there are predicates predicate template 

%This method enumerates all complete abstract executions of a small cluster, and extracts necessary conditions from all complete abstract executions to generate predicates. 



%----------------------------------------
\subsubsection{Extraction of Pruning Predicates}

The extraction of pruning predicates is similar to a "string matching" process. 
The predicate template is analogous to the pattern string to be searched, while all valid abstract executions of a query cluster as a whole is analogous to the text string being scanned.
Note that we are interested in predicates which are \textsf{TRUE} for all abstract executions of a given query cluster.
The query cluster can just be treated as a normal trace of data type acces, and we can directly use the brute-force the \vs checking algorithm (Algorithm \ref{A: VS}) to search all valid abstract executions. 
\color{blue}
We can regard the computing of extraction as constant complexity because the size of query cluster is rather small compared to the size of the history. We evaluate the time cost of pruing predicate extraction in Sec \ref{Sec: Exp}, and show that it is worth doing that. 
\color{black}
We extract from the executions concrete pruning predicates following the templates $\tarb$, $\tvis$ and $\tnotvis$. 

For an abstract execution $\pi_t$ = $\ang{{lin}^t, {vis}^t}$, we define that $lin(\pi_t)$ = $lin^t$, $vis(\pi_t)$ = $vis^t$. 
We define the not-visible relation of an abstract execution $\pi_t$ by $notvis(\pi_t)$ = $\{(x,y) \mid (x,y) \in lin^t \land (x,y) \notin vis^t\}$. 
% We define $\mathcal{U}(\mathcal{H}) = O \times O$ as a complete relation of operations in history $\mathcal{H}$.  

%\slt{下标似乎应该写在下面？跟前面讨论统一 \\
%    \indent \indent 全关系，定义去掉？放到伪码注释中？/* U is the complete relation which contains all possible pairs of operations.\\
%    \indent \indent yield T(op1, op2)。避免“未知数”的感觉}

It is straightforward to extract pruning predicates of template $\tarb$ from valid abstract executions. 
We just need to intersect every linearization of valid abstract executions, as shown in Algorithm \ref{A: T-ARB}.
Specifically, linearization of an abstract execution $\pi$ is a total order of operations. For each pair of operations, $(x,y) \in lin(\pi)$ means that operation $x$ is arbitrated before operation $y$ in abstract execution $\pi$. 
The intersection of all linearization is the arbitration order that every valid abstract execution must obey. 
Each concrete operation pair $(op1, op2)$ in the final intersection of linearizations can generate a concrete pruning predicate $\tarb(op1, op2)$. 

%--
\begin{algorithm}[ht]
    \caption{Extraction of Pruning Predicates for $\tarb$}
    \label{A: T-ARB}
    
    \KwIn{a set of abstract execution $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
    \KwOut{a set of pruning predicates of $\tarb$}
    
    $S_{\text{arb}}$ $\leftarrow$ $U$\quad\CommentSty{/* U is the complete relation which contains all possible pairs of operations. */}\\
    \ForEach{$\pi \in \mathcal{A}$}{
        $S_{\text{arb}}$ $\leftarrow$ $S_{\text{arb}} \bigcap lin(\pi)$
    }
    
    \ForEach{pair $(x,y) \in S_{\text{arb}}$}{
        \textbf{yield} $\tarb(x,y)$
    }
\end{algorithm}


To extract pruning predicates following the template $\tvis$, we union the visibility relation of all valid abstract executions: $\mathcal{V} = \bigcup_{t=1}^{m} vis(\pi_t)$. 
For each pair $(x,y) \in \mathcal{V}$, it means that operation $x$ is visible to operation $y$ in some valid abstract execution. 
Then we try to generate a concrete predicate of template $\tvis$ for every pair $(x,y) \in \mathcal{V}$. 

We first intersect the linerarization of valid abstract executions that contains the pair $(x,y)$. 
Any valid abstract execution whose visibility relation contains pair $(x,y)$ must obey the arbitration order in the intersection $S_{\text{arb}}$. 

Next we need to ensure that there exists no counterexample for this concrete predicate. %, or this concrete predicate is not a necessary condition for the subhistory. 
Because we extract this concrete predicate only from valid abstract executions which contain pair $(x,y)$ in their visibility relation. 
We must check whether it is a necessary condition for those valid abstract executions which do not contain pair $(x,y)$ in their visibility relation.
We discard this concrete predicate, if there is a valid abstract execution whose visibility relation does not contain pair $(x,y)$ but it obeys all arbitration order in the intersection $S_{\text{arb}}$.
The pseudocode of the extraction algorithm for $\tvis$ are listed in Algorithm \ref{A: T-VIS}.

%\slt{文字解释一下：为什么这个二次检测是必须的，不能遗漏。}

%--
\begin{algorithm}[ht]
    \caption{Extraction of Pruning Predicates for $\tvis$}
    \label{A: T-VIS}
    
    \KwIn{a set of abstract executions $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
    \KwOut{a set of pruning predicates of $\tvis$}
    
    $S_{vis}$ $\leftarrow$ $\bigcup_{t=1}^{m} vis(\pi_t)$\\
    \ForEach{pair $(x,y) \in S_{vis}$}{
        $S_{arb}$ $\leftarrow$ $U$\\
        \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \in vis(\pi)$}{
            $S_{arb}$ $\leftarrow$ $S_{arb} \bigcap lin(\pi)$
        }
        
        \textit{review} $\leftarrow$ \textsf{TRUE}\\
        \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \notin vis(\pi)$}{
            \If{$S_{arb} \subseteq lin(\pi)$}{
                \textit{review} $\leftarrow$ \textsf{FALSE}\\
                \textbf{break}
            }
        }
        \If{\textit{review} \textnormal{is} \textnormal{\textsf{TRUE}}}{
            \textbf{yield} $\tvis(S_{{arb}}, x, y)$
        } 
    }
\end{algorithm}

Since the template $\tnotvis$ is just the dual of $\tvis$, the extraction of concrete predicates for $\tnotvis$ is similar to the extraction for $\tvis$. 
We just replace the visibility relation in the $\tvis$ extraction algorithm with the not-visibility relation. 

%--
% \begin{algorithm}[ht]
%     \caption{Extraction of Pruning Predicates for $\tnotvis$}
%     \label{A: T-NOT-VIS}
    
%     \KwIn{a set of abstract executions $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
%     \KwOut{a set of pruning predicates of $\tnotvis$}
    
%     $S_{notvis}$ $\leftarrow$ $\bigcup_{i=1}^{m} notvis(\pi_i)$\\
%     \ForEach{pair $(x,y) \in S_{notvis}$}{
%         %$S_{arb}$ $\leftarrow$ $\mathcal{U}(\mathcal{H}_q)$\\
%         $S_{arb}$ $\leftarrow$ $U$\\
%         \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \in notvis(\pi)$}{
%             $S_{arb}$ $\leftarrow$ $S_{arb} \bigcap lin(\pi)$
%         }
        
%         \textit{review} $\leftarrow$ \textsf{TRUE}\\
%         \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \notin notvis(\pi)$}{
%             \If{$S_{arb} \subseteq lin(\pi)$}{
%                 \textit{review} $\leftarrow$ \textsf{FALSE}\\
%                 \textbf{break}
%             }
%         }
%         \If{\textit{review} \textnormal{is} \textnormal{\textsf{TRUE}}}{
%             \textbf{yield} $\tnotvis(S_{arb}, x, y)$
%         } 
%     }
% \end{algorithm}

%----------------------------------------
\subsubsection{Correctness of Pruning}
\color{red}
We now prove that the pruning is safe, i.e., no certificate execution can be discarded by the pruning predicates. 
Given a history $\mathcal{H}$ and a consistency model $\Phi$, if $\mathcal{H} \not\models \Phi$, it means that there exists no certificate abstract execution for $\Phi$. 
% An abstract execution of history $\mathcal{H}$ is certificate if and only if it satisfies the requirement of $\Phi$. 
So the pruning must be safe. 
Therefore in the rest of the proof, we focus on the case in which history $\mathcal{H}$ has a certificate abstract execution satisfying the consistency model $\Phi$. 

In fact, the \vs algorithm prunes abstract executions during the construction process at runtime. So we need to prove that no candidate abstract execution, which can be extended to a certificate execution in the future, is pruned.
%no constructing abstract execution which can be extended to a correct one is pruned by filter. 
However, if an abstract execution violates a pruning predicate, all of its extensions violate the filter too. 
Hence, we only need to prove that there does not exist a certificate execution which violates the pruning predicate. 

Here is the proof stretch of the correctness of pruning. 
We assume for contradiction that there exists a certificate abstract execution $\pi$ of history $\mathcal{H}$ which violates a pruning predicate $P$.
The pruning predicate $P$ is extracted from a certain query cluster in history $\mathcal{H}$, so we project the abstract execution $\pi$ on the query cluster and get a projection $\pi'$. 
The projection $\pi'$ is an abstract execution of the query cluster where the predicate $P$ is extracted. 

The arbitration and visibility relations among \textit{dictating updates} and \textit{dictated query} is reserved after projection, so $\pi'$ still violates the predicate $P$. 

For the same reason, the \textit{dictated query} of the query cluster has the same return value after projection. 
Since $\pi$ is a certificate abstract execution, each operation in $\pi$ does not omit any operations it must see according to the visibility constraint of $\Phi$. 
Compared to $\pi$, each operation in $\pi'$ only more omit  those operations discarded in projection, so the projection $\pi'$ still satisfies the visibility constraint. 
Hence the projection $\pi'$ still the consistency model $\Phi$. 

Because the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
Therefore, the pruning in \vs is safe. The candidate abstract executions discarded can never be extended to a valid certificate one.

\color{black}

% 证明剪枝正确性的方法一, 避开了繁琐的分类讨论, 引入新的概念函数G作为一个vis是否合法的判断依据
% 然后简单地通过投影后必须看见的操作应该相应地减少, 通过集合 \subseteq 的传递关系去完成证明
% 优点是证明看起来比较有理有据 不像分类讨论都是文字的叙述
% 缺点是引入了新的符号 新的形式化语言

% \color{red}
% Here is the proof stretch of the correctness of pruning. 
% We assume for contradiction that there exists a certificate abstract execution $\pi$ of history $\mathcal{H}$ which violates a pruning predicate $P$. The projection $\pi'$ is some abstract execution of the query cluster which generates predicate $P$. 
% We project the abstract execution $\pi$ on the subhistory where the predicate $P$ is extracted, and get the projection $\pi'$. %(可能需要补一下projection的定义)
% % The projection of the abstract execution $\mathcal{A} = ((E, op, rval, so), vis, ar)$ on $E' \subseteq E$ is $\mathcal{A'} = ((E', op, rval, so'), vis', ar')$, where $vis' = vis \cap (E' \times E')$ similar for $so$ and $ar$. 

% If the projection $\pi'$ still violates the predicate $P$ and satisfies the consistency model $\Phi$, we can prove that the pruning is safe. 
% Because the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
% This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
% Therefore, the pruning in \vs is safe. The candidate executions discarded can never be extended to a valid certificate abstract execution.

% It is trivival that the abstract execution $\pi'$ still violates the predicate $P$. Because $\pi'$ contains all the operations of the query cluster from which $P$ is extracted, and reserves the arbitration and visibility between these operations.

% We need to prove the satisfaction of the consistency model $\Phi$ from three points. Firstly the projection $\pi'$ is a legal abstract execution. Secondly the query operation in $\pi'$ has the same return value with the corresponding operation in $\pi$. Thirdly the abstract execution $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 

% The proof of the thrid point is a bit tricky. We define a relation $\mathcal{V}_k$ that describes the visibility of $o_k$, while the visibility relation of the first $k-1$ operations is fixed during the construction. 
% We extend the visibility relation of $\ang{lin_{k-1}, vis_{k-1}}$ to $\ang{lin_{k}, vis_{k}}$ by adding $\mathcal{V}_k$ to $vis_{k-1}$. 
% There exists a function $\mathcal{G}$ mapping a tuple $(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k)$ to a set $\mathcal{M}$. 
% The set $\mathcal{M}$ is the visibility relation that describles what $o_k$ at least see according to the visibility constraint of the consistency model. If $\mathcal{M} \subseteq \mathcal{V}_k$, $\mathcal{V}_k$ is a legal visibility extension for the consistency model $\Phi$. 

% After projection, some operations are discarded from the the abstract execution $\pi$. The visibility relation $\mathcal{V}_k$ becomes $\mathcal{V}_{k'}$, and we denote $\mathcal{R} = \mathcal{V}_k \setminus \mathcal{V}_{k'}$. 
% The operation $o_{k'}$ no longer need to see the discarded operations, and the discarded operations break the transitivity of visibility. So the $\mathcal{G}(\ang{lin_{k'-1}, vis_{k'-1}}, \mathcal{V}_{k'}, o_{k'}) = \mathcal{M'}$ is a subset of $\mathcal{M} \setminus \mathcal{R}$. 
% Hence there exists
% \begin{equation*}
%     \mathcal{M'} \subseteq \mathcal{M} \setminus \mathcal{R} \subseteq \mathcal{V}_k \setminus \mathcal{R} = \mathcal{V}_{k'}
% \end{equation*}
% The projection $\pi$ satisfies the visibility constraint of the consistency model $\Phi$. 

% Due to limited space, we put the detailed proof and the definition of function $\mathcal{G}$ on \cite{Shi22}. 

% \color{black}

% \begin{tbm}
% Here is the proof stretch of the correctness of pruning. 
% We assume for contradiction that there exists a certificate abstract execution $\pi$ of history $\mathcal{H}$ which violates a pruning predicate $P$. 
% We project the abstract execution $\pi$ on the subhistory where the predicate $P$ is extracted, and get the projection $\pi'$. %(可能需要补一下projection的定义)
% The projection of the abstract execution $\mathcal{A} = ((E, op, rval, so), vis, ar)$ on $E' \subseteq E$ is $\mathcal{A'} = ((E', op, rval, so'), vis', ar')$, where $vis' = vis \cap (E' \times E')$ similar for $so$ and $ar$. 
% The projection $\pi'$ is some abstract execution of the query cluster which generates predicate $P$.

% If the following two statement establish
% \begin{itemize}
%     \item the projection $\pi'$ still violates the predicate $P$;
%     \item the projection $\pi'$ satisfies the consistency model $\Phi$;
% \end{itemize}
% we can prove that the pruning is safe. 
% As the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
% This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
% Therefore, the pruning in \vs is safe. The candidate executions discarded can never be extended to a valid certificate abstract execution.
% % retains the linearization and visibility relation among operations in subhistory. 

% If the following two statement establish
% \begin{itemize}
%     \item the projection $\pi'$ still violates the predicate $P$;
%     \item the projection $\pi'$ satisfies the consistency model $\Phi$;
% \end{itemize}
% we can prove that the pruning is safe. 
% As the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
% This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
% Therefore, the pruning in \vs is safe. The candidate executions discarded can never be extended to a valid certificate abstract execution.

% Here is the detailed proof of the two statement. 
% The projection $\pi'$ contains all the operations of the query cluster from which $P$ is extracted, and the projection reserves the relations between operations of the query cluster. So the abstract execution $\pi'$ still violates the predicate $P$. 

% Next we prove that $\pi'$ satisfies the consistency model $\Phi$, which means $\pi'$ is a valid abstract execution of the query cluster. 

% First, the projection keeps a total order $ar'$ among remaining operations, and an acyclic and natural relation $vis'$. So $\pi'$ is a legal abstract execution. 

% Second, the query cluster only has one dictated query operation and some dictating update operations. 
% This dictated query operation has the same operation context, i.e., the same arbitration and visibility relations of the dictating update operations. The return value of the dictated query operation is only affected by dictating update operations. As a result, the query operation in $\pi'$ has the same return value with the corresponding operation in $\pi$, which satisfies the semantics constraint of the consistency model. 

% 第三点证明有两个可替换的版本

% Third, the abstract execution $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 
% As we construct the abstract execution by operation, the visibility relation of the first $k-1$ operations is fixed when we choose the visibility of the $k$-th operation $o_k$. 
% We define a set $\mathcal{V}_k$ consisting of operations that is visible to the $k$-th operation. 
% We extend the abstract execution $\ang{lin_{k-1}, vis_{k-1}}$ to $\ang{lin_{k}, vis_{k}}$ by adding 
% $\mathcal{V}_k$ to $vis_{k-1}$ and adding $o_k$ to the end of $lin_{k}$. 

% We define a function $\mathcal{G}$ mapping a tuple $(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k)$ to a set $\mathcal{M}$. 
% The set $\mathcal{M}$ is the visibility relation that describles what $o_k$ must see according to the visibility constraint of the consistency model. If $\mathcal{M} \subseteq \mathcal{V}_k$, $\mathcal{V}_k$ is a legal visibility extension for the consistency model $\Phi$. 
% For example, we list some function $\mathcal{G}$ according to the visibility predicates in \ref{SubSec: Vis-Relax}, 
% \begin{itemize}
%     \item $\mathcal{G}_{weak} = \emptyset$, which has no constraint for visibility. 
%     \item $\mathcal{G}_{basic}(\_, \_, o_k) = \{(x, o_k)\ \vert\ \forall x: (x, o_k) \in so \}$, which means $o_k$ must see all the operations that happens before it according to the session order. 
%     \item $\mathcal{G}_{monotonic}(\ang{lin_{k-1}, vis_{k-1}}, \_, o_k) = \{(x, o_k)\ \vert\ \forall x \exists y : (y, o_k) \in so \land (x, y) \in vis_{k-1}\}$, which means $o_k$ must see the operations that its predecessors see. For the sake of simplicity, each operation is visible to itself. 
%     \item $\mathcal{G}_{causal}(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k) =  \{(x, o_k)\ \vert\ \forall x :(x, o_k) \in (vis_{k-1} \bigcup \mathcal{V}_k)^{+}\} \bigcup \mathcal{G}_{basic}(\_, \_, o_k)$, which means $o_k$ must see operations visible to those $o_k$ sees, and the visibility is a transitive closure. 
% \end{itemize}

% The set $\mathcal{R}$ contains relation pairs in the abstract execution $\pi$ but not in the projection $\pi$. 
% $\mathcal{V}_{k'}$ is the visibility relation that describles operations visible to the $k$-th operation in $\pi$, i.e. the $k'$-th operation in $\pi'$ after projection.  
% All relation pairs in $\mathcal{R}$ are removed from $\mathcal{V}_k$ after projection, so $\mathcal{V}_{k'} = \mathcal{V}_k \setminus \mathcal{R}$. 
% Also operations in $\mathcal{R}$ are removed from $\mathcal{M}$ after projection. Considering the transitivity, some operations cannot see another operation via removed operations in $\mathcal{R}$ any more, 
% \begin{equation*}
%     \begin{split}
%         &\mathcal{M}' = \mathcal{G}(\ang{lin_{k'-1}, vis_{k'-1}}, \mathcal{V}_{k'}, o_{k'}) \\
%         &\subseteq \mathcal{G}(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k) \setminus \mathcal{R} = \mathcal{M} \setminus \mathcal{R}.
%     \end{split}
% \end{equation*} 

% As the original abstract execution $\pi$ satisfies the visibility constraint of the consistency model $\Phi$, we can conclude that
% $\mathcal{M} \subseteq \mathcal{V}_k$ and further deduce that $\mathcal{M} \setminus \mathcal{R} \subseteq \mathcal{V}_k \setminus \mathcal{R}$. 
% Combining the transitivity of $\subseteq$, we can conclude that 
% $\mathcal{M}' \subseteq \mathcal{V}_{k'}$. 
% Therefore, the projection $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 

% To sum up above three points, the projection $\pi'$ satisfies the consistency model $\Phi$. 
% \end{tbm}

% \color{red}
% Third, we want to prove that the abstract execution $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 
% To simplify the question, we first prove that if only one operation is discarded from the abstract execution $\pi$ via projection, $\pi'$ still satisfies the visibility constraint. Then we can decompose a projection into a series of projections, and each projection only discards one operation from the previous abstract execution. 

% Next, we discuss six visibility levels by case. 
% \begin{itemize}
%     \item \textit{Weak} visibility permits any observations made by an operation, so the projection never violate the visibility constraint. 
%     \item \textit{Basic} visibility requires that operations observe all operations which happen before them. The visibility of each operation in the original abstract execution must already contains all its the predecessors. Since the discarded operation cannot be the predecessor of some operation any more. the projection of abstract execution still satisfies the visibility constraint. 
%     \item The proof of \textit{monotonic} visibility is similar to the \textit{basic} visibility. The discarded operation cannot be visible to some operation, so the projected visibility of each operation still contains all operations visible to its predecessors. 
%     \item \textit{Peer} visibility requires each operation to see the predecessors of those operation visible to it. The discarded operation cannot be the predecessor of some operation any more, so the projected visibility of each operation still contains all the predecessors of those operation visible to it. 
%     \item \textit{Causal} visibility requires each operation to see what operations visible to it see. Considering the transitivity, some operations cannot see another operation via the discarded operations any more. The transitive closure of the visibility relation is the subset of the original one. After projection only one operation is discarded from the visibility of each operation, $\pi'$ still satisfies the visibility constraint. 
%     \item The proof of \textit{complete} visibility is similar to the \textit{basic} visibility. The discarded operation cannot be linearized before some operation any more. 
% \end{itemize}

% Therefore, the projection $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 

% To sum up above three points, the projection $\pi'$ satisfies the consistency model $\Phi$. 

% As we construct the abstract execution by operation, the visibility relation of the first $k-1$ operations is fixed when we choose the visibility of the $k$-th operation $o_k$. The visibility extension of the $k$-th operation does not effect whether the previous operations satisfy the visibility constraint. So if the visibility of the $o_1, o_2, \ldots, o_m$ in the projection $\pi'$ satisfies the visibility constraint, 


% Because the visibility relation in $\pi'$ is a subset of the visibility relation in $\pi$. Thus the visibility in $\pi'$ is stronger, in the sense that in the projection $\pi'$, the operations miss (i.e., cannot see) less operations in the subhistory. In contrast, the operations in $\pi$ miss more operations, considering the whole abstract execution.
% We thoroughly check each of the six consistency models (defined in Section \ref{SubSec: Vis-Relax}) and show that the satisfaction of each consistency model still holds after the projection (this detailed checking process only involves low-level details and is omitted in our proof).

% As the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each abstract execution $\pi'$ must satisfy predicate $P$. 
% %So $\pi'$ adheres to the filter $R$ and violates the filter $R$ at the same time. 
% This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
% %would result in a contradiction. 
% Therefore, the pruning in \vs is safe. The candidate executions discarded can never be extended to a valid certificate abstract execution.

%--------------------------------------------------------------------------------
\subsection{Parallelization of \vs}

All legal search states of a history are organized as a tree, as shown in Figure \ref{F: Parallel}. 
Each search state is a node in the tree, and the root node is the empty abstract execution $\ang{lin_0, vis_0}$.
For a node $\ang{lin, vis}$ in the tree, search states which are possible extensions of $\ang{lin, vis}$ in the next phase are the children of $\ang{lin, vis}$. 
%Conversely, $\ang{lin, vis}$ is the parent of all search states which are possible growth of it in one phase. 
There may exist many candidate extensions in one phase, different choices of extensions result in the search of different subtrees. %split into different branches of the tree. 

%--
\begin{figure}[htb]
    \includegraphics[width=0.9\linewidth]{figures/p_tree.jpg}
    \centering
    \caption{Parallel \vs}
    \label{F: Parallel}
\end{figure}


%\slt{因为是树所以可以无脑并行}

%The tree has a recursive structure. 
%A tree consists of a root, and zero or more subtrees $T_1, T_2, \ldots , T_k$, and the root of each subtree is the child node of root of the tree. 
The procedure of consistency checking in \vs is like a depth-first search in tree whose goal is to find a leaf node corresponding to a search state that constructs a certificate abstract execution.
Therefore, there exists natural parallelization for the search. 
Subtrees do not share any nodes and are independent of each other. So we can search the subtrees in parallel. 
If we find a certificate abstract execution in any subtree, we terminate tasks in other subtrees and the history satisfies the consistency model. 
If no subtrees can find certificate executions, the history does not satisfy the consistency model. 

%\slt{提出了并行优化}

%We devise parallel optimization to accelerate {\vs} called parallel {\vs}. 
%With parallelization, we can check the consistency of a history using multi-threading, which better utilizes the compute resources and improves checking speed. 
\begin{tbm}
At the beginning of the parallel \textsc{ViSearch}, we first run the sequential \vs algorithm in a breadth-first search way, and generate a batch of search states. 
The search states are evenly allocated to different threads. Then each thread runs an instance of the sequential \vs algorithm in a depth-first search way to continue the search from each search state allocated to it. 
Note that here we use the term "thread" in a broader sense. The thread is more like an abstract worker. It can also be, for example, a virtual or physical machine.
See the example in Figure \ref{F: Parallel}. We generate four search states (the root node of each subtree in the dashed box). 
Each of the four states is allocated to a thread. The four threads extend the search states in parallel and obtain four different subtrees (the colored subtrees in four dashed boxes).
\end{tbm}

\begin{tbm}
Since the search states are divided randomly to different threads, it may lead to imbalanced load. 
We design a simple but useful dynamic load balancing mechanism, which thanks to the transformation from recursive to non-recursive. 
Because we need to adjust the load of each thread according to the runtime execution. 
Since the search states are maintained in a deque which is manipulated by algorithm, we can easily fetch search states from one thread's deque and add to another thread's to balance the load between two threads. 
If we use a recursive algorithm where search states are stored in the stack of operating system, we can hardly change the execution flow of the checking algorithm. 

We implement a search coordinator to maintain the meta information of parallel search, including the number of idle threads and working threads. 
When the the parallel \vs starts, the number of idle threads is set as zero.  
If a thread has finished its load, it returns the search result to the coordinator. 
The coordinator will increase the number of idle threads, if the thread do not find a certificate execution. 
Otherwise, the coordinator will stop all working threads and return \textsf{TRUE}. 

To avoid overloading and starvation, every working thread checks the number of idle threads at frequent intervals. 
If the number of idle threads is more than 0, the working thread will try to acquire the mutex of the coordinator, and share half of search states in its deque with an idle thread. 
The reason why we choose this mechanism is that interrupting a running thread is more complex than regular self-examination of running threads. 

The interval of self-examination is also important. 
Idle threads will starve for a long time if the interval is too large. 
And working threads will spend too much time on competing for the mutex of coordinator if the interval is too small. 
We set the interval 1000 search states, which means working threads stop to check whether there exists idle threads every 1000 search states checked. 
According to our experience, most of time-consuming checkings need to checking over 10,000 search states, and 1000-search-state interval is an appropriate portion. 
We also add a 10\% random disturbance in order to avoid too many working threads acquiring the mutex of the coordinator at the same time. 
\end{tbm}


%\slt{结合伪代码讲一下}

%The parallel {\vs} algorithm is presented in Algorithm \ref{A: PVS}. 
%The algorithm generates initial states at first, which are search states with a certain number of operations. 
%We can easily implement the method \textsf{generateInitialStates} by revising the centralized \vs algorithm (Algorithm \ref{A: VS}). 
%We replace the stack in line 1 with a queue, and let the algorithm return all search states in the queue when the size of queue exceeds a certain number. 
%As the number of the initial states is not exactly equal to the number of threads, 
%the initial states are divided into k parts for each thread, where k is the number of threads. 
%
%After that, we start {\vs} in parallel, and each thread carries out a {\vs} task. 
%When a thread exits, we examine the result of this {\vs} task. 
%If this {\vs} task returns \textsf{TRUE}, the algorithm will stop other running threads and return \textsf{TRUE}. 
%If this {\vs} task returns \textsf{FALSE}, the algorithm will increase a counter which records how many {\vs} tasks have returned \textsf{FALSE}. 
%The algorithm returns \textsf{FALSE} if all {\vs} tasks return \textsf{FALSE}. 


%\slt{分析一下优化效果}

%Theoretically, the checking time of the parallel search can be reduced to the $\frac{1}{k}$ of that of the sequential search, where $k$ is the number of threads. 
%Because, parallel {\vs} checks $k$ times of search states as the single-threaded {\vs} checks in the same amount of time. 
%In other words, the checking time can be ideally reduced to $\frac{1}{k}$ of the original. 
%However in practice, the search of one subtree may cost significantly more time than the search of another subtree. It is because different subtrees mean different linearizations of the operations, and the possible visibility relations to be checked for different linearizations may vary quite a lot.
%This means that there may be some threads are overloaded while some threads starve. Thus the parallel search cost is often more than $\frac{1}{k}$ of the sequential search cost.
%How to analyze the search states and evenly allocate workload among the threads is left to future work.

%--
% \begin{algorithm}[ht]
%     \caption{Parallel \vs}
%     \label{A: PVS}
%     \SetKwBlock{DoParallel}{do in parallel}{end}
%     \KwIn{history $\mathcal{H}$, 
%         data type implementation \textit{Impl}, 
%         consistency model $\Phi$}
%     \KwOut{whether history $\mathcal{H}$ satisfies the given consistency model $\Phi$}
%     $\mathcal{I}$ $\leftarrow$ \textsf{generateInitialStates}()\\
%     Divide $\mathcal{I}$ into $\mathcal{I}_1, \mathcal{I}_2, \ldots, \mathcal{I}_k$\\
%     \DoParallel{
%         Visearch Checking with initial states $\mathcal{I}_1$\\
%         Visearch Checking with initial states $\mathcal{I}_2$\\
%         $\cdots$\\
%         Visearch Checking with initial states $\mathcal{I}_k$\\
%     }
% \end{algorithm}

==> ViSearch_complete_version/newcommands.tex <==
% newcommands.tex

% math
\newcommand{\set}[1]{\{#1\}}
\newcommand{\argmax}{\operatorname{arg\,max}}
\newcommand{\tord}[1]{\textsl{to}(#1)}

\newcommand{\mongodb}{MongoDB}
\newcommand{\mongodbcc}{\textsl{MongoDB-CC}}
\newcommand{\gentlerain}{\textsl{GentleRain}}

% color
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\teal}[1]{\textcolor{teal}{#1}}

% specification
\newcommand{\op}{\texttt{op}}
\newcommand{\rval}{\texttt{rval}}
\newcommand{\prel}{\texttt{rel}}

% FIFO queue
\newcommand{\intfq}{\textsf{fq}}
\newcommand{\fq}{\text{FIFO queue}}
\newcommand{\enq}{\texttt{enq}}
\newcommand{\deq}{\texttt{deq}}

% register
\newcommand{\intreg}{\textsf{reg}}
\newcommand{\rd}{\texttt{rd}}
\renewcommand{\wr}{\texttt{wr}}

% key-value
\newcommand{\kv}{\textsf{kv}}
\newcommand{\kvput}{\texttt{put}}
\newcommand{\kvget}{\texttt{get}}

% protocol
\newcommand{\compare}{\textsc{compare}}
\newcommand{\merge}{\textsc{merge}}
\newcommand{\get}{\textsc{get}}
\newcommand{\pput}{\textsc{put}}
\newcommand{\ok}{\textsf{ok}}
\newcommand{\store}{\textsf{store}}
\newcommand{\tick}{\textsc{tick}}
\newcommand{\replicate}{\textsc{replicate}}

% GentleRain
\newcommand{\getreq}{\textsc{get-request}}
\newcommand{\getreply}{\textsc{get-reply}}
\newcommand{\putreq}{\textsc{put-request}}
\newcommand{\putreply}{\textsc{put-reply}}
\newcommand{\partition}{\textsc{partition}}
\newcommand{\vc}{\texttt{vc}}
\newcommand{\version}{\texttt{ver}}

% algorithm
\newcommand{\send}{{\bf send}\;}
\newcommand{\receive}{{\bf receive}\;}

\newcommand{\sr}{\texttt{sr}}

\newcommand{\queryreq}{\textsc{get-request}}
\newcommand{\updatereq}{\textsc{put-request}}
\newcommand{\pulloplog}{\textsc{pull-oplog}}

\newcommand{\client}{\textsl{Client}}
\newcommand{\server}{\textsl{Server}}

\newcommand{\ct}{\textsf{ct}}
\newcommand{\ot}{\textsf{ot}}
\newcommand{\aot}{\textsf{aot}}
\newcommand{\clock}{\textsf{clock}}
\newcommand{\hlc}{\textsl{hlc}}

\newcommand{\primary}{\textsc{primary}}
\newcommand{\isPrimary}{\textsc{IsPrimary}}
\newcommand{\isSecondary}{\textsc{IsSecondary}}
\newcommand{\rs}{\textsc{Cluster}}

\newcommand{\oplog}{\textsf{oplog}}
\newcommand{\syncsource}{\textsc{SyncSrc}}

\newcommand{\noopwrite}{\textsc{Noop}}
\newcommand{\noop}{\textsc{no-op}}

% rdt
\newcommand{\Obj}{\textsl{Obj}}
\newcommand{\Val}{\textsl{Val}}
\newcommand{\Type}{\textsl{Type}}
\newcommand{\Op}{\textsl{Op}}

\newcommand{\eval}{\texttt{eval}}

% concrete execution
\newcommand{\eo}{\texttt{eo}}
\newcommand{\ret}{\texttt{ret}}

% abstract execution
\newcommand{\vis}{\texttt{vis}}
\newcommand{\ar}{\texttt{ar}}
\newcommand{\nar}{\texttt{ar'}}
\newcommand{\fv}{\texttt{V}}
\renewcommand{\v}{\texttt{v}}

% arrows for relations
\newcommand{\rel}[1]{\xrightarrow{#1}}

% proof
\renewcommand{\so}{\texttt{so}}
\newcommand{\po}{\texttt{po}}
\newcommand{\hb}{\texttt{hb}}
\newcommand{\rf}{\texttt{rf}}
\newcommand{\ts}{\texttt{ts}}
\newcommand{\request}{\texttt{request}}

% kvs
\newcommand{\key}{\texttt{k}}
\newcommand{\ut}{\texttt{ut}}
\newcommand{\dt}{\texttt{dt}}
\newcommand{\gst}{\texttt{gst}}
\newcommand{\kvs}{\textsf{kvs}}
\newcommand{\fkvs}{\mathcal{F}}
\newcommand{\f}{\mathcal{F}}

% consistency
\newcommand{\ctxt}{\texttt{ctxt}}
\newcommand{\oc}{\textsl{Ctxt}}
\newcommand{\context}{\mathbb{C}}
\newcommand{\retval}{\textsc{RVal}}
\newcommand{\cc}{\textsc{CausalConsistency}}
\newcommand{\cv}{\textsc{CausalVisibility}}
\newcommand{\ca}{\textsc{CausalArbitration}}
\newcommand{\ev}{\textsl{EV}}

% sc
\renewcommand{\sc}{\textsl{SC}}

% cc
\newcommand{\wcc}{\textsl{WCC}}
\newcommand{\wccv}{\textsl{WCCv}}
\newcommand{\cm}{\textsl{CM}}
\newcommand{\cmv}{\textsl{CMv}}
\newcommand{\ccc}{\texttt{CC}}
\newcommand{\ccv}{\texttt{CCv}}
\newcommand{\scc}{\textsl{SCC}}
\newcommand{\sccv}{\textsl{SCCv}}

% pc
\newcommand{\wpc}{\textsl{WPC}}
\newcommand{\pc}{\textsl{PC}}
\newcommand{\wpcv}{\textsl{WPCv}}
\newcommand{\pcv}{\textsl{PCv}}
\newcommand{\pram}{\textsl{PRAM}}
\newcommand{\suc}{\textsl{SUC}}
\newcommand{\uc}{\textsl{UC}}

% comments
\newcommand{\hfwei}{\red{hfwei:\;}}
\newcommand{\xj}{\blue{xj:\;}}


==> ViSearch_complete_version/preamble.tex <==
% preamble.tex

%== == == == == packages

% \usepackage{fontspec}
% \setmainfont{Times New Roman}
% \usepackage{xeCJK}

%--
\usepackage{CJK}
\usepackage[a-1b]{pdfx}

% \usepackage{CJKutf8}
% \usepackage{ctex}
% \usepackage{xcolor} % delete this finally
% \usepackage{paralist}
% \usepackage{cite}

% \usepackage{soul} % delete this finally
% \setstcolor{red}

% page numbering
%\usepackage{fancyhdr}
%\pagestyle{plain}
%\pagenumbering{arabic}

% math
% \usepackage{amsmath, amssymb, amsthm}

% theorems
% \theoremstyle{definition}
% \newtheorem{recipe}{Recipe}

% \theoremstyle{definition}
% \newtheorem{example}{Example}

\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{proofstretch}{Proof Stretch}

% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}

% \newtheorem*{remark}{Remark}

% \usepackage{algorithm}
% \usepackage[noend]{algpseudocode}
% \newcommand{\hStatex}[0]{\vspace{5pt}}
% \UseRawInputEncoding
\usepackage{balance}
\usepackage{multirow}
\usepackage{colortbl}
\usepackage{subfigure}
% \usepackage[table,xcdraw]{xcolor}

\usepackage[ruled,linesnumbered]{algorithm2e}

% figure
% \usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{float}

% table
\usepackage{multirow}
\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

% \usepackage{floatrow}
% \floatsetup[table]{capposition=top}

% \input{newcommands}

%--
% \renewcommand{\baselinestretch}{1.1}


%== == == == == commands

%-- for editing
\newcommand{\mypar}[1]{\vspace{0.5cm} \noindent 【#1】}
\newcommand{\mybreak}{\vspace{0.5cm}}

%-- -- colors
\newcommand{\cyan}{\color{cyan}}
\newcommand{\blk}{\color{black}}
\newcommand{\gray}{\color{gray}}

%-- -- for comments
\newcommand{\slt}[1]{\noindent \textcolor{red}{\noindent \large \bf #1}}
\newcommand{\hy}[1]{\noindent \textcolor{cyan}{\noindent \large #1}}

%-- -- formats
% \setlength\emergencystretch{\hsize}


%-- abbreviations, names
\newcommand{\vs}{\textsc{ViSearch}\ }
\newcommand{\visar}{\textsc{Vis-Ar}\ }
\newcommand{\rwf}{\textsc{Rwf}\ }
\newcommand{\rwfset}{\textsc{Rwf}-set}
\newcommand{\rwfrpq}{\textsc{Rwf}-rpq}

%-- math
\newcommand{\ang}[1]{\langle #1 \rangle}
\newcommand{\mydef}{\stackrel{\triangle}{=}}

%\newcommand{\rulearb}{\textsf{Tmpl$_{\text{\scriptsize ARB}}$}\ }
\newcommand{\tarb}{\mathcal{T}_{\text{\scriptsize ARB}}}
\newcommand{\tvis}{\mathcal{T}_{\text{\scriptsize VIS}}}
\newcommand{\tnotvis}{\mathcal{T}_{\text{\scriptsize NOT-VIS}}}
%\newcommand{\rulevis}{\textsf{Rule$_{\text{\scriptsize VIS}}$}\ }
%\newcommand{\rulenotvis}{\textsf{Rule$_{\text{\scriptsize NOT-VIS}}$}\ }

% edit
\newenvironment{tbm}{\color{blue}}{}






==> maintext_backup/abs.tex <==
%--
\begin{abstract}

    Large-scale replicated data type stores often resort to eventual consistency to guarantee low latency and high availability. It is widely accepted that programming over eventually consistent data stores is challenging, since arbitrary divergence among replicas is allowed. Moreover, pragmatic protocols actually achieve consistency guarantees stronger than eventual consistency, which can be and need to be utilized to facilitate the reasoning of and programming over replicated data types.
    Toward the challenges above, we propose the \vs framework for precise measurement of eventual consistency semantics.
    \vs employs the visibility-arbitration specification methodology in concurrent programming, which extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happen-before and linearization relations. 
    The consistency measurement using \vs is NP-hard in general. To enable practical and efficient consistency measurement in replicated data type stores, the \vs framework refactors the existing brute-force checking algorithm to a generic algorithm skeleton, which further enables efficient pruning of the search space and effective parallelization.
    We employ the \vs framework for consistency measurement in two replicated data type stores Riak and CRDT-Redis. The experimental evaluation shows the usefulness and cost-effectiveness of consistency measurement based on the \vs framework in realistic scenarios.    

\end{abstract}

==> maintext_backup/concl.tex <==
%--
\section{Conclusion and Future Work} \label{Sec: Concl}

In this work, we develop the \vs framework for consistency measurement of replicated data type stores. In our framework, different consistency levels are specified via the relaxation of the visibility relations among operations.
The measurement of data consistency is based on the \vs algorithm skeleton, which enables efficient pruning of the search space and effective parallelization.
We employ the \vs framework for consistency measurement in two replicated data type stores Riak and CRDT-Redis. The experimental evaluation shows the usefulness and cost-effectiveness of consistency measurement based on the \vs framework in realistic scenarios.

In our future work, we will investigate how to propose more predicate templates and extract efficient pruning predicates to further reduce the consistency measurement cost. 
Moreover, efficient heuristics can be employed to reduce the search cost.
%We also need to explore load balancing techniques for the parallel \vs algorithm.
Besides improvements on the \vs framework itself, we will conduct more case studies of realistic replicated data type stores and investigate whether knowledge of the specific data type store can be effectively utilized to reduce the consistency measurement cost using \textsc{ViSearch}.

==> maintext_backup/exp.tex <==
%--
\section{Experimental Evaluation} \label{Sec: Exp}

\begin{tbm}
    In this section, we apply the \vs framework for consistency measurement in two realistic replicated data stores in order to answer two main questions. One is that whether the \vs framework can measure out the subtle difference between different replicated data types. 
    The other one is how efficient the \vs framework is. 
\end{tbm}

We first present our experiment setup and design. Then we discuss the evaluation results.

The implementation of the \vs framework, as well as implementations, configurations and experiment scripts over the two replicated data type stores are available on the github \footnote{https://github.com/ViSearch/ViSearch}.

%--------------------------------------------------------------------------------
\subsection{Experiment Setup}

\begin{tbm}
We employ \vs to measure consistency for Riak \cite{Riak} and CRDT-Redis \cite{CRDT-Redis}. 
Riak is a distributed NoSQL key-value database, which provides Riak-specific data types based on CRDTs. 
CRDT-Redis revises Redis, a popular in-memory data structure store with built-in replication, into a multi-master architecture and supports CRDT-based conflict resolution for concurrent updates on multiple master nodes. 

We choose data types for experiments from two perspectives. The first perspective is the semantics of data type, in other words the interface exposed to users. 
We select three widely-used containers, \textit{set}, \textit{map}, and \textit{priority queue}, which are are representative and cover a range of data type semantics. 
Among them, \textit{set} is supported by both Riak and CRDT-Redis. \textit{Map} is only supported by Riak while \textit{priority queue} is only supported by CRDT-Redis. 
Riak and CRDT-Redis also support other data types like register, counter, and hyperloglog, but we think register and counter have too simple semantics, and hyperloglog seems like a probability algorithm rather than a traditional data structure. 

However, different implementations of the same data structure vary from each other. For example, the JDK provides LinkedList and ArrayList which both implement List interface, but they have different performance. 
Similarly, distributed data storage provides replicated data types with the same interface but different implementations. 
The second perspective is the implementation of data type, including different configurations and different conflict resolutions. 

Riak exposes a parameter $r$ to the clients, which denotes how many replicas a query request must contact. Contacting more replicas before returning a query request reduces the data inconsistency but increases the query delay.
The two data types with different parameters $r$ $(r=1$ or $r=2$) are denoted \textit{Set-r1}, \textit{Set-r2}, \textit{Map-r1} and \textit{Map-r2} in our experiment. 
Each data type in CRDT-Redis is designed with different conflict-resolution strategies: add-win (\textit{A} in short), remove-win (\textit{R} in short), and the \rwf framework (\textit{F} in short) \cite{Zhang21}. 
Data types with different conflict-resolve strategies are denoted \textit{Set-A}, \textit{Set-R}, \textit{Set-F}, \textit{PQ-A}, \textit{PQ-R}, and \textit{PQ-F}. 
All of our experiments is conducted on these ten data types, which combines high-level semantics and concrete implementations up. 
\end{tbm}

%% We study two widely-used container types \textit{Riak-set} and \textit{Riak-map}. Riak exposes a parameter $r$ to the clients, which denotes how many replicas a query request must contact. Contacting more replicas before returning a query request reduces the data inconsistency but increases the query delay.
%To match application needs, Riak KV enables users to trade off between data consistency and availability by adjusting replication configuration. 
%There exists wide and varied replication parameters available in Riak KV, and we focus on the number of servers that must respond to a read request(denoted as \textit{r}), which is concerned with the conflict-resolve strategy of Riak-specific data types. 
%Users can archieve higher accuracy by choosing higher values for \textit{r}, while higher values will also entail degraded responsiveness. 
%% The two data types with different parameters $r$ $(r=1$ or $r=2$) are denoted \textit{Set-r1}, \textit{Set-r2}, \textit{Map-r1} and \textit{Map-r2} in our experiment. 

%We experiment on Riak-specific data types with parameter \textit{r}=1, and 2 (3 replicas in total), marked as \textit{Set-r1}, \textit{Set-r2}, \textit{Map-r1}, and \textit{Map-r2}. 



%% CRDT-Redis currently provides two container types \textit{Redis-set} and \textit{Redis-priority-queue} (\textit{Redis-PQ} in short).


We run both distributed data stores in the Alibaba Cloud Elastic Compute Service (ECS) \cite{Alibaba-Cloud}. Each ECS server has two Intel Xeon Platinum CPU (2.50GHz), 4GB RAM, 40GB ESSD and 1MB/s network bandwidth. We build a Riak cluster with 5 servers, and replicate data types on 3 servers in the cluster. The CRDT-Redis cluster consists of 3 servers, and data types are replicated on all 3 servers. Another ECS server is dedicated to running clients. 

The checking of data type access traces using \vs is conducted on one workstation with an Intel i9-9900X CPU (3.50GHz), with 10 cores and 20 threads, and 32GB RAM, running Ubuntu Desktop 16.04.6 LTS.

The basic workflow of consistency measurement using \vs is shown in Figure \ref{F: Exp}.
We first generate the workloads for each data type. The workload module basically tells the clients what queries to send to the data store and when to issue the queries. %???
%The clients send queries to the data store as instructed by the workload module and wait for the reply. 
The clients record both the query invocation info (e.g., API name and arguments) and the return values (e.g., the value returned by a query request and the ACK returned by an update request) for all queries issued.
All the info of data type access collected by the clients in one experiment form one trace or history of data type access. 
Multiple traces of data type access are imported into the \vs module and \vs tells us the consistency levels of the traces measured, e.g., Co (complete visibility) or M (monotonic visibility). Detailed definitions of the consistency levels can be found in Section \ref{SubSec: Vis-Relax}.

% 单个client收集的叫info
% 所有client一起访问一个type，收集的叫一个trace，或者一个history。
% 一个实验，多次收集traces或者说histories。
% 这里，等于是把trace和history当成同义词。

%--
\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/exp.jpg}
    \caption{\vs workflow.}
    \label{F: Exp}
\end{figure}


%\mybreak

%\slt{为了获得全面的trace，需要做的工作}


%--------------------------------------------------------------------------------
\subsection{Experiment Design}

The optimized trace checking using \vs (as detailed in Section \ref{Sec: VS}) still requires exponential time in the worst case. Thus we cannot directly apply \vs over CRDT access traces of arbitrary length. As inspired by the measurement in \cite{Emmi19}, we explore locality in consistency measurement over CRDT traces to circumvent the NP-hardness obstacle.

As for a CRDT, any replica can be modified without coordination with other replicas. Thus the replicas  may temporarily diverge. 
When all updates are delivered to the replicas, possibly in different orders, the replicas converge, as required by the definition of eventual consistency \cite{Shapiro11a}.
We call the period when the replicas diverge the \textit{divergence interval}. 

Our key observation for consistency measurement of real data type access traces is that, the consistency level of given trace is decided by the divergence intervals in the trace. Thus we only need to measure the divergence intervals in the trace, instead of measuring the whole trace of arbitrary length. The consistency level of the whole trace is decided by the divergence interval of the weakest consistency level.

We can estimate the divergence interval by monitoring the communication channel. According to the definition of eventual consistency, the replicas only diverge when the updates are still in transmission. 
We estimate the maximum extent of divergence by monitoring how large the number of updates in transmission can be, during the experiment.

We reproduce the experiments in our previous work on CRDT design based on CRDT-Redis \cite{Zhang21}.
We set 1000 checkpoints for the replicas in the experiments where there are about 100,000 operations in the workload and the number of operations per second is bounded by 3000.
We find that the number of operations in transmission is bounded by 15. %, when the throughput is bounded by 3000 operations per second. 
Therefore in our experiment, we set the size of the workload, i.e., the number of operations to be sent to the data type, to 15. We let the clients launch the operations as quickly as possible to produce the maximal divergence.
Note that the specific value of the divergence interval is not essential in our experiment. In different experiment scenarios, we can estimate the divergence interval in the same way. Generally speaking, the more the throughput of the data type store, the larger the divergence interval.

\begin{tbm}
To obtain comprehensive and typical data type access traces, we generate a wide range of workloads. 
To avoid any bias and human factor in the collection of traces, we fill workloads with randomly-generated methods with randomly-generated arguments. 
As discussed above, each workload contains about 15$\sim$17 operations and 3$\sim$5 client threads shares the operations in a workload. 

In detail, we randomly choose arguments of operations from a small space. 
The space is usually set as 0$\sim$5, which is no more than 1/3 of the workload size. 
This ensures that there exists many collisions with operations, i.e. conflict operations invoked at the same element, since we generate sufficient workloads and execute workloads sufficient times. 
In our workloads, about 60\% operations are \textit{update}, and about 40\% operations are \textit{query}. 
For example, there are 40\% \textit{add} operations, 20\% remove operations, 20\% \textit{contains}, and 20\% \textit{size} operations in workloads for data type \textit{set} in CRDT-Redis. 
\end{tbm}

%According to experience and others' work, most of inconsistent behaviours can be exposed by several operations across two or three threads. 
%As long as there are sufficient executions, we can catch all these inconsistent behaviours with high probability. 
%On the other hand, we have to restrict the size of a single program to avoid combinatorial explosion in consistency checking. 

%The arguments are generated from a certain range to ensure that there exists collisions with operations invoked on the same elements concurrently. 
%For example, in the experiment of set, we make the range of elements small so that there might be more \textit{add} and \textit{remove} invoked on the same elements concurrently. 

\begin{tbm}
Though we try to generate comprehensive and typical traces, the final result of the measurement is still an approximation of the consistency level but not a guarantee. 
Because our finite workloads cannot exhaust all possible executions of a replicated data type, unless we make a strict proof or do model checking on these data types. 

To ensure accuracy, we measure the consistency level of a certain data type by round. 
Every round we generate workloads randomly and obtain 100K data type access traces. 
According to our experience, 100K traces is large enough to construct all corner cases in the CRDT design and cover the various cases in the conflict resolution. 
Then the \vs framework measures the consistency level of each trace, and the weakest consistency level measured over all these 100K traces is the measurement result in this round. 
The final measurement result will be updated if the measurement result of the current round is weaker than it. 
We repeat above procedure, and terminate when at least 3 rounds have been finish and the final measurement result keeps unchanged in the last two consecutive rounds. 

We believe that our measurement over a sufficiently large number of workloads is a cost-effective and accurate enough approach to obtaining the precise consistency semantics of one replicated data type. 
\end{tbm}

% In our experiment, we randomly generate 400,000 workloads for each data type. According to our experience in testing CRDT implementations, the workload of 15 operations is sufficient for constructing all corner cases in the CRDT design, and 400,000 workloads are sufficient to cover the various cases in the conflict resolution \cite{Zhang21}. 
% The  weakest consistency level measured over all the workloads is approximately the actual consistency level the data type provides. 
% Since it is usually quite difficult to strictly prove the consistency level certain CRDT design guarantees, we believe that our measurement over a sufficiently large number of workloads is a cost-effective and accurate enough approach to obtaining the precise consistency semantics of one replicated data type.

Given the workloads generated above, the main objective of the experimental evaluation is to answer the following two questions:
%--
\begin{itemize}
    \item[Q1.] Are the measurement results useful, for the developers to understand the consistency semantics a CRDT design actually provides?

    \item[Q2.] Can the consistency measurement be efficiently conducted with reasonable testing budget?
\end{itemize}

\noindent We discuss the evaluation results below in light of these two questions.

%--------------------------------------------------------------------------------
\subsection{Evaluation Results}

Based on the evaluation results, we first discuss what the application developers and CRDT designers can obtain from our consistency measurement. Then we study the time cost for the measurement. We also study the checking cost saved by the two optimization we develop, i.e., the pruning of search space and the parallelization of the checking process.

%----------------------------------------
\subsubsection{Consistency Measurement Results}

\begin{tbm}
We measure the consistency levels of 10 replicated data types from two data type stores. 
Due to different configurations and conflict resolutions, these replicated data types satisfy different consistency levels with high probability. 
If \vs can measure the consistency level precisely, the measurement results should spread on different consistency levels. 
\end{tbm}

The measurement results are listed in Table. \ref{T: Result}. %, and each row is the experiment result of a replicated data type.
Each row of the table corresponds to one data type.
For each of the 6 consistency levels, we list the number of violations found by \textsc{ViSearch}.
The strongest consistency level with 0 violation (colored gray in the table) is the consistency level of the data type.
The '/' means that the checking is unnecessary and the violation must be zero, since there are no violations for stronger consistency levels.

We demonstrate the usefulness of the consistency measurement results from the perspective of the "cosistency-latency tradeoff", which is a refinement of the widely used CAP theorem \cite{Brewer12, Gilbert12} and the PACELC tradeoff \cite{Abadi12} in CRDT scenarios.
Different CRDT designs and implementations principally have the same data update delay, since the replica is updated locally at once and the updates are propagated asynchronously. The query delay is also principally the same if the query only contacts one replica. In some data stores like Riak, the client can choose to contact multiple replicas, sacrificing certain query delay and improving the consistency level of the query.
Thus, from the perspective of the consistency-latency tradeoff, it is the consistency semantics of the data type which capture all the differences in CRDT designs and implementations.

In light of the discussions above, we study whether the consistency measurement results can tell the CRDT designers and application developers the essential differences in different data types in our experiment.
%In each store, the data type can adopt different implementations with different conflict resolution strategies. The data type can also have different configuration, e.g., $Set\text{-}r1$ and $Set\text{-}r2$. 
%
%The eventual consistency semantics cannot show the differences among different implementations and configurations. 
%Our consistency measurement using \vs show the different consistency semantics provided by different implementations and configurations.
%
Specifically, the consistency measurement of CRDT-Redis data types demonstrates the different consistency semantics resulting from different conflict resolution strategies.
%that Redis replicated data types with different conflict-resolve strategies vary in consistency level. 
The priority queue \textit{PQ-R} designed with the remove-win strategy merely provides the "Weak" consistency level, while the priority queue \textit{PQ-A} designed with the add-win strategy and \textit{PQ-F} designed with the \rwf framework both provide the stronger consistency level "Peer".
Moreover, the number of violations of the remove-win strategy is much larger than that of the other two strategies on the causal consistency level.
%The data type \textit{PQ-A} and \textit{PQ-F} satisfy the consistency level \textit{monotonic}, which guarantees the monotonic reads. 

Considering the high level design rationale, we may reasonably think that the remove-win strategy and the add-win strategy are dual of each other and are principally the same. However, the measurement by \vs show important difference in the consistency semantics. 
%Add-win and remove-win are dual strategies. However, applied to a complex data type like the priority queue, the consistency semantics are different.
%The consistency level resulting from the add-win strategy is stronger ("Peer"), while the remove-win strategy provides weaker consistency level ("Weak").
%Moreover, the violations of the remove-win strategy are significantly more than those of the add-win strategy.
The \rwf framework is an improvement on the traditional remove-win strategy. The remove-win strategy puts the remove operation behind the non-remove operation. In \textsc{RWF}, the remove-operation just removes the element from the container, thus avoiding the conflict. This \rwf strategy, seen as an improvement of the traditional remove-win strategy, strengthens the consistency semantics to the same level with the semantics of the add-win strategy.
%further utilize the potential of the remove-win strategy. It not only eases the development, but also provides stronger consistency semantics.
The consistency measurement results can help the CRDT designers to further understand the semantics of different resolution strategies. The application developers can also use the measurement results to choose appropriate data types they actually need.

The consistency measurement results of the set data type have important differences with those of the priority queue data type.
As for the add-win and \rwf resolution strategy, the consistency level of \textit{Set-A} and \textit{Set-F} is still "Peer", which is the same with the level of their counterparts \textit{PQ-A} and \textit{PQ-F}.
The main difference appears when considering the remove-win strategy. As for the set type, \textit{Set-R} also provides "Peer", while \textit{PQ-R} only provides "Weak".
The difference mainly results from that the priority queue has much more complex semantics than the set. When coping with complex semantics of the data type, the remove-win strategy will reduce the consistency semantics provided to the upper-layer applications. 
These measurement results show that the semantics of the data type should also be considered when choosing the conflict resolution strategies. 

%This measurement result can better instruct the applications developers to choose conflict resolution strategies. 
%The result can also help the CRDT designer better understand the cons and pros of each conflict resolution strategy and design more efficient strategies.

%Overall the data types designed with remove-win strategy generally provide weaker consistency than the ones designed with add-win strategy or the \rwf framework. 
%Moreover, we find that the data types designed with add-win strategy satisfy the same consistency level with the ones designed with the \rwf framework. 

%The findings are useful for designers and users of CRDTs. 
%Designers can choose a proper conflict-resolve strategy for data types, and users can minimize compensations to the inconsistency of data store during developing applications. 

As for the Riak case, the configuration of parameter $r$ plays the most important role in the consistency measurement. The effect of $r$ can be quantified by the consistency measurement based on \textsc{ViSearch}.
%The measurement result of Riak data types is easier to explain. 
%The parameters $r$ dominates the consistency level of different Riak data types. 
%Data types provide a stronger consistency when $r$ is larger. 
We find that both data types merely provide the "Weak" consistency level when $r=1$.
%In a high concurrency scenario, contacting only one replica before returning a query request guarantees a very weak data consistency. 
When $r=2$, a query request must contact a majority of replicas before returning. 
According to quorum-based protocol, data types with $r=2$ cannot strictly guarantee strong consistency. 
However, \textit{Set-r2} and \textit{Map-r2} actually provide strong consistency (the "Complete" consistency level) in the experiment.
The measurement results show that when the network condition is relatively reliable and the communication delay is low, e.g., in an intra-datacenter environment, the "$r=2$" configuration actually provides strong consistency, at least with high probability.
%because network condition is good in data center. 
This result is quite useful for applications which want strong consistency, but can tolerate data inconsistency in rare cases \cite{Wei17, Ouyang21}. The limited sacrifice in data consistency can greatly reduce the query delay.

%This measurement result may help Riak users a lot. 
%They can choose a small $r$ for lower latency without loss of consistency when network condition is good. 
%For subsequent improvements of Riak, the findings are also helpful. 

%\color{black}

%Though replicated data types are designed for eventual consistency, their behavior may actually adhere to stronger consistency models due to different client-server interaction modes and conflict resolution strategies, 
%and {\vs} can identify how much the consistency is strengthened.

%We will continue to measure consistency level across a wide range of replicated data types and consistency models. 
%We also try to increase the size of histories in the future, including more operations and concurrent threads. 

%--
\begin{table}[htb]
    \caption{Measurements for Data Types}
    \label{T: Result}
    \resizebox{\linewidth}{!}{  
        \begin{tabular}{|c|cccccc|l|l|}
            \hline
            & \multicolumn{6}{c|}{Violations}       &       &       \\ \cline{2-7}
            \multirow{-2}{*}{\begin{tabular}[c]{@{}c@{}}Data \\ Type\end{tabular}} & \multicolumn{1}{c|}{Co}            & \multicolumn{1}{c|}{Ca}       & \multicolumn{1}{c|}{P}        & \multicolumn{1}{c|}{M}        & \multicolumn{1}{c|}{B}        & W         & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}\# of \\ Histories\end{tabular}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}Total \\ Time\end{tabular}} \\ \hline
            \textit{Set-r1}     & \multicolumn{1}{c|}{366}                      & \multicolumn{1}{c|}{339}                      & \multicolumn{1}{c|}{334}                              & \multicolumn{1}{c|}{295}       & \multicolumn{1}{c|}{188}       & \cellcolor[gray]{.8}0     & 300k          & 8h 3min      \\ \hline
            \textit{Set-r2}     & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}    & \multicolumn{1}{c|}{/}                        & \multicolumn{1}{c|}{/}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 300k          & 0h 11min      \\ \hline
            \textit{Map-r1}     & \multicolumn{1}{c|}{788}                      & \multicolumn{1}{c|}{734}                      & \multicolumn{1}{c|}{732}                                & \multicolumn{1}{c|}{712}    & \multicolumn{1}{c|}{542}      & \cellcolor[gray]{.8}0     & 300k          & 24h 26min       \\ \hline         
            \textit{Map-r2}     & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}    & \multicolumn{1}{c|}{/}                        & \multicolumn{1}{c|}{/}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 300k          & 0h 11min      \\ \hline
            \textit{PQ-A}       & \multicolumn{1}{c|}{478}                      & \multicolumn{1}{c|}{3}                        & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}            & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                        & 300k          & 4h 49min       \\ \hline                
            \textit{PQ-R}       & \multicolumn{1}{c|}{704}                      & \multicolumn{1}{c|}{131}                        & \multicolumn{1}{c|}{130}            & \multicolumn{1}{c|}{119}        & \multicolumn{1}{c|}{119}        & \cellcolor[gray]{.8}0                        & 300k          & 14h 17min       \\ \hline                
            \textit{PQ-F}       & \multicolumn{1}{c|}{1153}                      & \multicolumn{1}{c|}{3}                        & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}            & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                        & 300k          & 0h 18min       \\ \hline                
            \textit{Set-A}      & \multicolumn{1}{c|}{45}                        & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 500k          & 0h 19min         \\ \hline                
            \textit{Set-R}      & \multicolumn{1}{c|}{15}                        & \multicolumn{1}{c|}{4}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 400k          & 8h 9min         \\ \hline                
            \textit{Set-F}      & \multicolumn{1}{c|}{5}                        & \multicolumn{1}{c|}{1}    & \multicolumn{1}{c|}{\cellcolor[gray]{.8}0}                                & \multicolumn{1}{c|}{/}        & \multicolumn{1}{c|}{/}        & /                         & 500k          & 0h 19min         \\ \hline                
    \end{tabular}}
\end{table}

%----------------------------------------
\subsubsection{Consistency Measurement Cost}

To obtain the consistency measurement results in Table \ref{T: Result}, the checking time of \vs varies from 11 minutes to 24 hours. 
The consistency measurement time varies significantly as for different data types. In our experiment three out of ten types, \textit{Set-r1}, \textit{Map-r1} and \textit{PQ-R}, require significantly more time that other data types. Thus for most data types, the number of traces checked can be increased to a much larger number (e.g., 1 million) in bounded time. 
The checking time results demonstrate that consistency measurement using \vs can be accomplished under reasonable testing budget.
Also note that, the measurement process is not on the critical path of CRDT design, implementation, testing and maintenance. It can "borrow" the traces from the testing process and be finished in parallel with testing of CRDT implementations.

%The results of measurement clearly demonstrate the efficiency of {\vs} checking framework, and the ability of measuring out different consistency model. 
%The {\vs} framework can check a large number of histories which satisfy different consistency models in an acceptable time. 

Besides the total checking time using \textsc{ViSearch}, we further study the effects of the optimizations we propose, namely the pruning of search space and the parallelization of checking.
\begin{tbm}
    We use the \vs without pruning and parallelization as our baseline. Considering that the \vs without any optimization is just a non-recursive version of the existing algorithm, we actually compare the effects of optimizations with the checking algorithm in \cite{Emmi18}. 
\end{tbm}

%----------------------------------------
%\subsubsection{Efficay of parallelization}

As for the parallelization of consistency measurement, we study two data types \textit{Set-r1} and \textit{PQ-F}.
We measure 100K traces and change the number of threads of checking from 1 to 16. 
 %Our second measurement demonstrates the impact of our parallel optimization consistency checking. 
%We check the consistency 100000 \textit{Set-r1} histories and 80000 \textit{PQ-F} histories with single thread checking as the baseline. 
%Then we use parallel {\vs} to check these histories with different thread number. 
As shown in Figure \ref{parallel}, the checking time decreases as we increase the number of threads regardless of using or not using pruning.
The decrease in time is quite significant when we increase the thread number from 1 to 6 in the case of \textit{PQ-F}, and 1 to 6 in the case of \textit{Set-r1}. 
As we add more threads, the checking time decreases approximately linearly. This means that the time decreases slowly than the ideal case where the time decreases to $\frac{1}{k}$ $(k$ is the number of threads).
%The checking time is not exactly $\frac{1}{k}$ of the single-threaded(\textit{k} is thread number) 
\begin{tbm}
This is because we cannot totally get rid of the overloading of some threads and the starvation of some other threads. 
Also the cost of thread scheduling increases when the thread number becomes larger, which drags the efficiency of parallelization. 
\end{tbm}
% This is because we simply divide the subtrees to be checked to the threads (see Figure \ref{F: Parallel}). This straightforward allocation of workloads often results in significantly uneven workloads on the threads, especially when the number of threads increases.
% The overloading of some threads and the starvation of some other threads greatly reduce the effectiveness of parallelization.
This evaluation results can tell us what are the sweet points to choose the number of threads. It also motivates us to design better schemes to evenly divide the workload among threads.

\color{red}
    It is worth noting that there is a sharp fall of time consumption between 4 and 6 parallel threads in the evaluation of \textit{PQ-F}. 
    It costs 0.36(0.30), 0.35(0.26), 0.26(0.21), 0.16(0.14) hours without(with) pruning when parallel threads is 6, 8, 12, and 16.
\color{blue}
    If a history satisfies a consistency model, the time consumption of checking is determined by the first thread that find a certificate abstract execution. 
    For a thread, it may construct a certificate abstract execution after hausting most of allocated search state, or it may construct one just after several search state. 
    When we use more threads checking in parallel, there is a higher probability that a thread constructs a certificate abstract execution only in a short time. 
    So it is reasonable that the time consumption decreases steeply from the number of parallel threads is 4 to the number of parallel threads is 6. 
\color{black}


%The effect of parallel optimization becomes less noticeable when thread number becomes large, because thread scheduling overhead drags the efficiency of parallelization. 
%In general, parallelization substantially improves the efficiency of measurement, and reduces the time costs. 

%--
\begin{figure}[htb]
    \centering
    \subfigure[PQ-F] {
        \includegraphics[width=0.47\hsize]{figures/pq-f-bar.png}
    }
    \subfigure[Set-r1] {
        \includegraphics[width=0.47\hsize]{figures/set-r1-bar.png}
    }
    \caption{Evaluation of Time Cost}
    \label{parallel}
\end{figure}

%--------------------
%\subsubsection{Efficacy of Filtering}
As for the pruning, we use the \textit{pruning ratio} as the performance metric. 
For a data access trace, we measure the consistency level serially and count the number of explored search states. 
We calculate the \textit{pruning ratio}, i.e. the ratio of the number of explored search states checked with the pruning to the number without the pruning.
%Our third measurement demonstrates the efficacy of filter. 
%We check a history without filter, and check the same history with filter. 
%We count the explored \textit{search states} for two checking. 
%We evaluate the optimization of filter by the ratio of explored states with filter to explored states without filter. 
For data types studied in the experiment, we pick one representative from multiple configurations of this data type. Specifically, we calculate the pruning ratio of four data types: \textit{Set-r1}, \textit{Map-r1}, \textit{Set-F}, and \textit{PQ-F}. %, and we check 10000 histories for each data type. 

As for the pruning ratio, we find that the effects of pruning significantly vary, as the number of search states (without pruning) increases. Our intuition is that the effects of pruning are more significant when there are more states to be explored by \textsc{ViSearch}, and the evaluation results prove this intuition correct.
Specifically, we divide the number of explored states without the pruning into four grades: small ((0,30]), moderate ([31, 300]), large ([301, 3000]) and huge ([3001, $+\infty$]).
%types by the number of explored states without state filter: 
%(0,30] for small search, [31,300] for medium search, [301, 3000] for big search, and [3001, +$\infty$) for huge search. 
%Then we calculate the average optimization ratio for histories of each type . 
As shown in Figure \ref{F: Pruning}, except for the 'small' grade, the pruning can reduce the number of search states approximately by half. Note that, for 'small' traces, the checking time is quite limited, with or without the pruning. This shows that, for the total checking time using the \vs framework, the pruning can significantly reduce the checking time (approximately by half).

One exception is \textit{Set-r1}. The pruning ratio of \textit{Set-r1} is more than 70\%, even for huge traces. This is mainly because \textit{Set-r1} provides weak visibility (see Table \ref{T: Result}), and the weak visibility checking takes most of the time. However, the weak visibility consistency predicate imposes few constraints on the visibility relation. We can find few pruning predicates conforming to the predicate template over all possible abstract executions. 
Therefore, the effect of pruning for \textit{Set-r1} is limited. 

We can also find that the pruning does not work well for the set type. Because the semantics of set only cares about the existence of elements and imposes fewer constraints on operations than other data types. 
So we find fewer pruning predicates for set. 

\begin{figure}[htb]
    \centering
    \includegraphics[width=\linewidth]{figures/pruningratio.png}
    \caption{Evaluation of State Filter}
    \label{F: Pruning}
\end{figure}

\begin{tbm}
Since the extraction and application of pruning predicates is also time-consuming, we also evaluate its impact on the overall checking time. 
As shown in Figure \ref{parallel}, the blue bar is the checking time without pruning and the orange bar is the checking time including predicate extraction and application. 
The orange bars is generally lower than the blue bars, which means pruning reduce the time consumption. Though the extraction algorithm is exponential, it is worth doing. 

In Figure \ref{F: Pruning}, \textit{PQ-F} has a better pruning ratio than \textit{Set-r1}, and it reflects on the time cost. In Figure \ref{parallel}, pruning has a better effect in \textit{PQ-F} compared to \textit{Set-r1}. 

We find that there is a negtive correlation between the effect of pruning and parallelization. When the effect of parallelization does not increases with the number of parallel threads any more, the effect of pruning is notable either. The parallelization increases the search state examined by \vs in unit time, and the pruning generally reduces a constant amount of state in the search space. So the pruning has a smaller impact on the time consumption, when the number of parallel threads becomes larger. 
\end{tbm}

%Our extraction of pruning predicates cannot find effective predicates for the pruning.

%the filter works well on big and huge searches which need to explore over 300 \textit{search states}, and these searches consume most of measuring time. 
%On short checkings, the filter does not have a good performance
%because the checking algorithm can easily find out an abstract execution for these histories by exploring only a few \textit{search states}, which can not leverage the state filter fully. 
%In general, the filter significantly reduces the explored \textit{search states} of checking, especially for those histories which cost long time to check. 

%--










==> maintext_backup/intro.tex <==
%--
\section{Introduction}

%\hy{背景}

Large-scale distributed systems often resort to replication techniques to achieve fault-tolerance and load distribution \cite{Burckhardt14, Shapiro11a, Enes19}. For a large class of applications, user-perceived latency and overall service availability are widely regarded as the most critical factors. Thus, many distributed systems are designed for low latency and high availability in the first place \cite{Lloyd13}. These systems have to trade data consistency for high availability and low latency \cite{Brewer12, Gilbert12}. A common approach is to resort to \textit{eventual consistency}, i.e., allowing replicas of some data type to temporarily diverge, and making sure these replicas will eventually converge to the same state in a deterministic way. The Conflict-free Replicated Data Type (CRDT) framework provides a principled approach to maintaining eventual consistency \cite{Shapiro11a, Burckhardt14}. 

CRDTs are key components in modern geo-replicated systems, such as Riak \cite{Riak}, Redis-Enterprise \cite{Redis-Enterprise}, and Cosmos DB \cite{CosmosDB}. Though CRDT designs and implementations widely use the notion of eventual consistency, this is a rather fuzzy consistency term and covers a broad range of actual consistency behaviors. Providing only eventual consistency makes programming over CRDTs difficult, in the sense that there can be arbitrary divergence between the replicas \cite{Bermbach14, Lloyd13}. 

The tension between the wide use of eventual consistency and the difficulty of programming over CRDTs motivates the measurement of eventual consistency \cite{Bailis14-vldbj, Burckhardt14-book, Golab14}. On the one hand, both providers and consumers of the distributed storage service benefit from knowing the precise degree of data (in)consistency. Quantifying the degree of data inconsistency can even enable customers and service providers to negotiate compensations proportional to the severity of violations in certain scenarios \cite{Golab11}.
\begin{tbm} On the other hand, pragmatic protocols in the practice of Cassandra, Mongodb, and Eiger actually achieve consistency guarantees stronger than eventual consistency \cite{Lloyd13}. \end{tbm} Existing practical stronger consistency semantics can be and should be utilized. Precise reasoning about the consistency semantics will significantly ease the burden of programming over CRDT data stores.

\begin{tbm}
Existing consistency measurement schemes are mainly based on certain metrics delineating the staleness of data, e.g., how long the data has been stale and how many new versions of data has been generated. 
These schemes measure data consistency by how many time units the value returned has been stale, or how many versions the data has been updated when the returned value is obtained. 
Since time units and versions can be expressed in numerical values, it is easy to compare the consistency of different data types. 
However, above consistency measurement schemes have their drawbacks. 
Neither time-based or version-based consistency measurement schemes can give a insight about how the data type actually works and how updates propogate across replicas. 
\end{tbm}

\begin{tbm} 
In this work we investigate a methodology for the precise measurement of replicated data type consistency semantics. 
We employ a formal specification framework for concurrent objects \cite{Bermbach14, Emmi18, Emmi19}. 
It is based on the \textit{visibility} and \textit{arbitration} relation over events of a history, and we call it the \textit{Visibility-Arbitration} framework (\visar in short). 
The \visar framework extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happen-before and linearization relations. 
The arbitration relation is a total order and plays the role as linearization in the linearizability. 
It indicates how the system resolves the conflicts between concurrent events. 
The visibility relation is an acyclic relation that describes the relative timing of update propagation among operations. 
If an operation $a$ is visible to $b$, it means that the effect of $a$ is visible to the client performing $b$. 
We consider that two events are concurrent, if they are invisibile to each other. 
\end{tbm}
The weaker the visibility relation, the more an operation is allowed to ignore the effects of concurrent operations that are linearized before it. 
Tuning the definition of the visibility relation gives us different levels of data consistency. 
We use diverse constraints on the visibility relation to define different levels of data consistency.

%\mybreak

%\hy{挑战}
\begin{tbm}
Visibility relaxation using the \visar framework is mainly used to precisely specify the consistency semantics of concurrent objects optimized for high-performance multithreaded code \cite{Emmi19, Emmi18}. 
Since concurrent objects often employ lock-free implementations and do not provide atomicity, the \visar framework is designed to measure the deviation from atomicity. 
However, in our replicated data type store scenarios, the replicated data types are designed to provide eventual consistency in the first place, and practical implementations often provide stronger semantics than the mere requirement of eventual consistency. 
Our main objective is not to measure the deviation from strong consistency, but to measure the augmentation over weak consistency.
\end{tbm}

\begin{tbm}
Though consistency measurement using the \visar framework is NP-hard in general \cite{Gibbons97, Emmi18}, brute-force checking algorithm is employed in the measurement. 
In Emmi et al.'s work, they use a brute-force checking algorithm to enumerate all correct executions, and quite small workload is studied (two threads, no more than 6 operations, and up to 2 values) \cite{Emmi19}. 
The key insight to circumvent the NP-hardness obstacle is that the violations are often local. That is, only a few operations can witness the violation. 
The small workload is repeated a sufficient number of (millions of) times to find and measure the deviation from atomicity. 

An optimization with greedy algorithm is proposed in another work \cite{Emmi18}. 
This algorithm constructs the correct execution with minimal exetension, which avoids some unnecessary enumeration in the above brute-force checking algorithm. 
However, the performance of the recursive algorithm is not efficient enough for consistency measurement in replicated data type store scenarios. 
We continue to optimize the checking algorithm based on this. 
\end{tbm}

%To find atomicity violations in concurrent programming, this is enough and it works. Small workload guarantees exhaustive checking. Exhaustiveness is more essential to find atomicity violations.

%\color{teal}

Our intuition is that the NP-hardness obstacle can also be circumvented in consistency measurement in replicated data type store scenarios. 
Certain domain knowledge can be leveraged to reduce the measurement cost, while moderately sacrificing the generality of the measurement algorithm.
Following this intuition, our first challenge is to refactor the brute-force consistency algorithm to conveniently incorporate such optimizations.
The second challenge is to find the locality of weak consistency measurement in realistic replicated data type store scenarios.

Toward the challenges above, we first transform the brute-force recursive algorithm for consistency measurement to a non-recursive algorithm skeleton.
Note that, the basic rationale of the measurement based on \visar is to try all possible abstract executions, i.e., all possible permutations of operations as well as all possible visibility relations between operations.
In the non-recursive algorithm skeleton, the intermediate state for construction of the abstract execution is explicitly maintained at runtime.
\begin{tbm}
Although it is a rewirte of the recursive algorithm, it facilitates the pruning and parallelization. 
Thus predicates which can be used to prune the search space can be flexibly "plugged" into the search skeleton. 
For load balancing, the algorithm needs to dynamic dispatch work to threads. 
But the recursive algorithm maintains the intermediate state in stack frame, which means that the visit order of states is fixed at recursive call, and cannot adjust dynamically any more. 
We discuss more details about the gains achieved from the transformation from recursive to non-recursive in Sec \ref{Sec: VS}. 
\end{tbm}

We extract useful filters by exhaustively enumerate all valid abstract executions for subhistories pertaining to one single data element. 
We name the subhistory we consider the query cluster. The query cluster contains multiple \textit{dictating updates} on some data element and one \textit{dictated query} on the very data element.
We enumerate all valid abstract executions over the query cluster, to extract "pruning predicates", i.e., arbitration and visibility relations that any valid abstract execution of the query cluster must hold. These pruning predicates must also hold on all valid abstract executions of the whole history. Thus \vs can use the pruning predicates to avoid unnecessary searching.
Moreover, since the construction of different abstract executions are independent, the search can be parallelized in a straightforward way.

We conduct experiments on two replicated data type stores Riak \cite{Riak} and CRDT-Redis \cite{CRDT-Redis}. %\footnote{Redis-CRDT is our revision of Redis. Redis-CRDT adopts the peer-to-peer multi-master architecture and CRDTs are used to resolve conflicting updates.} \cite{} 
Since our optimization of the consistency checking algorithm is still exponential in the worst-case, it is still intractable to measure data type access traces of arbitrary length.
As inspired by the application of the \visar framework in \cite{Emmi19}, we utilize the locality of consistency measurement in replicated data type scenarios, and measure the consistency of data type access traces at reasonable cost. We also study the effects of the pruning predicates and the parallelization through experiments.

The experimental evaluation also shows that the consistency measurement results are useful for both replicated data type designers and upper-layer application developers.
The measurement quantifies the difference between different conflict resolution strategies, as well as the difference between different configurations of the replicated data type store. 

The rest of this work is organized as follows.
Section \ref{Sec: Preli} introduces the basic concepts of conflict-free replicated data types and those of the \visar framework.
Section \ref{Sec: VS} introduces the \vs consistency measurement framework, and Section \ref{Sec: Exp} presents the experimental evaluation.
Section \ref{Sec: RW} discusses the related work. 
In Section \ref{Sec: Concl}, we conclude this work and discuss the future work.


==> maintext_backup/preli.tex <==
%--
\section{Preliminaries} \label{Sec: Preli}

In this section, we first introduce the basic concepts of Conflict-free Replicated Data Types (CRDTs). Then we introduce the Visibility-Arbitration (\textsc{Vis-Ar}) framework and consistency measurement based on visibility relaxation.

%--------------------------------------------------------------------------------
\subsection{Data Types}

We consider objects of data types stored in a replicated data store. 

\begin{definition}
    (Data Types). A data type $\tau \in \textit{Type}$ is a pair $\tau = (\textit{Op}, \textit{Val})$ such that
    \begin{itemize}
        \item \textit{Op} is the set of operations supported by $\tau$;
        \item \textit{Val} is the set of values allowed by $\tau$. We denote $\perp \in \textit{Val}$ to indicate that there is no return values for some operations. 
    \end{itemize}
\end{definition}

\begin{definition}
    (Sequential Semantics). The sequential semantics of a data type $\tau \in \textit{Type}$ is defined by a function $\mathcal{F}_{\tau}: \textit{Op}^{*} \times \textit{Op} \rightarrow \textit{Val}$. It means that given a sequence of operations $S$ and an operation $o$, the return value of $o$ is $\mathcal{F}_{\tau}(S, o) \in \textit{Val}$ when $o$ is performed right after $S$. 
\end{definition}

We denote an operation in the form of "$m(arg_1, \ldots, arg_n)\Rightarrow r$" to represent the invocation of a method $m$, with arguments $arg_1, \ldots, arg_n$, resulting in a return value $r$. 
We use sequential semantics to explain the execution of operations. The return value of an operation is determined by a certain sequence of operations that are performed before or concurrent with it. 

In this work, we consider operations are either queries or updates. 
Query operations only inspect state of the data type and do not change the state, while update operations modify state of the data type. 
Some data types may provide query-update primitives, i.e., operations inspect state of the data type and modify it at the same time. For example, the $extract\text{-}max()$ primitive of a priority queue is a query-update primitive, since it both obtains the maximum priority value and deletes the element with the maximum priority.
We can rewrite the history with query-updates and decompose each query-update operation into a pair of query and update \cite{Wang19}. 
So we only consider query operations and update operations in this work. 

% The salient feature of the CRDT is that the update operations are handled immediately without communication with remote replicas. Then the updates are asynchronously propagated to remote replicas. 
% We often omit the return value of update operations as they usually only return \textsf{ACK}. 


% An implementation \textit{Impl} of a replicated data type is a mapping from operations sequence $o_1 o_2 \ldots o_n$ to a return value sequence $Impl (o_1 o_2 \ldots o_n)=r_1 r_2 \ldots r_n$. For a total order of operations conducted on the data type, the return values of query operations and effects of updates operations follow the semantics of the standard data types. As for concurrent and conflicting updates, the effects of the updates are decided by the semantics of the CRDT, which are rigorously specified by the CRDT protocol.
% The logics for querying multiple replicas and merging the results from different replicas are often left to the upper layer application.

%--------------------------------------------------------------------------------
\subsection{\visar Framework Basics}

A consistency model acts as the contract between the underlying data type store and the upper-layer applications.
The \visar framework is an axiomatic consistency specification of concurrent objects \cite{Bermbach14, Emmi18, Emmi19}. 
It extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happens-before and linearization relations. 
The weaker the visibility relation, the more an operation is allowed to ignore the the effects of concurrent operations that are linearized before it. 
Tuning the definition of the visibility relation gives us different levels of data consistency. We use various predicates (i.e., constraints) on the visibility relations to define different levels of data consistency.

% We consider an abstract notion of executions, or behaviors, which captures observed return values and platform-defined happens-before orders among invocations in a given program. 
Histories, i.e., traces of data type access, are a set of all observable behaviors $\mathcal{H}$. The history defines how the clients interact with the data type store, and specifies what information is recorded about this interaction.
\begin{definition}
    (History). A history is an event graph represented by a tuple $\mathcal{H} = (E, op, rval, so)$ such that
    \begin{itemize}
        \item $E$ is the set of all events of operations performed by clients in a single execution; 
        \item $op : E \rightarrow Op$ describes the operation of an event; 
        \item $rval : E \rightarrow Val$ describes the return value of the operation $op(e)$ of an event $e$; 
        \item $so \subseteq E \times E$ is a partial order over $E$, called \textit{session order}.It describes the order of operations invoked by clients within a session. 
    \end{itemize}
\end{definition}

In this work, we only record the order between operations within the same session. The happens-before relation in this paper is limited to events/operations within the same session. 
 We do not record the \textit{returns-before} order over events which captures the real-time ordering of non-overlaping operations \cite{Burckhardt14-book}. Because we do not have a global time in distributed scenarios considering the clock drifting. 

%as there does not exist a unique write for each read operation in replicated data type scenarios. 

% Abstract Execution
In order to tell whether a history is consistent or not, the basic rationale underlying the \visar framework is that, a history is consistent if and only if we can justify it, by augmenting it with some additional information that explains the observed return values. 
For example, the linearizability consistency model inserts commit points in the timeline to justify the correctness of the observed return values. 

Based on the \visar framework, we add arbitration (i.e., linearization) and visibility relations to a history, and the augmented history is called an \textit{abstract execution}.
%Abstract executions are histories enriched by additional information about visibility and arbitration. 
%In the Vis-ar framework, the methodology of checking consistency of an implementation is based on abstract executions. 
% * This allows us to define not just linearizability, but the 
% By turning the arbitration and visibility relations in abstract executions, we can define a spectrum of consistency models that are commonly used for eventually consistent data type stores. Specifically, \textit{arbitration} is a linearization or total order on operations which indicates how the system resolves conflicting updates.
% If an operation $a$ is arbitrated before $b$ (denoted by $a \stackrel{ar}{\rightarrow} b$), it means that the system considers operation $a$ to happen earlier than operation $b$. 

% The \textit{visibility} relation is an acyclic relation, which describes the relative timing of update propagation among operations.
% If an operation $a$ is visible to $b$ (denoted by $a \stackrel{vis}{\rightarrow} b$), it means that the effect of $a$ is visible to the client performing $b$. 
% In replicated data type stores where replicas communicate with each other via messages, this means that the replica that performs operation $b$ receives the message containing operation $a$ before operation $b$ was performed. 
% In this work, we use $vis$ to represent visibility relation. 
% Given the definition of $lin$ and $vis$, an abstract execution is defined as an event graph $\mathcal{A} = (E, op, rval, hb, ss, lin, vis)$. 
%where \textsf{vis} is an acyclic and natural relation, and \textsf{ar} is a total order. 

\begin{definition}
    (Abstract Execution). An abstract execution is a triple $\mathcal{A} = ((E, op, rval, so), vis, ar)$ such that
    \begin{itemize}
        \item $(E, op, rval, so)$ is a history;
        \item Visibility $vis \subseteq E \times E$ is an acyclic and natural relation; A relation $R \subseteq A \times A$ is natural if $\forall x \in A : \left\vert R^{-1}(x) \right\vert < \infty$;
        \item Arbitration $ar \subseteq E \times E$ is a total. 
    \end{itemize}
\end{definition}

If an operation $a$ is visible to $b$ (denoted by $a \stackrel{vis}{\rightarrow} b$), it means that the effect of $a$ is visible to the client performing $b$. 
If an operation $a$ is arbitrated before $b$ (denoted by $a \stackrel{ar}{\rightarrow} b$), it means that the system considers operation $a$ to happen earlier than operation $b$. 
We use $lin$ to denote the linearization of operations after we decide the arbitration for concurrent operations. 

\setlength\emergencystretch{\hsize}

% We introduce the notion of subhistory $\mathcal{H}' = (E', op', rval', hb', ss')$, which denotes the projection of history $\mathcal{H}$ on a subset of events $E' \subseteq E$. 
% The notions $op'$ and $rval'$ are $op$ and $rval$ restricted on $E'$ respectively.
% The happens-before order $hb'$ is defined as $hb' = hb \bigcap (E' \times E')$ and the same-session relation $ss'$ is defined as $ss' = ss \bigcap (E' \times E')$. 
% Similarly, we can define the notion of projection for an abstract execution. 
% The projection of an abstract execution $\mathcal{A}$ on $E'$ is $\mathcal{A'} = (E', op', rval', hb', ss', lin', vis')$, 
% where $(E', op', rval', hb', ss')$ is the projection of the original history on $E'$. 
% The arbitration $lin'$ is defined as $lin' = lin \bigcap (E' \times E')$ and the visibility relation $vis'$ is defined as $vis' = vis \bigcap (E' \times E')$. 

\begin{definition}
    (Consistency Models). A consistency model is a set of consistency guarantees on abstract executions. 
\end{definition}

A consistency guarantee $\mathcal{\phi}$ is a constraint or property of an abstract execution $\mathcal{A}$. 
We write $\mathcal{A} \models \mathcal{\phi}$ if the abstract execution $\mathcal{A}$ satisfies the consistency guarantee $\mathcal{\phi}$. 

We can define a large variety of consistency guarantees by formulating conditions on the various attributes and relations appearing in the abstract execution.

An abstract execution $\mathcal{A}$ satisfies consistency model $\Phi = \{\mathcal{\phi}_1, \mathcal{\phi}_2, \ldots, \mathcal{\phi}_n\}$, if it satisfies every consistency guarantees in $\Phi$. Formally, $\mathcal{A} \models \Phi \Leftrightarrow \mathcal{A} \models \mathcal{\phi}_1 \land \mathcal{A} \models \mathcal{\phi}_2 \land \ldots \land \mathcal{A} \models \mathcal{\phi}_n$. 

A history $\mathcal{H}$ satisfies the consistency model $\Phi$, denoted $\mathcal{H} \models \Phi$, if it can be extended (by adding visibility and arbitration) to an abstract execution that satisfies consistency model $\Phi$. Formally, $\mathcal{H} (E, op, rval, so) \models \Phi \Leftrightarrow \exists vis, ar. ((E, op, rval, so), vis, ar) \models \Phi$. 

There are mainly two types of consistency guarantees. 
One is about ordering of operations. This type of guarantees mainly consist of constraints on arbitration and visibility relations.
%guarantees (such as causality) that defines rules for reordering of operations, 
%and convergence guarantees that ensure eventual consistency. 
The other is about data type semantics that gives meaning to operations. %Every event in an abstract execution must have a return value which is allowed by the semantics $Impl$ of given replicated data type. 

\subsection{Consistency Measurement via Visibility Relaxation} \label{SubSec: Vis-Relax}

In \cite{Emmi19}, a consistency spectrum consisting of six consistency models is defined by visibility relaxation, i.e., gradually relaxing the constraints on the visibility relations in the abstract execution.
These models, from weak to strong, are \textit{weak}, \textit{basic}, \textit{monotonic}, \textit{peer}, \textit{causal} and \textit{complete} visibility.

The two ends of the consistency spectrum are weak and complete visibility. The weak visibility permits any observations made by an operation, while the complete visibility requires that operations observe all operations which are linearized before them. 

Between the two ends, the basic visibility requires operations to see their happens-before predecessors which corresponds to a strengthening of the read-your-writes guarantee. 
The monotonic visibility requires each operation to see those its happens-before predecessors see. It corresponds to the monotonic reads guarantee, which states that reads observe an increasing sets of updates. 
On the basis of monotonic, the peer visibility requires a read to observe an update only if it has observed all the predecessors from the update's session, which corresponds to the monotonic writes guarantee.
The causal visibility requires that the visibility relation be transitive. It means that each operation is require to see those visible to the operations that it sees. 

We call them six consistency levels in the rest of this work, and use this 6-level scale of consistency levels for the consistency measurement.

\begin{tbm}
    We define a set of predicates which constraint the observation made by a given operation. 
    Formally, a visibility predicate $\varphi(o, \mathcal{A})$ is a first-order predicate on operation $o$ in an abstract execution $\mathcal{A}$. Given an abstract execution $\mathcal{A}$, we define $vis(o)$ is a set of operations visible to $o$; $hb(o)$ is a set of operations that happens before $o$ according to the session order $so$; $lin(o)$ is a set of operations arbitrated before $o$. 
    \begin{itemize}
        \item weak$(o, \mathcal{A}) \Leftrightarrow \textbf{\textit{true}}$
        \item basic$(o, \mathcal{A}) \Leftrightarrow hb(o) \subseteq vis(o)$
        \item monotonic$(o, \mathcal{A}) \Leftrightarrow \forall o' \in hb(o): vis(o') \subseteq vis(o)$
        \item peer$(o, \mathcal{A}) \Leftrightarrow$ monotonic$(o, \mathcal{A}) \land \forall o' \in vis(o): hb(o') \subseteq vis(o)$ 
        \item causal$(o, \mathcal{A}) \Leftrightarrow$ basic$(o, \mathcal{A}) \land \forall o' \in vis(o): vis(o') \subseteq vis(o)$ 
        \item complete$(o, \mathcal{A}) \Leftrightarrow lin(o) \subseteq vis(o)$
    \end{itemize}
\end{tbm}

\color{blue}
In Figure \ref{F: Visibility}, we show the difference of several level of visibility. 
The operations(rounded rectangle) visible to the given operation(bold rounded rectangle) depend on the visibility level. 
The \textit{basic} imples that visibility(solid arrow) of happens-before predecessors(horizontal line) while \textit{monotonic} implies visibility of those visible(dashed arrow) to predecessors. 
The \textit{peer} implies visibility of predecessors of visible operations, and \textit{causal} implies transitive visibility. 
visibility of predecessors of visible operations
\color{black}

\begin{figure}[htb]
    \includegraphics[width=\linewidth]{figures/visibility.jpg}
    \centering
    \caption{Visibility}
    \label{F: Visibility}
\end{figure}

Basically, the consistency measurement is conducted on one history or trace of replicated data type access. Theoretically speaking, to measure consistency guarantee of one data type, we need to measure all possible traces of this data type, which is simply not possible. Moreover, it is usually quite difficult to strictly prove the consistency level certain replicated data type provides. In this work, when we say consistency measurement for one data type, we mean that a sufficiently large number of traces generated by this data type is measured, and the result of this measurement is a sufficiently accurate approximation of the consistency level provided by this data type.

==> maintext_backup/rw.tex <==
%--
\section{Related Work} \label{Sec: RW}

%\hy{怎么规约}

The fuzzy nature of eventual consistency and its wide adoption motivate the quantification of severity of consistency violations \cite{Golab11, Golab14, Golab18}. Existing quantification techniques can be viewed from two perspectives. From the micro-perspective, existing consistency measurement schemes are mainly based on certain metrics delineating the staleness of data, e.g., how long the data has been stale and how many new versions of data has been generated.
%The metric can be how long the data has been stale, e.g. $\Delta$- and $\Gamma$-consistency \cite{Golab14}, and how many new versions of data has been generated, e.g. $k$-atomicity \cite{Golab18}. 
Time-based quantification techniques, e.g. $\Delta$-atomicity \cite{Golab11} and $\Gamma$-atomicity \cite{Golab14}, are adopted for applications sensitive to realtime consistency requirements. Time-based techniques measure data consistency by how many time units the value returned has been stale. 
For applications sensitive to the frequency of data updates, version-based quantification techniques , e.g. k-atomicity \cite{Golab18}, are proposed. Version-based techniques measure data consistency by how many times the data has been updated when the returned value is obtained.
From the macro-perspective, Yu and Vahdat propose TACT (Tunable Availability and Consistency Tradeoffs), a middleware layer that supports application-dependent consistency
semantics expressed as a vector of metrics defined over a logical consistency unit or conit \cite{Yu02-TOCS}. Inconsistencies in the observed value of a conit are bounded using three metrics: numerical error, order error, and staleness.

The consistency measurement schemes above are from the end user's perspective. In order to better facilitate the development of upper-layer applications, we need to measurement schemes which focus on how data are updated, in a similar way to how linearizability is specified. To this end, in this work we borrow the \visar framework which is an axiomatic consistency specification framework of concurrent objects. %which consider operation visibility. 
The \visar framework extends the linearizability-based specification methodology with a dynamic visibility relation among operations, in addition to the standard dynamic happens-before and linearization relations. 
The \visar framework is more suitable for developers to reason about the correctness of the implementation of a replicated data type. It is also suitable for upper-layer application developers to reason about the correctness of applications.

%\hy{关于checking}

The checking of data type access traces is NP-Complete in general \cite{Gibbons97}.
However, this intractability result can be circumvented by reasonable assumptions in specific scenarios. For example, the write values are often assumed to be unique %, which can makes the checking problem tractable in many scenarios 
\cite{Gibbons97}. This assumption is reasonable and easy to satisfy, since we can append certain meta-data to the values written to make them unique. 
In replicated data type store scenarios, the number of concurrent writes is often assumed to be bounded by some constant \cite{Golab18}. 
Practitioners can also limit the pattern of the input and derive an input specific efficient checking algorithm \cite{Bouajjani17}. 

The checking of data type access traces using \vs is also intractable in the worst case. As inspired by the existing techniques to circumvent the NP-hardness obstacle, we refactor the brute-force checking algorithm to a generic algorithm skeleton. This refactor enables practical pruning of the exponential search space in certain scenarios. We also employ the locality of the checking of CRDT access traces to make the consistency measurement practical in realistic scenarios.

%\slt{关于粒度}
% The existing work measures the consistency of Java's concurrent objects at the per-method granularity \cite{Emmi19}. 


==> maintext_backup/vs.tex <==
%--
\section{\vs Framework} \label{Sec: VS}

In this section, we first overview the basic design rationale behind the \vs framework. Then we present the key techniques. In the next Section \ref{Sec: Exp}, we will demonstrate how to apply the \vs framework in realistic data type store scenarios.

%--------------------------------------------------------------------------------
\subsection{\vs  Overview}

Consistency measurement using \vs boils down to the search of an abstract execution satisfying certain constraints on the arbitration and visibility relations. 
This search process involves enumerating the linearizations, i.e. arbitrations of all operations, as well as the visibility relations between operations.
To prove that one trace satisfies certain consistency model, it is sufficient to find one single abstract execution that satisfies all the constraints. % on the arbitration and visibility relations.
We name this abstract execution the "certificate" abstract execution (there could be more than one certificate execution).
%The success in finding one single abstract execution which satisfies the consistency model can prove that the trace satisfied certain consistency model
%Below we note arbitration as linearization because arbitration is actually a permutation of all operations. 
%The checking of each consistency level boils down to finding an arbitration of as well as the visibility among all operations. 

The search process is intractable in general \cite{Gibbons97, Emmi19, Emmi18}. However, the search can still be practical and cost-effective in replicated data type store scenarios. %, since the traces in real scenarios do not always force the checking algorithm to the worst case.
To enable efficient search of abstract executions, we first refactor the existing search algorithm to a non-recursive algorithm skeleton.
The intermediate states for construction of the abstract executions are explicitly maintained by the algorithm skeleton at runtime. 

\color{blue}
The traversal order of search is fixed in the existing recursive algorithm as the intermediate states are stored in the stack frame, which is actually a depth-first search. 
This is a simple way but has a drawback. The algorithm cannot adjust the traversal order according the runtime feedback, which impacts the parallel performance greatly. 
Because we only roughly estimate the workload of each thread before parallel search starting, and it leads to overloading and starvation between threads. We need to re-allocate the workload in a regular cycle, moving intermediate search states from overloading threads to starving threads. We can hardly do this in the recursive algorithm since all the intermediate search states are stored in the system's stack. 
\color{black}

Based on the \vs skeleton, we propose optimizations from two orthogonal dimensions. 
First, the non-recursive algorithm skeleton enables efficient pruning of the search space. 
We can flexibly plug pruning predicates into the algorithm skeleton to avoid the unnecessary search of certain abstract executions, while the pruning predicates can be extracted from the subhistory concerning multiple update operations and one query operation on one single data element. %certain part of the data type access traces. 
\begin{tbm}
Noted that a subhistory $\mathcal{H}'$ is the projection history $\mathcal{H}$ on a subset of events $E' \subseteq E$, and only keeps relations in the set $E' \times E'$. 
\end{tbm}
Second, we also find that the search process is stateless, i.e., the enumerate of different candidate executions are independent. Thus we further parallelize the search.  

%--------------------------------------------------------------------------------
\subsection{\vs Algorithm Skeleton}

We first briefly review the existing recursive search algorithm \cite{Emmi19, Emmi18}. Then we present the non-recursive algorithm skeleton.

%----------------------------------------
\subsubsection{The Original Recursive Search Algorithm}

Consistency measurement using the \vs framework can simply use a recursive backtracking algorithm to search the possible arbitration and visibility relations among operations in a brute-force way. We use $\ang{lin, vis}$ to denote an abstract execution. If an abstract execution $\ang{lin, vis}$ satisfies a consistency model $\Phi$, we have $\langle lin, vis \rangle \models \Phi$. 
During the search process, we manipulate some prefix of $lin$, denoted by $lin_i$. We use $vis_i$ to denote the visibility relation on operations in $lin_i$. 
The search algorithm can be view as extending candidate executions from $\ang{lin_i, vis_i}$ to $\ang{lin_{i+1}, vis_{i+1}}$.


%It is intuitive that $\langle lin_i, vis_i \rangle \models \varPhi$ if $\langle lin, vis \rangle \models \varPhi$. 
\setlength\emergencystretch{\hsize}
%until the abstract execution includes all operations.

The search algorithm tries all possible extensions from the current candidate execution $\ang{lin_i, vis_i}$. 
When valid extensions cannot be obtained, the current "candidate" is discarded and the search algorithm backtracks to another candidate execution.
%An abstract execution $\langle lin_i, vis_i \rangle$ can be extended with different choices of operations, and obtains a series of abstract execution $\left\{ \langle lin_{i+1}', vis_{i+1}' \rangle, \langle lin_{i+1}'', vis_{i+1}'' \rangle, \ldots \right\}$ as candidates. 
%We can select one of them as the extension of $\langle lin_i, vis_i \rangle$. 
When we finally extend the prefix to a whole abstract execution containing all the operations in the data type access trace, we successfully get the certificate abstract execution, and the search algorithm returns \textsf{TRUE}.
If no certificate extension can be obtained after trying all possible candidates, the search algorithm returns \textsf{FALSE}.

%At some point in construction, the abstract execution is invalidated if it is extended with any operation, and at that time the algorithm has to backtracks and search for other candidates. 

%If the algorithm finally manage to construct a complete abstract execution that includes all operation in the history, we obtain the certificate abstract execution which proves that the history satisfies the consistency model.

%Otherwise, the history does not satisfy the consistency model. 

%As construction of abstract execution follows the way of backtracking to search in a solution space, we name our algorithm framework {\vs} which means \textit{visibility-relaxation search}. 

%----------------------------------------
\subsubsection{The revised non-recursive search} \label{SubSubSec: Revised-VS}

The main improvement made to the recursive search algorithm is that we refactor it to a non-recursive one. This means that, the algorithm skeleton itself maintains a double-ended queue to store the intermediate search states $\ang{lin_i, vis_i}$ at runtime.
%To enable flexible optimization, we revise the original recursive search.
%The key in the refactorization is to use a stack to explicitly maintain the intermediate state of the search at runtime.
The explicit maintenance of intermediate search states greatly facilitates further pruning of unnecessary searches.

The non-recursive \vs algorithm searches abstract executions through phases, as shown in Figure \ref{F: Tree}. In each phase, it extends $\ang{lin_i, vis_i}$ to $\ang{lin_{i+1}, vis_{i+1}}$. There are two steps in each phase. In the 'ar step', we add one operation to $lin_i$ and obtain $lin_{i+1}$. In the 'vis step', we extend $vis_i$ to $vis_{i+1}$ by adding visibility relations concerning the newly added operation. 

%In each phase, we start from $\ang{lin_i, vis_i}$ and add a new operation to the linearization of the old search state and find a proper visibility relation for the newly added operation. 

\color{blue}
Formally, we denote a set $\mathcal{O}$ that contains all operations already in the $\ang{lin_i, vis_i}$. And we denote a set $\mathcal{U}$ that contains all operations in the history. 
In the 'ar step', we select an operation $o \in \mathcal{U} \setminus \mathcal{O}$, and obtain the new arbitration order $lin_{i+1} = lin_{i} \bigcup \mathcal{O} \times \{o\}$. 
In the 'vis step', we extend the visibility relation $vis_{i}$ by unioning a subset of $\mathcal{O} \times \{o\}$. And the new visibility relation $vis_{i+1}$ must satisfy the visibility constraint of consistency model. 

%--
\begin{figure}[htb]
    \includegraphics[width=\linewidth]{figures/tree.jpg}
    \centering
    \caption{Search State Extension}
    \label{F: Tree}
\end{figure}


As shown in Figure \ref{F: Tree}, the algorithm has already constructed a certificate abstract execution $\ang{lin_2, vis_2}$ that contains operations \textit{add}(1) and \textit{add}(2). Then the algotirhm starts phase 3. In the "ar step", the algorithm first appends operation \textit{size}() to the $lin_2$ and obatins $lin_3$. In this example, we require each operation must be visible to operations within the same session. So the operation \textit{size}() can return 1 if $add(1) \stackrel{vis}{\rightarrow} size()$, or return 2 if $add(1), add(2) \stackrel{vis}{\rightarrow} size()$. But neither of two visibility relations bring the correct return value, the algorithm backtracks for other candidates. 

Then we append operation \textit{remove}(2) to the $lin_2$. We can construct a certificate abstract execution $\ang{lin_3, vis_3}$ and finish phase 3. At last we start phase 4, and append the last operation \textit{size}() to the linearization. The operation \textit{size}() has four visibility extension candidates: $\left\{\textit{add(2)}\right\}\stackrel{vis}{\rightarrow}\textit{size}()$, $\left\{\textit{add(1)}, \textit{add(2)}\right\}\stackrel{vis}{\rightarrow}\textit{size}()$, $\left\{\textit{add(2)}, \textit{remove(2)}\right\}\stackrel{vis}{\rightarrow}\textit{size}()$, and $\left\{\textit{add(1)}, \textit{add(2)}, \textit{remove}(2)\right\}\stackrel{vis}{\rightarrow}\textit{size}()$. We omit candidates $\{\textit{add(2)}\}\stackrel{vis}{\rightarrow}\textit{size}()$ and $\{\textit{add(1)}, \textit{add(2)}, \textit{remove}(2)\}\stackrel{vis}{\rightarrow}\textit{size}()$ due to limited space in the picture. The operation \textit{size}() returns 0 only if $add(2), remove(2) \stackrel{vis}{\rightarrow} size()$, which means the operation \textit{size}() ignore the effect of the operation \textit{add}(1). Finaly, we find a certificate abstract execution, and prove the history satisfies the consistency model. 
\color{black}

%\slt{这里Impl前面没有定义？预计要在sec2定义，参考ra-lin的定义方式。}
%\mybreak
%\slt{下面，明确写出phase的概念，然后phase中分arb部分和vis部分。第一部分，统一用lin，不用再跟arb混着讲。}

%In detail, there are two steps in a phase: one for linearization and the other for visibility. 
%We first add a new operation to the total order, whose predecessors must have been already in the \textit{linearization}. 
%It means that $\langle \textit{lin}_i, \textit{vis}_i \rangle$ is extended to $\langle \textit{lin}_{i+1}, \textit{vis}_i \rangle$. 

%Then we extend the visibility relation which is compatible with the new linearization. 
%The visibility $\textit{vis}_i$ can be regarded as $\bigcup_{k = 1}^{i} v_k$ where $v_k$ is the visibility relation for the \textit{k}th operation in the linearization. 
%We construct the visibility relation incrementally by choosing a visibility relation \textit{v} for the operations that is newly added. 
%The visibility relation \textit{v} must adhere to the visibility specification of the given consistency model. 
%It means that we extend $\langle \textit{lin}_i, \textit{vis}_i \rangle$ to $\langle \textit{lin}_{i+1}, \textit{vis}_{i+1} \rangle$, where $\textit{vis}_{i+1} = \textit{vis}_{i} \cup v $. 

%There may be multiple choices to extend the linearization the visibility relation. 
%The candidate extensions of linearization are all equal. 
%But the candidate extensions of visibility can be ordered according to set inclusion, and we only need to consider the minimal visibility relations \cite{Emmi18}.

%\mybreak

%\slt{因为现在是强调我们的非递归重构，所以需要专门讲“非递归，自己搞栈”的一些细节，如果成功，就压栈如何继续。当不成功，就丢弃xxx，然后从栈里抽取出xxx，如何如何继续。}

%During the search process, we keep checking the consistency predicate. Whenever the consistency predicate is violated, the current candidate execution is discarded and we backtrack to search new candidates.

Upon initialization, we build a \textit{search state deque} with the initial search state $\ang{lin_0, vis_0}$. State $\ang{lin_0, vis_0}$ contains no operation and has an empty visibility relation. 
During the search process, we keep polling search states from the head of deque.
The newly popped search state is verified by the method \textsf{isValidAbstractExecution} ({Line 6 in Algorithm \ref{A: VS}}). This method basically checks whether the return values of all query operations in the current search state are allowed by the semantics \textit{Impl} of the data type under concern.
Invalid search states are discarded and valid ones are extended as follows. %We throw invalidated \textit{search states} away and extend validated \textit{search states}. 

For a given valid search state $\ang{lin_i, vis_i}$, we first extend the linearization by \textsf{linExtend} (Line 10 in Algorithm \ref{A: VS}), and get a set of new search states:
$$newLin = \left\{ \ang{lin_{i+1}^1, vis_i}, 
\ang{lin_{i+1}^2, vis_i}, \ldots, \ang{lin_{i+1}^p, vis_i} \right\}.$$
\color{blue}
Each new search state in \textit{newLin} represents a selection in $\mathcal{U} \setminus \mathcal{O}$. In fact, the number of new states $p$ should be less than or equal to the cardinality of \textit{newLin} because the extension of linearization needs to adhere to the same-session order. 
\color{black}

%\slt{把下标的i加上。把尖括号命令，换成新定义的ang{}命令。后续的search state不用再斜体。\\
%    \indent 发现i这个下标过载了，商量一下新的下标体系。}

Then we extend visibility relations according to the newly added operation.
%extend each \textit{search state} in \textit{newLins} for visibility. 
Each newly-extended \textit{search state} $\ang{lin_{i+1}^{r}, vis_i}$ will be extended to a set of \textit{search states}, 
$$newVis_r = \left\{ \ang{lin_{i+1}^{r}, vis_{i+1}^1}, \ang{lin_{i+1}^{r}, vis_{i+1}^2}, \ldots, \ang{lin_{i+1}^{r}, vis_{i+1}^{q}} \right\}.$$

%\slt{改下标等所有细节。}
\color{blue}
Each search state in $newVis_r$ corresponds to the selection of a subset of $\mathcal{O} \times \{o\}$, where $o$ is the newly-added operation and $\mathcal{O}$ contains operations in $lin_{i}$. 
\color{black}
Each search state in $\bigcup_{i=1}^{p} newVis_i$ is a possible extension of $\ang{lin_i, vis_i}$.We push all the candidate states into the head of deque. 
In the next step, the search algorithm will get a candidate from the head of deque and repeat this extension process. 
Once the search state cannot be extended any more, the algorithm will backtrack by polling older candidates from the head of deque. 

The {\vs} algorithm returns \textsf{TRUE} if it obtains a certificate abstract execution.
The algorithm returns \textsf{FALSE} if it runs out of candidates and still cannot obtain any certificate execution.
The pseudocode of the \vs algorithm skeleton is listed in Algorithm \ref{A: VS}.

%--
\begin{algorithm}[ht]
    \caption{The \vs Algorithm Skeleton}
    \label{A: VS}
    \KwIn{history $\mathcal{H}$, 
        data type implementation \textit{Impl}, 
        consistency model $\Phi$}
    \KwOut{whether history $\mathcal{H}$ satisfies the given consistency model $\Phi$}
    \textit{deque} $\leftarrow$ \{\ \}\\
    \textit{initState} $\leftarrow$ $\ang{\emptyset, \emptyset}$\\
    \textit{deque}.\textsf{push}(\textit{initState})\\
    \While{$\lnot$deque.\textnormal{\textsf{isEmpty}( )}}{
        \textit{state} $\leftarrow$ \textit{deque}.\textsf{pollHead}( )\\
        \If{\textnormal{\textsf{isValidAbstractExecution}(}Impl, state\textnormal{)}}{
            \If{state\textnormal{.\textsf{isComplete}( )}}{
                \Return{\textnormal{\textbf{true}}}
            }
            \textit{newLin} $\leftarrow$ \textit{state}.\textsf{linExtend}($\mathcal{H}$)\\
            \ForEach{\textit{newLinState} $\in$ \textit{newLin}}{
                \textit{newVis} $\leftarrow$ \textit{newLinState}.\textsf{visExtend}($\Phi$)\\
                \text{/* <Pruning is Plugged Here> */}\\
                \textit{deque}.\textsf{pushTailAll}(\textit{newVis})\\
            }
        }
    }
    \Return{\textnormal{\textbf{false}}}
\end{algorithm}


%---------------------------------------
\subsection{Pruning of the Search Space}

The key to circumventing the NP-hardness obstacle of abstract execution searching is to leverage specific knowledge of the data type under search and prune the search space. 
%We prune the search space to reduce the cost for searching valid abstract executions.
Thus, we inspect the data type access trace and automatically extract \textit{pruning predicates}, which can be plugged into the \vs algorithm skeleton (Algorithm \ref{A: VS}). 
For each candidate abstract execution, the search algorithm check the pruning predicates. Once any pruning predicate is detected \textsf{FALSE}, the candidate abstract execution is directly discarded.
We will prove that the pruning process is "safe", i.e., the pruning process never discards any candidate abstract execution which can be extended to a certificate abstract execution.

In this section, we first present the basic rationale of pruning with three illustrating examples.
Then we present the design and correctness proof of the pruning algorithm.

%--------------------
\subsubsection{Rationale of the Pruning}

The search algorithm enumerates every valid abstract execution in a brute-force way.
The insight behind our pruning scheme is that, for a  given data element in a container type, the update and query operations concerning this element cannot be linearized in an arbitrary way. Moreover, the visibility relations among these operations also have only limited patterns.
\color{blue}
% The insight behind our pruning scheme is that, the linearizations and visibility relations must follow some rules. 
For example, when we check a history of multiple shared variable access, 
% for each query operation that the set contains a certain element, there exists an update operation that add the element into the set.  
for each read operation \textit{r}, there exists a unique write operation \textit{w}. The operation \textit{r} and \textit{w} reads/writes the same variable and the same value. The operation \textit{w} must happen before \textit{r}. The rule mentioned above can be formally defined as the write-to order \cite{Wei16}. 
\color{black}

However, the \vs algorithm is not aware of this type of knowledge concerning one specific data element, and enumerates all abstract executions it thinks that is possible.
Thus, we can extract this type of knowledge and express it as pruning predicates. The predicates can be plugged into the \vs algorithm skeleton and prune the search space. %reduce the search cost.
\color{blue}
We will use these pruning predicates before adding new search states into deque ({Line 6 in Algorithm \ref{A: VS}}). 

We find that in a data type update and query operations invoked on a same data element usually form a cluster. The update operations determine the return values of query operations in the same cluster, while update operations rarely affect the query operations in the other cluster. 
\color{black}

Based on the insight above, we introduce the notion of a \textit{query cluster}. All operations in the query cluster are explicitly associated with the same data element.
The query cluster contains exactly one query operation, which is denoted the \textit{dictated query}. The query cluster contains one or more update operations, which are denoted \textit{dictating updates}. The dictating updates are those update operations which can potentially affect the return value of the dictated query. 

\color{blue}
We consider two situations. One situation is that the update operations are the necessary and sufficient condition for the result of a query operation. For example, whether the set contains the element \textit{x} is determined by the arbitration and visibility of all \textit{add} and \textit{remove} operations associated with element \textit{x}. 
The other situation is that the update operations are the necessary condition for the result of a query operation. For example, \textit{get\_max} tells that the maximum element of the priority queue is \textit{x} with value \textit{v}. All update operations associated with element \textit{x} only guarantee that there exists an element \textit{x} with value \textit{v} in the priority queue at that point, but there might be some elements with larger value than \textit{x}. However, the necessary condition is enough to ensure the safety of pruning. 

\color{black}

For example, inserting one element into the priority queue and increasing the priority value of the element, and returning the existence or priority value of the element.
We do not consider operations which correspond to multiple data elements, e.g., the $isEmpty()$ operation, which returns whether the data container is empty.

%like this, and do not take operations like $isEmpty()$ into account as they do not refer to a specific element. 

%\mybreak

%\slt{query被几个update完全决定}


% >>>>>具体的单元素操作的例子
%
%For example, an operation \textit{contains}(\textit{z}) is related to the its argument, the element \textit{z}, 
%and an operation \textit{get\_max}()$\Rightarrow$(\textit{x; v}) is related to its return value. 
%
%Update operations involved in the related element potentially determine the return value of the query operation. 
%
%The return value of operation \textit{contains}(\textit{z}) is totally decided by operation \textit{add} and \textit{remove} on element \textit{z}. 
%
%Similarly, operation \textit{get\_pri}(\textit{e}) is totally decided by operation \textit{insert}, \textit{remove}, and \textit{inc} on element \textit{e}. 
%
%Different from \textit{contains}() and \textit{get\_pri}(), operation \textit{get\_max}()$\Rightarrow$(\textit{x;v}) is not decided by update operation on element \textit{x}. 
%Because we need to assure that there does not exist any other element whose \textit{priority} is bigger than \textit{v}, 
%besides the necessary condition that there exists an element in the priority queue whose \textit{id} is \textit{x} and \textit{priority} is \textit{v}. 
%However, the existence of the element (\textit{x;v}) is totally decided by updates on element \text{x}. 
%So due to the the necessary condition, we say that operation \textit{get\_max}()$\Rightarrow$(\textit{x;v}) is partly decided by operation \textit{insert}, \textit{remove}, and \textit{inc} on element \textit{x}. 
%
% >>>>>



We will use two data types \textit{set} and \textit{priority queue} as illustrating examples for the extraction of pruning predicates.
The set is a container of elements, in which each element is identified by its unique \textit{id}. 
The following primitives are involved in examples: 
%--
\begin{itemize}
    \item $add(e)$ : add element $e$. 
    \item $remove(e)$ : remove the element $e$. 
    \item $contains(e)$ : return \textsf{TRUE} if $e$ is in the set.
    % \item $isEmpty()$ : return \textsf{TRUE} if the set is empty. 
\end{itemize}

\noindent The priority queue is a container of elements of the form $e = (id, priority)$.
The following primitives are involved in examples: 
%--
\begin{itemize}
    \item $insert(e, x)$ : enqueue element $e$ with initial priority $x$. 
    % \item $remove(e)$ : remove the element \textit{e}. 
    \item $inc(e, \delta)$ : increase the priority of element $e$ by $\delta$ (may be negative). 
    \item $get\_pri(e)$ : return the priority value of $e$.
    \item $get\_max()$ : return the \textit{id} and \textit{priority} of the element with the highest priority. 
    % \item $isEmpty()$ : return \textsf{TRUE} if the priority queue is empty. 
\end{itemize}

% 之前的版本侧重于讲我们如何利用cluster之间的locality去进行剪枝
% 新增的部分主要是说明为什么需要有template和extraction, 因为 
%   1. data type的语义变复杂了, 不是简单的shared variables, 读写之间的因果链条不再是直接的了. 很难人工为每一个data type定义出write-to order那样的规则
%   2. 引入vis之后一个操作可以忽略之前的操作了, 变得更加烧脑, 人定规则可能会遗漏case
% 所以需要template和extraction保证不管什么data type都能剪, 提取的剪枝谓词肯定safe

\color{blue}
It becomes difficult to seek out explicit rules like write-to order to extract pruning predicates, when we check data types with enriched semantics. For example, we can add or remove an element in the data type set. We can even increase and decrease the priority of an element. All these rich semantics of data types make the cause and effect between query operation and update operation are unclear. 
Visibility relations being introduced into consistency specification makes things much more complicated. because an operation may ignore the effects of other operations. Pruning predicates formulated by human are hardly perfectly safe. 

We want to extract pruning predicates automatically, and make sure that they are correct. In this context we define some templates which applies to various data types, and design a suite of algorithms that extract correct pruning predicates. 
\color{black}


The pruning predicate is obtained by inspecting the query cluster pertaining to one specific data element.
There can be two types of pruning predicates. 
The first type is simpler, which only considers the arbitration relation between operations, while the second type considers both the arbitration and the visibility relations.

%\mybreak

By in-depth inspection of the data type access trace and manual exploration of the brute-force checking process, we come up with three predicate templates, i.e. patterns of pruning predicates we want to extract.
The first predicate template focuses on the arbitration relation. It aims to find that two operations always have the arbitration relation, no matter how you construct the linearization of operations. Specifically, $\tarb$ states that operation $x$ must be arbitrated before operation $y$ in every search state $\ang{lin, vis}$:
%--
\begin{eqnarray*}
    \tarb(x, y) \mydef \forall \ang{lin, vis}, (x,y) \in lin
\end{eqnarray*}


To extract pruning predicates following the template $\tarb$, we enumerate all valid abstract executions of the subhistory consisting of all operations in one query cluster.
For example, assume that there is a subhistory with two client sessions.
One session has operation $insert(x,5)$, followed by $inc(x,1)$.
The second session has one single operation $get\_pri(x) \Rightarrow 6$.
For the ease of illustration, we simply assume that there are no other operations on $x$ in the whole trace. 

It is evident that the return value of $get\_pri(x)$ is 6 only if it is linearized after $inc(x,1)$.
All valid abstract executions of this query cluster must have this arbitration order $inc(x,1)  \stackrel{ar}{\rightarrow} get\_pri(x) \Rightarrow 6$.
This fact must also hold for all candidate abstract executions the \vs algorithm constructs. Thus it can be extracted as a pruning predicate and plugged into \vs to avoid unnecessary searches.

The second and the third predicate templates are of the second type and concern both the arbitration and the visibility relations. 
As for the $\tvis$ example in Figure \ref{F: Template}, if the arbitration relations among operations have been decided, we can infer that there must be the visibility relation between $remove(z)$ and $contains(z) \Rightarrow \textsf{FALSE}$. Otherwise, the semantics of the set type are violated.
The $\tnotvis$ example is the dual of the $\tvis$ one. If the return value of $contain(z)$ is \textsf{TRUE}, there should be no visibility relation between $remove(z)$ and $contain(z)$.

%According to *rulearb, we find a filter that $(ins, inc) \in lin$. In running the \vs checking algorithm, whenever this pruning predicate is false, the candidate abstract execution is discarded.

%Therefore, whenever the algorithm constructs an abstract execution which \textit{inc}(\textit{x},1) is linearized before \textit{insert}(\textit{x},5), 
%we prune this search state as the current abstract execution cannot be extended to a complete one. 

%The pair of \textit{insert}(\textit{x},5) and \textit{inc}(\textit{x},1) is a fact for $\mathcal{P}_{A}(x, y)$. 

%Moreover, it is reasonable to infer that \textit{insert}(\textit{x},5) and \textit{inc}(\textit{x},1) must be linearized before \textit{get\_pri}(\textit{x})$\Rightarrow$6. 

%\slt{Fig2要换成我们黑板上讨论的例子，不然文字读起来，读者易误解}

%--
\begin{figure}[htb]
    \includegraphics[width=\linewidth]{figures/rule.jpg}
    \centering
    \caption{Rule Examples}
    \label{F: Template}
\end{figure}

%\slt{图里的true，false要改字体，与正文统一。\\
%    \indent \indent 用not-vis，而不是non-vis。\\
%    \indent \indent rulea，ruleb要改，要是数学不好写，可以写the arb template, the vis template, the not-vis template之类的。}

Generalizing the examples above, $\tvis$ states that certain arbitration relations and certain visibility relation always co-occur:
%--
\begin{eqnarray*}
    \tvis(S_{lin}, x, y) \mydef \forall \ang{lin, vis} : (a,b) \in S_{lin} \rightarrow (x,y) \in vis %\\
    %\mathcal{P}(a, b, x, y) \stackrel{\triangle}{=} \forall \langle lin, vis \rangle : (a,b) \in lin \rightarrow (x,y) \in vis
\end{eqnarray*}

\noindent where $S_{lin}$ is a subset of the arbitration relation (a subset of operation pairs having the arbitration relation).
The dual template $\tnotvis$ states that if there are certain arbitration relations, certain visibility relation cannot occur:
%--
\begin{eqnarray*}
    \tnotvis(S_{lin}, x, y) \mydef \forall \ang{lin, vis} : (a,b) \in S_{lin} \rightarrow (x,y) \not \in vis %\\
    %\mathcal{P}(a, b, x, y) \stackrel{\triangle}{=} \forall \langle lin, vis \rangle : (a,b) \in lin \rightarrow (x,y) \not \in vis
\end{eqnarray*}

\noindent We scan all valid abstract executions of the query cluster and check whether there are operation patterns that can be match by the two predicate templates $\tvis$ and $\tnotvis$.

%To solve these problems, we develop a predicate extraction method. 

%We focus on subhistories consisting of multiple updates and one query all pertaining to one data element.

%We enumerate all possible abstract executions of the subhistory. 

%We match the predicate template over all possible executions, to see whether there are pruning predicates.

%We present the details below.

%For every abstract execution, we check whether there are predicates predicate template 

%This method enumerates all complete abstract executions of a small cluster, and extracts necessary conditions from all complete abstract executions to generate predicates. 



%----------------------------------------
\subsubsection{Extraction of Pruning Predicates}

The extraction of pruning predicates is similar to a "string matching" process. 
The predicate template is analogous to the pattern string to be searched, while all valid abstract executions of a query cluster as a whole is analogous to the text string being scanned.
Note that we are interested in predicates which are \textsf{TRUE} for all abstract executions of a given query cluster.
The query cluster can just be treated as a normal trace of data type acces, and we can directly use the brute-force the \vs checking algorithm (Algorithm \ref{A: VS}) to search all valid abstract executions. 
\color{blue}
We can regard the computing of extraction as constant complexity because the size of query cluster is rather small compared to the size of the history. We evaluate the time cost of pruing predicate extraction in Sec \ref{Sec: Exp}, and show that it is worth doing that. 
\color{black}
We extract from the executions concrete pruning predicates following the templates $\tarb$, $\tvis$ and $\tnotvis$. 

For an abstract execution $\pi_t$ = $\ang{{lin}^t, {vis}^t}$, we define that $lin(\pi_t)$ = $lin^t$, $vis(\pi_t)$ = $vis^t$. 
We define the not-visible relation of an abstract execution $\pi_t$ by $notvis(\pi_t)$ = $\{(x,y) \mid (x,y) \in lin^t \land (x,y) \notin vis^t\}$. 
% We define $\mathcal{U}(\mathcal{H}) = O \times O$ as a complete relation of operations in history $\mathcal{H}$.  

%\slt{下标似乎应该写在下面？跟前面讨论统一 \\
%    \indent \indent 全关系，定义去掉？放到伪码注释中？/* U is the complete relation which contains all possible pairs of operations.\\
%    \indent \indent yield T(op1, op2)。避免“未知数”的感觉}

It is straightforward to extract pruning predicates of template $\tarb$ from valid abstract executions. 
We just need to intersect every linearization of valid abstract executions, as shown in Algorithm \ref{A: T-ARB}.
Specifically, linearization of an abstract execution $\pi$ is a total order of operations. For each pair of operations, $(x,y) \in lin(\pi)$ means that operation $x$ is arbitrated before operation $y$ in abstract execution $\pi$. 
The intersection of all linearization is the arbitration order that every valid abstract execution must obey. 
Each concrete operation pair $(op1, op2)$ in the final intersection of linearizations can generate a concrete pruning predicate $\tarb(op1, op2)$. 

%--
\begin{algorithm}[ht]
    \caption{Extraction of Pruning Predicates for $\tarb$}
    \label{A: T-ARB}
    
    \KwIn{a set of abstract execution $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
    \KwOut{a set of pruning predicates of $\tarb$}
    
    $S_{\text{arb}}$ $\leftarrow$ $U$\quad\CommentSty{/* U is the complete relation which contains all possible pairs of operations. */}\\
    \ForEach{$\pi \in \mathcal{A}$}{
        $S_{\text{arb}}$ $\leftarrow$ $S_{\text{arb}} \bigcap lin(\pi)$
    }
    
    \ForEach{pair $(x,y) \in S_{\text{arb}}$}{
        \textbf{yield} $\tarb(x,y)$
    }
\end{algorithm}


To extract pruning predicates following the template $\tvis$, we union the visibility relation of all valid abstract executions: $\mathcal{V} = \bigcup_{t=1}^{m} vis(\pi_t)$. 
For each pair $(x,y) \in \mathcal{V}$, it means that operation $x$ is visible to operation $y$ in some valid abstract execution. 
Then we try to generate a concrete predicate of template $\tvis$ for every pair $(x,y) \in \mathcal{V}$. 

We first intersect the linerarization of valid abstract executions that contains the pair $(x,y)$. 
Any valid abstract execution whose visibility relation contains pair $(x,y)$ must obey the arbitration order in the intersection $S_{\text{arb}}$. 

Next we need to ensure that there exists no counterexample for this concrete predicate. %, or this concrete predicate is not a necessary condition for the subhistory. 
Because we extract this concrete predicate only from valid abstract executions which contain pair $(x,y)$ in their visibility relation. 
We must check whether it is a necessary condition for those valid abstract executions which do not contain pair $(x,y)$ in their visibility relation.
We discard this concrete predicate, if there is a valid abstract execution whose visibility relation does not contain pair $(x,y)$ but it obeys all arbitration order in the intersection $S_{\text{arb}}$.
The pseudocode of the extraction algorithm for $\tvis$ are listed in Algorithm \ref{A: T-VIS}.

%\slt{文字解释一下：为什么这个二次检测是必须的，不能遗漏。}

%--
\begin{algorithm}[ht]
    \caption{Extraction of Pruning Predicates for $\tvis$}
    \label{A: T-VIS}
    
    \KwIn{a set of abstract executions $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
    \KwOut{a set of pruning predicates of $\tvis$}
    
    $S_{vis}$ $\leftarrow$ $\bigcup_{t=1}^{m} vis(\pi_t)$\\
    \ForEach{pair $(x,y) \in S_{vis}$}{
        $S_{arb}$ $\leftarrow$ $U$\\
        \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \in vis(\pi)$}{
            $S_{arb}$ $\leftarrow$ $S_{arb} \bigcap lin(\pi)$
        }
        
        \textit{review} $\leftarrow$ \textsf{TRUE}\\
        \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \notin vis(\pi)$}{
            \If{$S_{arb} \subseteq lin(\pi)$}{
                \textit{review} $\leftarrow$ \textsf{FALSE}\\
                \textbf{break}
            }
        }
        \If{\textit{review} \textnormal{is} \textnormal{\textsf{TRUE}}}{
            \textbf{yield} $\tvis(S_{{arb}}, x, y)$
        } 
    }
\end{algorithm}

Since the template $\tnotvis$ is just the dual of $\tvis$, the extraction of concrete predicates for $\tnotvis$ is similar to the extraction for $\tvis$. 
We just replace the visibility relation in the $\tvis$ extraction algorithm with the not-visibility relation. 

%--
% \begin{algorithm}[ht]
%     \caption{Extraction of Pruning Predicates for $\tnotvis$}
%     \label{A: T-NOT-VIS}
    
%     \KwIn{a set of abstract executions $\mathcal{A} = \{\pi_1, \pi_2 \ldots \pi_m\}$}
%     \KwOut{a set of pruning predicates of $\tnotvis$}
    
%     $S_{notvis}$ $\leftarrow$ $\bigcup_{i=1}^{m} notvis(\pi_i)$\\
%     \ForEach{pair $(x,y) \in S_{notvis}$}{
%         %$S_{arb}$ $\leftarrow$ $\mathcal{U}(\mathcal{H}_q)$\\
%         $S_{arb}$ $\leftarrow$ $U$\\
%         \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \in notvis(\pi)$}{
%             $S_{arb}$ $\leftarrow$ $S_{arb} \bigcap lin(\pi)$
%         }
        
%         \textit{review} $\leftarrow$ \textsf{TRUE}\\
%         \ForEach{$\pi \in \mathcal{A}$ \textnormal{which} $(x,y) \notin notvis(\pi)$}{
%             \If{$S_{arb} \subseteq lin(\pi)$}{
%                 \textit{review} $\leftarrow$ \textsf{FALSE}\\
%                 \textbf{break}
%             }
%         }
%         \If{\textit{review} \textnormal{is} \textnormal{\textsf{TRUE}}}{
%             \textbf{yield} $\tnotvis(S_{arb}, x, y)$
%         } 
%     }
% \end{algorithm}

%----------------------------------------
\subsubsection{Correctness of Pruning}
\color{red}
We now prove that the pruning is safe, i.e., no certificate execution can be discarded by the pruning predicates. 
Given a history $\mathcal{H}$ and a consistency model $\Phi$, if $\mathcal{H} \not\models \Phi$, it means that there exists no certificate abstract execution for $\Phi$. 
% An abstract execution of history $\mathcal{H}$ is certificate if and only if it satisfies the requirement of $\Phi$. 
So the pruning must be safe. 
Therefore in the rest of the proof, we focus on the case in which history $\mathcal{H}$ has a certificate abstract execution satisfying the consistency model $\Phi$. 

In fact, the \vs algorithm prunes abstract executions during the construction process at runtime. So we need to prove that no candidate abstract execution, which can be extended to a certificate execution in the future, is pruned.
%no constructing abstract execution which can be extended to a correct one is pruned by filter. 
However, if an abstract execution violates a pruning predicate, all of its extensions violate the filter too. 
Hence, we only need to prove that there does not exist a certificate execution which violates the pruning predicate. 

Here is the proof stretch of the correctness of pruning. 
We assume for contradiction that there exists a certificate abstract execution $\pi$ of history $\mathcal{H}$ which violates a pruning predicate $P$.
The pruning predicate $P$ is extracted from a certain query cluster in history $\mathcal{H}$, so we project the abstract execution $\pi$ on the query cluster and get a projection $\pi'$. 
The projection $\pi'$ is an abstract execution of the query cluster where the predicate $P$ is extracted. 

The arbitration and visibility relations among \textit{dictating updates} and \textit{dictated query} is reserved after projection, so $\pi'$ still violates the predicate $P$. 

For the same reason, the \textit{dictated query} of the query cluster has the same return value after projection. 
Since $\pi$ is a certificate abstract execution, each operation in $\pi$ does not omit any operations it must see according to the visibility constraint of $\Phi$. 
Compared to $\pi$, each operation in $\pi'$ only more omit  those operations discarded in projection, so the projection $\pi'$ still satisfies the visibility constraint. 
Hence the projection $\pi'$ still the consistency model $\Phi$. 

Because the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
Therefore, the pruning in \vs is safe. The candidate abstract executions discarded can never be extended to a valid certificate one.

\color{black}

% 证明剪枝正确性的方法一, 避开了繁琐的分类讨论, 引入新的概念函数G作为一个vis是否合法的判断依据
% 然后简单地通过投影后必须看见的操作应该相应地减少, 通过集合 \subseteq 的传递关系去完成证明
% 优点是证明看起来比较有理有据 不像分类讨论都是文字的叙述
% 缺点是引入了新的符号 新的形式化语言

% \color{red}
% Here is the proof stretch of the correctness of pruning. 
% We assume for contradiction that there exists a certificate abstract execution $\pi$ of history $\mathcal{H}$ which violates a pruning predicate $P$. The projection $\pi'$ is some abstract execution of the query cluster which generates predicate $P$. 
% We project the abstract execution $\pi$ on the subhistory where the predicate $P$ is extracted, and get the projection $\pi'$. %(可能需要补一下projection的定义)
% % The projection of the abstract execution $\mathcal{A} = ((E, op, rval, so), vis, ar)$ on $E' \subseteq E$ is $\mathcal{A'} = ((E', op, rval, so'), vis', ar')$, where $vis' = vis \cap (E' \times E')$ similar for $so$ and $ar$. 

% If the projection $\pi'$ still violates the predicate $P$ and satisfies the consistency model $\Phi$, we can prove that the pruning is safe. 
% Because the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
% This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
% Therefore, the pruning in \vs is safe. The candidate executions discarded can never be extended to a valid certificate abstract execution.

% It is trivival that the abstract execution $\pi'$ still violates the predicate $P$. Because $\pi'$ contains all the operations of the query cluster from which $P$ is extracted, and reserves the arbitration and visibility between these operations.

% We need to prove the satisfaction of the consistency model $\Phi$ from three points. Firstly the projection $\pi'$ is a legal abstract execution. Secondly the query operation in $\pi'$ has the same return value with the corresponding operation in $\pi$. Thirdly the abstract execution $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 

% The proof of the thrid point is a bit tricky. We define a relation $\mathcal{V}_k$ that describes the visibility of $o_k$, while the visibility relation of the first $k-1$ operations is fixed during the construction. 
% We extend the visibility relation of $\ang{lin_{k-1}, vis_{k-1}}$ to $\ang{lin_{k}, vis_{k}}$ by adding $\mathcal{V}_k$ to $vis_{k-1}$. 
% There exists a function $\mathcal{G}$ mapping a tuple $(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k)$ to a set $\mathcal{M}$. 
% The set $\mathcal{M}$ is the visibility relation that describles what $o_k$ at least see according to the visibility constraint of the consistency model. If $\mathcal{M} \subseteq \mathcal{V}_k$, $\mathcal{V}_k$ is a legal visibility extension for the consistency model $\Phi$. 

% After projection, some operations are discarded from the the abstract execution $\pi$. The visibility relation $\mathcal{V}_k$ becomes $\mathcal{V}_{k'}$, and we denote $\mathcal{R} = \mathcal{V}_k \setminus \mathcal{V}_{k'}$. 
% The operation $o_{k'}$ no longer need to see the discarded operations, and the discarded operations break the transitivity of visibility. So the $\mathcal{G}(\ang{lin_{k'-1}, vis_{k'-1}}, \mathcal{V}_{k'}, o_{k'}) = \mathcal{M'}$ is a subset of $\mathcal{M} \setminus \mathcal{R}$. 
% Hence there exists
% \begin{equation*}
%     \mathcal{M'} \subseteq \mathcal{M} \setminus \mathcal{R} \subseteq \mathcal{V}_k \setminus \mathcal{R} = \mathcal{V}_{k'}
% \end{equation*}
% The projection $\pi$ satisfies the visibility constraint of the consistency model $\Phi$. 

% Due to limited space, we put the detailed proof and the definition of function $\mathcal{G}$ on \cite{Shi22}. 

% \color{black}

% \begin{tbm}
% Here is the proof stretch of the correctness of pruning. 
% We assume for contradiction that there exists a certificate abstract execution $\pi$ of history $\mathcal{H}$ which violates a pruning predicate $P$. 
% We project the abstract execution $\pi$ on the subhistory where the predicate $P$ is extracted, and get the projection $\pi'$. %(可能需要补一下projection的定义)
% The projection of the abstract execution $\mathcal{A} = ((E, op, rval, so), vis, ar)$ on $E' \subseteq E$ is $\mathcal{A'} = ((E', op, rval, so'), vis', ar')$, where $vis' = vis \cap (E' \times E')$ similar for $so$ and $ar$. 
% The projection $\pi'$ is some abstract execution of the query cluster which generates predicate $P$.

% If the following two statement establish
% \begin{itemize}
%     \item the projection $\pi'$ still violates the predicate $P$;
%     \item the projection $\pi'$ satisfies the consistency model $\Phi$;
% \end{itemize}
% we can prove that the pruning is safe. 
% As the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
% This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
% Therefore, the pruning in \vs is safe. The candidate executions discarded can never be extended to a valid certificate abstract execution.
% % retains the linearization and visibility relation among operations in subhistory. 

% If the following two statement establish
% \begin{itemize}
%     \item the projection $\pi'$ still violates the predicate $P$;
%     \item the projection $\pi'$ satisfies the consistency model $\Phi$;
% \end{itemize}
% we can prove that the pruning is safe. 
% As the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each valid abstract execution of the query cluster must satisfy predicate $P$ according to the extraction algorithm. 
% This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
% Therefore, the pruning in \vs is safe. The candidate executions discarded can never be extended to a valid certificate abstract execution.

% Here is the detailed proof of the two statement. 
% The projection $\pi'$ contains all the operations of the query cluster from which $P$ is extracted, and the projection reserves the relations between operations of the query cluster. So the abstract execution $\pi'$ still violates the predicate $P$. 

% Next we prove that $\pi'$ satisfies the consistency model $\Phi$, which means $\pi'$ is a valid abstract execution of the query cluster. 

% First, the projection keeps a total order $ar'$ among remaining operations, and an acyclic and natural relation $vis'$. So $\pi'$ is a legal abstract execution. 

% Second, the query cluster only has one dictated query operation and some dictating update operations. 
% This dictated query operation has the same operation context, i.e., the same arbitration and visibility relations of the dictating update operations. The return value of the dictated query operation is only affected by dictating update operations. As a result, the query operation in $\pi'$ has the same return value with the corresponding operation in $\pi$, which satisfies the semantics constraint of the consistency model. 

% 第三点证明有两个可替换的版本

% Third, the abstract execution $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 
% As we construct the abstract execution by operation, the visibility relation of the first $k-1$ operations is fixed when we choose the visibility of the $k$-th operation $o_k$. 
% We define a set $\mathcal{V}_k$ consisting of operations that is visible to the $k$-th operation. 
% We extend the abstract execution $\ang{lin_{k-1}, vis_{k-1}}$ to $\ang{lin_{k}, vis_{k}}$ by adding 
% $\mathcal{V}_k$ to $vis_{k-1}$ and adding $o_k$ to the end of $lin_{k}$. 

% We define a function $\mathcal{G}$ mapping a tuple $(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k)$ to a set $\mathcal{M}$. 
% The set $\mathcal{M}$ is the visibility relation that describles what $o_k$ must see according to the visibility constraint of the consistency model. If $\mathcal{M} \subseteq \mathcal{V}_k$, $\mathcal{V}_k$ is a legal visibility extension for the consistency model $\Phi$. 
% For example, we list some function $\mathcal{G}$ according to the visibility predicates in \ref{SubSec: Vis-Relax}, 
% \begin{itemize}
%     \item $\mathcal{G}_{weak} = \emptyset$, which has no constraint for visibility. 
%     \item $\mathcal{G}_{basic}(\_, \_, o_k) = \{(x, o_k)\ \vert\ \forall x: (x, o_k) \in so \}$, which means $o_k$ must see all the operations that happens before it according to the session order. 
%     \item $\mathcal{G}_{monotonic}(\ang{lin_{k-1}, vis_{k-1}}, \_, o_k) = \{(x, o_k)\ \vert\ \forall x \exists y : (y, o_k) \in so \land (x, y) \in vis_{k-1}\}$, which means $o_k$ must see the operations that its predecessors see. For the sake of simplicity, each operation is visible to itself. 
%     \item $\mathcal{G}_{causal}(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k) =  \{(x, o_k)\ \vert\ \forall x :(x, o_k) \in (vis_{k-1} \bigcup \mathcal{V}_k)^{+}\} \bigcup \mathcal{G}_{basic}(\_, \_, o_k)$, which means $o_k$ must see operations visible to those $o_k$ sees, and the visibility is a transitive closure. 
% \end{itemize}

% The set $\mathcal{R}$ contains relation pairs in the abstract execution $\pi$ but not in the projection $\pi$. 
% $\mathcal{V}_{k'}$ is the visibility relation that describles operations visible to the $k$-th operation in $\pi$, i.e. the $k'$-th operation in $\pi'$ after projection.  
% All relation pairs in $\mathcal{R}$ are removed from $\mathcal{V}_k$ after projection, so $\mathcal{V}_{k'} = \mathcal{V}_k \setminus \mathcal{R}$. 
% Also operations in $\mathcal{R}$ are removed from $\mathcal{M}$ after projection. Considering the transitivity, some operations cannot see another operation via removed operations in $\mathcal{R}$ any more, 
% \begin{equation*}
%     \begin{split}
%         &\mathcal{M}' = \mathcal{G}(\ang{lin_{k'-1}, vis_{k'-1}}, \mathcal{V}_{k'}, o_{k'}) \\
%         &\subseteq \mathcal{G}(\ang{lin_{k-1}, vis_{k-1}}, \mathcal{V}_k, o_k) \setminus \mathcal{R} = \mathcal{M} \setminus \mathcal{R}.
%     \end{split}
% \end{equation*} 

% As the original abstract execution $\pi$ satisfies the visibility constraint of the consistency model $\Phi$, we can conclude that
% $\mathcal{M} \subseteq \mathcal{V}_k$ and further deduce that $\mathcal{M} \setminus \mathcal{R} \subseteq \mathcal{V}_k \setminus \mathcal{R}$. 
% Combining the transitivity of $\subseteq$, we can conclude that 
% $\mathcal{M}' \subseteq \mathcal{V}_{k'}$. 
% Therefore, the projection $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 

% To sum up above three points, the projection $\pi'$ satisfies the consistency model $\Phi$. 
% \end{tbm}

% \color{red}
% Third, we want to prove that the abstract execution $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 
% To simplify the question, we first prove that if only one operation is discarded from the abstract execution $\pi$ via projection, $\pi'$ still satisfies the visibility constraint. Then we can decompose a projection into a series of projections, and each projection only discards one operation from the previous abstract execution. 

% Next, we discuss six visibility levels by case. 
% \begin{itemize}
%     \item \textit{Weak} visibility permits any observations made by an operation, so the projection never violate the visibility constraint. 
%     \item \textit{Basic} visibility requires that operations observe all operations which happen before them. The visibility of each operation in the original abstract execution must already contains all its the predecessors. Since the discarded operation cannot be the predecessor of some operation any more. the projection of abstract execution still satisfies the visibility constraint. 
%     \item The proof of \textit{monotonic} visibility is similar to the \textit{basic} visibility. The discarded operation cannot be visible to some operation, so the projected visibility of each operation still contains all operations visible to its predecessors. 
%     \item \textit{Peer} visibility requires each operation to see the predecessors of those operation visible to it. The discarded operation cannot be the predecessor of some operation any more, so the projected visibility of each operation still contains all the predecessors of those operation visible to it. 
%     \item \textit{Causal} visibility requires each operation to see what operations visible to it see. Considering the transitivity, some operations cannot see another operation via the discarded operations any more. The transitive closure of the visibility relation is the subset of the original one. After projection only one operation is discarded from the visibility of each operation, $\pi'$ still satisfies the visibility constraint. 
%     \item The proof of \textit{complete} visibility is similar to the \textit{basic} visibility. The discarded operation cannot be linearized before some operation any more. 
% \end{itemize}

% Therefore, the projection $\pi'$ still satisfies the visibility constraint of the consistency model $\Phi$. 

% To sum up above three points, the projection $\pi'$ satisfies the consistency model $\Phi$. 

% As we construct the abstract execution by operation, the visibility relation of the first $k-1$ operations is fixed when we choose the visibility of the $k$-th operation $o_k$. The visibility extension of the $k$-th operation does not effect whether the previous operations satisfy the visibility constraint. So if the visibility of the $o_1, o_2, \ldots, o_m$ in the projection $\pi'$ satisfies the visibility constraint, 


% Because the visibility relation in $\pi'$ is a subset of the visibility relation in $\pi$. Thus the visibility in $\pi'$ is stronger, in the sense that in the projection $\pi'$, the operations miss (i.e., cannot see) less operations in the subhistory. In contrast, the operations in $\pi$ miss more operations, considering the whole abstract execution.
% We thoroughly check each of the six consistency models (defined in Section \ref{SubSec: Vis-Relax}) and show that the satisfaction of each consistency model still holds after the projection (this detailed checking process only involves low-level details and is omitted in our proof).

% As the pruning predicate $P$ is extracted from all valid abstract executions of the query cluster, each abstract execution $\pi'$ must satisfy predicate $P$. 
% %So $\pi'$ adheres to the filter $R$ and violates the filter $R$ at the same time. 
% This leads to contradiction, since we have $\pi'$ must satisfy $P$ and violate $P$ at the same time.
% %would result in a contradiction. 
% Therefore, the pruning in \vs is safe. The candidate executions discarded can never be extended to a valid certificate abstract execution.

%--------------------------------------------------------------------------------
\subsection{Parallelization of \vs}

All legal search states of a history are organized as a tree, as shown in Figure \ref{F: Parallel}. 
Each search state is a node in the tree, and the root node is the empty abstract execution $\ang{lin_0, vis_0}$.
For a node $\ang{lin, vis}$ in the tree, search states which are possible extensions of $\ang{lin, vis}$ in the next phase are the children of $\ang{lin, vis}$. 
%Conversely, $\ang{lin, vis}$ is the parent of all search states which are possible growth of it in one phase. 
There may exist many candidate extensions in one phase, different choices of extensions result in the search of different subtrees. %split into different branches of the tree. 

%--
\begin{figure}[htb]
    \includegraphics[width=0.9\linewidth]{figures/p_tree.jpg}
    \centering
    \caption{Parallel \vs}
    \label{F: Parallel}
\end{figure}


%\slt{因为是树所以可以无脑并行}

%The tree has a recursive structure. 
%A tree consists of a root, and zero or more subtrees $T_1, T_2, \ldots , T_k$, and the root of each subtree is the child node of root of the tree. 
The procedure of consistency checking in \vs is like a depth-first search in tree whose goal is to find a leaf node corresponding to a search state that constructs a certificate abstract execution.
Therefore, there exists natural parallelization for the search. 
Subtrees do not share any nodes and are independent of each other. So we can search the subtrees in parallel. 
If we find a certificate abstract execution in any subtree, we terminate tasks in other subtrees and the history satisfies the consistency model. 
If no subtrees can find certificate executions, the history does not satisfy the consistency model. 

%\slt{提出了并行优化}

%We devise parallel optimization to accelerate {\vs} called parallel {\vs}. 
%With parallelization, we can check the consistency of a history using multi-threading, which better utilizes the compute resources and improves checking speed. 
\begin{tbm}
At the beginning of the parallel \textsc{ViSearch}, we first run the sequential \vs algorithm in a breadth-first search way, and generate a batch of search states. 
The search states are evenly allocated to different threads. Then each thread runs an instance of the sequential \vs algorithm in a depth-first search way to continue the search from each search state allocated to it. 
Note that here we use the term "thread" in a broader sense. The thread is more like an abstract worker. It can also be, for example, a virtual or physical machine.
See the example in Figure \ref{F: Parallel}. We generate four search states (the root node of each subtree in the dashed box). 
Each of the four states is allocated to a thread. The four threads extend the search states in parallel and obtain four different subtrees (the colored subtrees in four dashed boxes).
\end{tbm}

\begin{tbm}
Since the search states are divided randomly to different threads, it may lead to imbalanced load. 
We design a simple but useful dynamic load balancing mechanism, which thanks to the transformation from recursive to non-recursive. 
Because we need to adjust the load of each thread according to the runtime execution. 
Since the search states are maintained in a deque which is manipulated by algorithm, we can easily fetch search states from one thread's deque and add to another thread's to balance the load between two threads. 
If we use a recursive algorithm where search states are stored in the stack of operating system, we can hardly change the execution flow of the checking algorithm. 

We implement a search coordinator to maintain the meta information of parallel search, including the number of idle threads and working threads. 
When the the parallel \vs starts, the number of idle threads is set as zero.  
If a thread has finished its load, it returns the search result to the coordinator. 
The coordinator will increase the number of idle threads, if the thread do not find a certificate execution. 
Otherwise, the coordinator will stop all working threads and return \textsf{TRUE}. 

To avoid overloading and starvation, every working thread checks the number of idle threads at frequent intervals. 
If the number of idle threads is more than 0, the working thread will try to acquire the mutex of the coordinator, and share half of search states in its deque with an idle thread. 
The reason why we choose this mechanism is that interrupting a running thread is more complex than regular self-examination of running threads. 

The interval of self-examination is also important. 
Idle threads will starve for a long time if the interval is too large. 
And working threads will spend too much time on competing for the mutex of coordinator if the interval is too small. 
We set the interval 1000 search states, which means working threads stop to check whether there exists idle threads every 1000 search states checked. 
According to our experience, most of time-consuming checkings need to checking over 10,000 search states, and 1000-search-state interval is an appropriate portion. 
We also add a 10\% random disturbance in order to avoid too many working threads acquiring the mutex of the coordinator at the same time. 
\end{tbm}


%\slt{结合伪代码讲一下}

%The parallel {\vs} algorithm is presented in Algorithm \ref{A: PVS}. 
%The algorithm generates initial states at first, which are search states with a certain number of operations. 
%We can easily implement the method \textsf{generateInitialStates} by revising the centralized \vs algorithm (Algorithm \ref{A: VS}). 
%We replace the stack in line 1 with a queue, and let the algorithm return all search states in the queue when the size of queue exceeds a certain number. 
%As the number of the initial states is not exactly equal to the number of threads, 
%the initial states are divided into k parts for each thread, where k is the number of threads. 
%
%After that, we start {\vs} in parallel, and each thread carries out a {\vs} task. 
%When a thread exits, we examine the result of this {\vs} task. 
%If this {\vs} task returns \textsf{TRUE}, the algorithm will stop other running threads and return \textsf{TRUE}. 
%If this {\vs} task returns \textsf{FALSE}, the algorithm will increase a counter which records how many {\vs} tasks have returned \textsf{FALSE}. 
%The algorithm returns \textsf{FALSE} if all {\vs} tasks return \textsf{FALSE}. 


%\slt{分析一下优化效果}

%Theoretically, the checking time of the parallel search can be reduced to the $\frac{1}{k}$ of that of the sequential search, where $k$ is the number of threads. 
%Because, parallel {\vs} checks $k$ times of search states as the single-threaded {\vs} checks in the same amount of time. 
%In other words, the checking time can be ideally reduced to $\frac{1}{k}$ of the original. 
%However in practice, the search of one subtree may cost significantly more time than the search of another subtree. It is because different subtrees mean different linearizations of the operations, and the possible visibility relations to be checked for different linearizations may vary quite a lot.
%This means that there may be some threads are overloaded while some threads starve. Thus the parallel search cost is often more than $\frac{1}{k}$ of the sequential search cost.
%How to analyze the search states and evenly allocate workload among the threads is left to future work.

%--
% \begin{algorithm}[ht]
%     \caption{Parallel \vs}
%     \label{A: PVS}
%     \SetKwBlock{DoParallel}{do in parallel}{end}
%     \KwIn{history $\mathcal{H}$, 
%         data type implementation \textit{Impl}, 
%         consistency model $\Phi$}
%     \KwOut{whether history $\mathcal{H}$ satisfies the given consistency model $\Phi$}
%     $\mathcal{I}$ $\leftarrow$ \textsf{generateInitialStates}()\\
%     Divide $\mathcal{I}$ into $\mathcal{I}_1, \mathcal{I}_2, \ldots, \mathcal{I}_k$\\
%     \DoParallel{
%         Visearch Checking with initial states $\mathcal{I}_1$\\
%         Visearch Checking with initial states $\mathcal{I}_2$\\
%         $\cdots$\\
%         Visearch Checking with initial states $\mathcal{I}_k$\\
%     }
% \end{algorithm}

==> newcommands.tex <==
% newcommands.tex

% math
\newcommand{\set}[1]{\{#1\}}
\newcommand{\argmax}{\operatorname{arg\,max}}
\newcommand{\tord}[1]{\textsl{to}(#1)}

\newcommand{\mongodb}{MongoDB}
\newcommand{\mongodbcc}{\textsl{MongoDB-CC}}
\newcommand{\gentlerain}{\textsl{GentleRain}}

% color
\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\teal}[1]{\textcolor{teal}{#1}}

% specification
\newcommand{\op}{\texttt{op}}
\newcommand{\rval}{\texttt{rval}}
\newcommand{\prel}{\texttt{rel}}

% FIFO queue
\newcommand{\intfq}{\textsf{fq}}
\newcommand{\fq}{\text{FIFO queue}}
\newcommand{\enq}{\texttt{enq}}
\newcommand{\deq}{\texttt{deq}}

% register
\newcommand{\intreg}{\textsf{reg}}
\newcommand{\rd}{\texttt{rd}}
\renewcommand{\wr}{\texttt{wr}}

% key-value
\newcommand{\kv}{\textsf{kv}}
\newcommand{\kvput}{\texttt{put}}
\newcommand{\kvget}{\texttt{get}}

% protocol
\newcommand{\compare}{\textsc{compare}}
\newcommand{\merge}{\textsc{merge}}
\newcommand{\get}{\textsc{get}}
\newcommand{\pput}{\textsc{put}}
\newcommand{\ok}{\textsf{ok}}
\newcommand{\store}{\textsf{store}}
\newcommand{\tick}{\textsc{tick}}
\newcommand{\replicate}{\textsc{replicate}}

% GentleRain
\newcommand{\getreq}{\textsc{get-request}}
\newcommand{\getreply}{\textsc{get-reply}}
\newcommand{\putreq}{\textsc{put-request}}
\newcommand{\putreply}{\textsc{put-reply}}
\newcommand{\partition}{\textsc{partition}}
\newcommand{\vc}{\texttt{vc}}
\newcommand{\version}{\texttt{ver}}

% algorithm
\newcommand{\send}{{\bf send}\;}
\newcommand{\receive}{{\bf receive}\;}

\newcommand{\sr}{\texttt{sr}}

\newcommand{\queryreq}{\textsc{get-request}}
\newcommand{\updatereq}{\textsc{put-request}}
\newcommand{\pulloplog}{\textsc{pull-oplog}}

\newcommand{\client}{\textsl{Client}}
\newcommand{\server}{\textsl{Server}}

\newcommand{\ct}{\textsf{ct}}
\newcommand{\ot}{\textsf{ot}}
\newcommand{\aot}{\textsf{aot}}
\newcommand{\clock}{\textsf{clock}}
\newcommand{\hlc}{\textsl{hlc}}

\newcommand{\primary}{\textsc{primary}}
\newcommand{\isPrimary}{\textsc{IsPrimary}}
\newcommand{\isSecondary}{\textsc{IsSecondary}}
\newcommand{\rs}{\textsc{Cluster}}

\newcommand{\oplog}{\textsf{oplog}}
\newcommand{\syncsource}{\textsc{SyncSrc}}

\newcommand{\noopwrite}{\textsc{Noop}}
\newcommand{\noop}{\textsc{no-op}}

% rdt
\newcommand{\Obj}{\textsl{Obj}}
\newcommand{\Val}{\textsl{Val}}
\newcommand{\Type}{\textsl{Type}}
\newcommand{\Op}{\textsl{Op}}

\newcommand{\eval}{\texttt{eval}}

% concrete execution
\newcommand{\eo}{\texttt{eo}}
\newcommand{\ret}{\texttt{ret}}

% abstract execution
\newcommand{\vis}{\texttt{vis}}
\newcommand{\ar}{\texttt{ar}}
\newcommand{\nar}{\texttt{ar'}}
\newcommand{\fv}{\texttt{V}}
\renewcommand{\v}{\texttt{v}}

% arrows for relations
\newcommand{\rel}[1]{\xrightarrow{#1}}

% proof
\renewcommand{\so}{\texttt{so}}
\newcommand{\po}{\texttt{po}}
\newcommand{\hb}{\texttt{hb}}
\newcommand{\rf}{\texttt{rf}}
\newcommand{\ts}{\texttt{ts}}
\newcommand{\request}{\texttt{request}}

% kvs
\newcommand{\key}{\texttt{k}}
\newcommand{\ut}{\texttt{ut}}
\newcommand{\dt}{\texttt{dt}}
\newcommand{\gst}{\texttt{gst}}
\newcommand{\kvs}{\textsf{kvs}}
\newcommand{\fkvs}{\mathcal{F}}
\newcommand{\f}{\mathcal{F}}

% consistency
\newcommand{\ctxt}{\texttt{ctxt}}
\newcommand{\oc}{\textsl{Ctxt}}
\newcommand{\context}{\mathbb{C}}
\newcommand{\retval}{\textsc{RVal}}
\newcommand{\cc}{\textsc{CausalConsistency}}
\newcommand{\cv}{\textsc{CausalVisibility}}
\newcommand{\ca}{\textsc{CausalArbitration}}
\newcommand{\ev}{\textsl{EV}}

% sc
\renewcommand{\sc}{\textsl{SC}}

% cc
\newcommand{\wcc}{\textsl{WCC}}
\newcommand{\wccv}{\textsl{WCCv}}
\newcommand{\cm}{\textsl{CM}}
\newcommand{\cmv}{\textsl{CMv}}
\newcommand{\ccc}{\texttt{CC}}
\newcommand{\ccv}{\texttt{CCv}}
\newcommand{\scc}{\textsl{SCC}}
\newcommand{\sccv}{\textsl{SCCv}}

% pc
\newcommand{\wpc}{\textsl{WPC}}
\newcommand{\pc}{\textsl{PC}}
\newcommand{\wpcv}{\textsl{WPCv}}
\newcommand{\pcv}{\textsl{PCv}}
\newcommand{\pram}{\textsl{PRAM}}
\newcommand{\suc}{\textsl{SUC}}
\newcommand{\uc}{\textsl{UC}}

% comments
\newcommand{\hfwei}{\red{hfwei:\;}}
\newcommand{\xj}{\blue{xj:\;}}

